Higher Order Imprecise Probabilities and Statistical Testing

We generalize standard credal set models for imprecise probabilities to include higher order credal sets -- confidences about confidences. In doing so, we specify how an agent's higher order confidences (credal sets) update upon observing an event. Our model begins to address standard issues with imprecise probability models, like Dilation and Belief Inertia. We conjecture that when higher order credal sets contain all possible probability functions, then in the limiting case the highest order confidences converge to form a uniform distribution over the first order credal set, where we define uniformity in terms of the statistical distance metric (total variation distance). Finite simulation supports the conjecture. We further suggest that this convergence presents the total-variation-uniform distribution as a natural, privileged prior for statistical hypothesis testing.

==> data/binom_hocs_data_1_10.tex <==
% Value at 0.1: 3.866381637
\pgfplotstableread{
proportion hocsratio
0	0
0.001	0.09890347
0.002	0.196032014
0.003	0.291406889
0.004	0.385049152
0.005	0.476979667
0.006	0.567219097
0.007	0.655787918
0.008	0.742706408
0.009	0.827994657
0.01	0.911672565
0.011	0.993759845
0.012	1.074276021
0.013	1.153240434
0.014	1.230672241
0.015	1.306590415
0.016	1.381013751
0.017	1.453960863
0.018	1.525450184
0.019	1.595499976
0.02	1.66412832
0.021	1.731353126
0.022	1.797192131
0.023	1.8616629
0.024	1.924782827
0.025	1.986569139
0.026	2.047038894
0.027	2.106208985
0.028	2.164096139
0.029	2.22071692
0.03	2.27608773
0.031	2.33022481
0.032	2.383144239
0.033	2.43486194
0.034	2.485393678
0.035	2.534755062
0.036	2.582961545
0.037	2.630028428
0.038	2.675970858
0.039	2.720803832
0.04	2.764542197
0.041	2.80720065
0.042	2.848793742
0.043	2.889335876
0.044	2.92884131
0.045	2.96732416
0.046	3.004798395
0.047	3.041277845
0.048	3.076776199
0.049	3.111307007
0.05	3.144883678
0.051	3.177519486
0.052	3.209227568
0.053	3.240020926
0.054	3.269912429
0.055	3.29891481
0.056	3.327040674
0.057	3.354302492
0.058	3.380712608
0.059	3.406283235
0.06	3.43102646
0.061	3.454954243
0.062	3.478078417
0.063	3.500410694
0.064	3.521962659
0.065	3.542745777
0.066	3.56277139
0.067	3.58205072
0.068	3.60059487
0.069	3.618414825
0.07	3.635521451
0.071	3.6519255
0.072	3.667637605
0.073	3.682668287
0.074	3.697027954
0.075	3.7107269
0.076	3.723775308
0.077	3.736183249
0.078	3.747960686
0.079	3.759117472
0.08	3.769663354
0.081	3.779607968
0.082	3.788960849
0.083	3.797731422
0.084	3.805929012
0.085	3.813562838
0.086	3.820642016
0.087	3.827175563
0.088	3.833172393
0.089	3.838641321
0.09	3.843591063
0.091	3.848030236
0.092	3.851967361
0.093	3.855410862
0.094	3.858369068
0.095	3.860850211
0.096	3.862862432
0.097	3.864413776
0.098	3.865512198
0.099	3.866165561
0.1	3.866381637
0.101	3.866168107
0.102	3.865532565
0.103	3.864482515
0.104	3.863025374
0.105	3.861168473
0.106	3.858919056
0.107	3.856284282
0.108	3.853271226
0.109	3.849886879
0.11	3.846138149
0.111	3.842031861
0.112	3.837574761
0.113	3.832773512
0.114	3.827634698
0.115	3.822164823
0.116	3.816370313
0.117	3.810257517
0.118	3.803832704
0.119	3.797102071
0.12	3.790071735
0.121	3.78274774
0.122	3.775136057
0.123	3.767242581
0.124	3.759073135
0.125	3.750633469
0.126	3.741929263
0.127	3.732966124
0.128	3.723749592
0.129	3.714285132
0.13	3.704578146
0.131	3.694633964
0.132	3.684457848
0.133	3.674054995
0.134	3.663430536
0.135	3.652589533
0.136	3.641536985
0.137	3.630277827
0.138	3.61881693
0.139	3.607159099
0.14	3.595309079
0.141	3.583271552
0.142	3.571051139
0.143	3.5586524
0.144	3.546079834
0.145	3.53333788
0.146	3.520430918
0.147	3.507363271
0.148	3.494139203
0.149	3.480762919
0.15	3.467238569
0.151	3.453570246
0.152	3.439761987
0.153	3.425817775
0.154	3.411741535
0.155	3.397537143
0.156	3.383208416
0.157	3.368759122
0.158	3.354192975
0.159	3.339513635
0.16	3.324724714
0.161	3.309829771
0.162	3.294832315
0.163	3.279735804
0.164	3.264543647
0.165	3.249259206
0.166	3.233885792
0.167	3.218426669
0.168	3.202885054
0.169	3.187264116
0.17	3.171566978
0.171	3.155796716
0.172	3.139956363
0.173	3.124048903
0.174	3.10807728
0.175	3.092044391
0.176	3.075953088
0.177	3.059806183
0.178	3.043606443
0.179	3.027356593
0.18	3.011059317
0.181	2.994717257
0.182	2.978333014
0.183	2.961909148
0.184	2.945448179
0.185	2.928952588
0.186	2.912424815
0.187	2.895867263
0.188	2.879282297
0.189	2.86267224
0.19	2.846039383
0.191	2.829385974
0.192	2.812714229
0.193	2.796026325
0.194	2.779324404
0.195	2.762610571
0.196	2.745886897
0.197	2.729155418
0.198	2.712418135
0.199	2.695677016
0.2	2.678933994
0.201	2.662190969
0.202	2.645449808
0.203	2.628712347
0.204	2.611980387
0.205	2.5952557
0.206	2.578540023
0.207	2.561835066
0.208	2.545142504
0.209	2.528463986
0.21	2.511801127
0.211	2.495155514
0.212	2.478528704
0.213	2.461922227
0.214	2.445337581
0.215	2.428776237
0.216	2.41223964
0.217	2.395729204
0.218	2.379246317
0.219	2.36279234
0.22	2.346368608
0.221	2.329976428
0.222	2.313617081
0.223	2.297291823
0.224	2.281001885
0.225	2.264748471
0.226	2.248532762
0.227	2.232355913
0.228	2.216219055
0.229	2.200123295
0.23	2.184069716
0.231	2.16805938
0.232	2.152093321
0.233	2.136172555
0.234	2.120298073
0.235	2.104470844
0.236	2.088691814
0.237	2.07296191
0.238	2.057282035
0.239	2.041653072
0.24	2.026075882
0.241	2.010551307
0.242	1.995080166
0.243	1.979663262
0.244	1.964301374
0.245	1.948995263
0.246	1.933745671
0.247	1.91855332
0.248	1.903418915
0.249	1.888343139
0.25	1.87332666
0.251	1.858370126
0.252	1.843474167
0.253	1.828639397
0.254	1.81386641
0.255	1.799155786
0.256	1.784508084
0.257	1.769923851
0.258	1.755403614
0.259	1.740947884
0.26	1.726557157
0.261	1.712231914
0.262	1.697972617
0.263	1.683779717
0.264	1.669653647
0.265	1.655594825
0.266	1.641603655
0.267	1.627680527
0.268	1.613825815
0.269	1.600039879
0.27	1.586323068
0.271	1.572675714
0.272	1.559098136
0.273	1.545590641
0.274	1.532153521
0.275	1.518787057
0.276	1.505491516
0.277	1.492267152
0.278	1.479114207
0.279	1.466032912
0.28	1.453023485
0.281	1.440086131
0.282	1.427221045
0.283	1.41442841
0.284	1.401708398
0.285	1.389061169
0.286	1.376486872
0.287	1.363985646
0.288	1.351557619
0.289	1.339202909
0.29	1.326921622
0.291	1.314713856
0.292	1.302579699
0.293	1.290519226
0.294	1.278532507
0.295	1.266619598
0.296	1.254780549
0.297	1.243015399
0.298	1.231324179
0.299	1.219706911
0.3	1.208163607
0.301	1.196694271
0.302	1.185298899
0.303	1.17397748
0.304	1.162729991
0.305	1.151556405
0.306	1.140456685
0.307	1.129430786
0.308	1.118478657
0.309	1.107600238
0.31	1.096795462
0.311	1.086064256
0.312	1.075406539
0.313	1.064822221
0.314	1.054311209
0.315	1.043873402
0.316	1.03350869
0.317	1.02321696
0.318	1.01299809
0.319	1.002851953
0.32	0.992778417
0.321	0.982777343
0.322	0.972848584
0.323	0.962991991
0.324	0.953207407
0.325	0.94349467
0.326	0.933853613
0.327	0.924284064
0.328	0.914785845
0.329	0.905358772
0.33	0.89600266
0.331	0.886717313
0.332	0.877502537
0.333	0.868358127
0.334	0.859283879
0.335	0.85027958
0.336	0.841345016
0.337	0.832479966
0.338	0.823684208
0.339	0.814957514
0.34	0.80629965
0.341	0.797710383
0.342	0.789189472
0.343	0.780736675
0.344	0.772351744
0.345	0.76403443
0.346	0.755784478
0.347	0.747601632
0.348	0.739485632
0.349	0.731436214
0.35	0.723453111
0.351	0.715536055
0.352	0.707684773
0.353	0.699898989
0.354	0.692178425
0.355	0.684522802
0.356	0.676931835
0.357	0.669405239
0.358	0.661942726
0.359	0.654544004
0.36	0.647208781
0.361	0.639936763
0.362	0.63272765
0.363	0.625581145
0.364	0.618496945
0.365	0.611474748
0.366	0.604514247
0.367	0.597615137
0.368	0.590777107
0.369	0.583999848
0.37	0.577283047
0.371	0.570626391
0.372	0.564029564
0.373	0.557492249
0.374	0.55101413
0.375	0.544594885
0.376	0.538234196
0.377	0.531931739
0.378	0.525687193
0.379	0.519500232
0.38	0.513370533
0.381	0.507297768
0.382	0.501281611
0.383	0.495321734
0.384	0.489417809
0.385	0.483569506
0.386	0.477776494
0.387	0.472038444
0.388	0.466355024
0.389	0.460725901
0.39	0.455150744
0.391	0.449629219
0.392	0.444160993
0.393	0.438745732
0.394	0.433383102
0.395	0.428072769
0.396	0.422814398
0.397	0.417607655
0.398	0.412452203
0.399	0.407347709
0.4	0.402293837
0.401	0.397290251
0.402	0.392336618
0.403	0.3874326
0.404	0.382577863
0.405	0.377772073
0.406	0.373014894
0.407	0.368305992
0.408	0.363645031
0.409	0.359031679
0.41	0.354465601
0.411	0.349946464
0.412	0.345473934
0.413	0.341047678
0.414	0.336667365
0.415	0.332332662
0.416	0.328043237
0.417	0.323798761
0.418	0.319598902
0.419	0.31544333
0.42	0.311331717
0.421	0.307263734
0.422	0.303239053
0.423	0.299257346
0.424	0.295318288
0.425	0.291421552
0.426	0.287566814
0.427	0.283753748
0.428	0.279982033
0.429	0.276251345
0.43	0.272561362
0.431	0.268911764
0.432	0.265302231
0.433	0.261732444
0.434	0.258202085
0.435	0.254710836
0.436	0.251258383
0.437	0.247844408
0.438	0.2444686
0.439	0.241130644
0.44	0.237830229
0.441	0.234567044
0.442	0.231340779
0.443	0.228151126
0.444	0.224997778
0.445	0.221880427
0.446	0.21879877
0.447	0.215752501
0.448	0.212741319
0.449	0.209764922
0.45	0.20682301
0.451	0.203915283
0.452	0.201041444
0.453	0.198201197
0.454	0.195394247
0.455	0.192620299
0.456	0.189879061
0.457	0.187170242
0.458	0.184493552
0.459	0.181848702
0.46	0.179235406
0.461	0.176653378
0.462	0.174102333
0.463	0.171581989
0.464	0.169092063
0.465	0.166632276
0.466	0.164202349
0.467	0.161802004
0.468	0.159430966
0.469	0.157088961
0.47	0.154775715
0.471	0.152490957
0.472	0.150234417
0.473	0.148005826
0.474	0.145804918
0.475	0.143631427
0.476	0.141485088
0.477	0.13936564
0.478	0.137272821
0.479	0.135206371
0.48	0.133166034
0.481	0.131151551
0.482	0.129162669
0.483	0.127199134
0.484	0.125260693
0.485	0.123347098
0.486	0.121458098
0.487	0.119593446
0.488	0.117752898
0.489	0.115936209
0.49	0.114143136
0.491	0.112373438
0.492	0.110626876
0.493	0.108903212
0.494	0.107202209
0.495	0.105523633
0.496	0.103867251
0.497	0.102232831
0.498	0.100620143
0.499	0.099028959
0.5	0.097459051
0.501	0.095910194
0.502	0.094382165
0.503	0.092874742
0.504	0.091387703
0.505	0.089920829
0.506	0.088473904
0.507	0.087046711
0.508	0.085639036
0.509	0.084250667
0.51	0.082881391
0.511	0.081531
0.512	0.080199284
0.513	0.078886039
0.514	0.077591059
0.515	0.076314139
0.516	0.07505508
0.517	0.073813679
0.518	0.07258974
0.519	0.071383063
0.52	0.070193454
0.521	0.069020719
0.522	0.067864665
0.523	0.0667251
0.524	0.065601836
0.525	0.064494685
0.526	0.063403459
0.527	0.062327975
0.528	0.061268048
0.529	0.060223497
0.53	0.059194141
0.531	0.058179802
0.532	0.057180302
0.533	0.056195465
0.534	0.055225117
0.535	0.054269084
0.536	0.053327196
0.537	0.052399282
0.538	0.051485175
0.539	0.050584706
0.54	0.04969771
0.541	0.048824024
0.542	0.047963484
0.543	0.04711593
0.544	0.046281201
0.545	0.045459139
0.546	0.044649588
0.547	0.043852391
0.548	0.043067395
0.549	0.042294447
0.55	0.041533396
0.551	0.040784092
0.552	0.040046387
0.553	0.039320133
0.554	0.038605184
0.555	0.037901397
0.556	0.037208628
0.557	0.036526736
0.558	0.03585558
0.559	0.035195023
0.56	0.034544925
0.561	0.033905151
0.562	0.033275565
0.563	0.032656036
0.564	0.032046429
0.565	0.031446614
0.566	0.030856462
0.567	0.030275844
0.568	0.029704633
0.569	0.029142703
0.57	0.02858993
0.571	0.02804619
0.572	0.027511362
0.573	0.026985324
0.574	0.026467957
0.575	0.025959143
0.576	0.025458765
0.577	0.024966706
0.578	0.024482853
0.579	0.024007092
0.58	0.023539311
0.581	0.023079398
0.582	0.022627244
0.583	0.02218274
0.584	0.021745778
0.585	0.021316253
0.586	0.020894059
0.587	0.020479092
0.588	0.020071249
0.589	0.019670429
0.59	0.01927653
0.591	0.018889453
0.592	0.0185091
0.593	0.018135374
0.594	0.017768177
0.595	0.017407416
0.596	0.017052996
0.597	0.016704823
0.598	0.016362807
0.599	0.016026855
0.6	0.015696879
0.601	0.015372789
0.602	0.015054498
0.603	0.014741919
0.604	0.014434965
0.605	0.014133554
0.606	0.013837599
0.607	0.01354702
0.608	0.013261734
0.609	0.01298166
0.61	0.012706719
0.611	0.012436832
0.612	0.01217192
0.613	0.011911907
0.614	0.011656717
0.615	0.011406274
0.616	0.011160506
0.617	0.010919337
0.618	0.010682696
0.619	0.010450512
0.62	0.010222714
0.621	0.009999232
0.622	0.009779997
0.623	0.009564942
0.624	0.009353999
0.625	0.009147103
0.626	0.008944187
0.627	0.008745188
0.628	0.008550042
0.629	0.008358685
0.63	0.008171056
0.631	0.007987094
0.632	0.007806738
0.633	0.007629928
0.634	0.007456605
0.635	0.007286713
0.636	0.007120192
0.637	0.006956987
0.638	0.006797042
0.639	0.006640302
0.64	0.006486712
0.641	0.006336219
0.642	0.006188771
0.643	0.006044314
0.644	0.005902799
0.645	0.005764173
0.646	0.005628388
0.647	0.005495393
0.648	0.005365141
0.649	0.005237583
0.65	0.005112672
0.651	0.004990361
0.652	0.004870605
0.653	0.004753359
0.654	0.004638577
0.655	0.004526216
0.656	0.004416233
0.657	0.004308584
0.658	0.004203228
0.659	0.004100124
0.66	0.003999229
0.661	0.003900505
0.662	0.003803912
0.663	0.003709409
0.664	0.00361696
0.665	0.003526526
0.666	0.003438069
0.667	0.003351553
0.668	0.003266941
0.669	0.003184199
0.67	0.00310329
0.671	0.003024181
0.672	0.002946836
0.673	0.002871223
0.674	0.002797309
0.675	0.002725061
0.676	0.002654446
0.677	0.002585434
0.678	0.002517994
0.679	0.002452094
0.68	0.002387706
0.681	0.002324799
0.682	0.002263344
0.683	0.002203313
0.684	0.002144677
0.685	0.00208741
0.686	0.002031482
0.687	0.001976869
0.688	0.001923543
0.689	0.001871479
0.69	0.00182065
0.691	0.001771032
0.692	0.001722601
0.693	0.001675331
0.694	0.0016292
0.695	0.001584184
0.696	0.001540259
0.697	0.001497403
0.698	0.001455593
0.699	0.001414809
0.7	0.001375028
0.701	0.001336229
0.702	0.001298391
0.703	0.001261495
0.704	0.001225519
0.705	0.001190445
0.706	0.001156253
0.707	0.001122923
0.708	0.001090438
0.709	0.001058779
0.71	0.001027927
0.711	0.000997866
0.712	0.000968578
0.713	0.000940045
0.714	0.000912252
0.715	0.000885181
0.716	0.000858816
0.717	0.000833142
0.718	0.000808144
0.719	0.000783805
0.72	0.000760111
0.721	0.000737047
0.722	0.000714599
0.723	0.000692753
0.724	0.000671494
0.725	0.00065081
0.726	0.000630687
0.727	0.000611111
0.728	0.000592071
0.729	0.000573553
0.73	0.000555545
0.731	0.000538034
0.732	0.00052101
0.733	0.000504461
0.734	0.000488374
0.735	0.00047274
0.736	0.000457547
0.737	0.000442783
0.738	0.00042844
0.739	0.000414506
0.74	0.000400972
0.741	0.000387827
0.742	0.000375062
0.743	0.000362668
0.744	0.000350635
0.745	0.000338953
0.746	0.000327615
0.747	0.000316612
0.748	0.000305935
0.749	0.000295575
0.75	0.000285525
0.751	0.000275776
0.752	0.000266321
0.753	0.000257152
0.754	0.000248262
0.755	0.000239643
0.756	0.000231288
0.757	0.00022319
0.758	0.000215342
0.759	0.000207739
0.76	0.000200372
0.761	0.000193236
0.762	0.000186324
0.763	0.000179631
0.764	0.00017315
0.765	0.000166876
0.766	0.000160803
0.767	0.000154925
0.768	0.000149237
0.769	0.000143733
0.77	0.000138409
0.771	0.000133259
0.772	0.000128278
0.773	0.000123462
0.774	0.000118806
0.775	0.000114305
0.776	0.000109955
0.777	0.000105752
0.778	0.00010169
0.779	9.77664971e-05
0.78	9.39768458e-05
0.781	9.03171452e-05
0.782	8.67835337e-05
0.783	8.33722459e-05
0.784	8.00796115e-05
0.785	7.69020523e-05
0.786	7.38360815e-05
0.787	7.08783008e-05
0.788	6.80253994e-05
0.789	6.52741515e-05
0.79	6.26214152e-05
0.791	6.00641302e-05
0.792	5.75993166e-05
0.793	5.52240725e-05
0.794	5.29355732e-05
0.795	5.07310688e-05
0.796	4.86078832e-05
0.797	4.65634120e-05
0.798	4.45951214e-05
0.799	4.27005462e-05
0.8	4.08772887e-05
0.801	3.91230169e-05
0.802	3.74354635e-05
0.803	3.58124238e-05
0.804	3.42517547e-05
0.805	3.27513734e-05
0.806	3.13092558e-05
0.807	2.99234352e-05
0.808	2.85920012e-05
0.809	2.73130979e-05
0.81	2.60849231e-05
0.811	2.49057271e-05
0.812	2.37738110e-05
0.813	2.26875259e-05
0.814	2.16452714e-05
0.815	2.06454949e-05
0.816	1.96866898e-05
0.817	1.87673951e-05
0.818	1.78861937e-05
0.819	1.70417115e-05
0.82	1.62326166e-05
0.821	1.54576179e-05
0.822	1.47154644e-05
0.823	1.40049436e-05
0.824	1.33248815e-05
0.825	1.26741406e-05
0.826	1.20516196e-05
0.827	1.14562523e-05
0.828	1.08870067e-05
0.829	1.03428841e-05
0.83	9.82291801e-06
0.831	9.32617369e-06
0.832	8.85174707e-06
0.833	8.39876396e-06
0.834	7.96637924e-06
0.835	7.55377610e-06
0.836	7.16016523e-06
0.837	6.78478409e-06
0.838	6.42689617e-06
0.839	6.08579024e-06
0.84	5.76077965e-06
0.841	5.45120166e-06
0.842	5.15641672e-06
0.843	4.87580783e-06
0.844	4.60877988e-06
0.845	4.35475901e-06
0.846	4.11319202e-06
0.847	3.88354571e-06
0.848	3.66530634e-06
0.849	3.45797899e-06
0.85	3.26108704e-06
0.851	3.07417162e-06
0.852	2.89679103e-06
0.853	2.72852023e-06
0.854	2.56895032e-06
0.855	2.41768808e-06
0.856	2.27435538e-06
0.857	2.13858882e-06
0.858	2.01003917e-06
0.859	1.88837095e-06
0.86	1.77326199e-06
0.861	1.66440299e-06
0.862	1.56149708e-06
0.863	1.46425944e-06
0.864	1.37241688e-06
0.865	1.28570744e-06
0.866	1.20388003e-06
0.867	1.12669404e-06
0.868	1.05391901e-06
0.869	9.85334233e-07
0.87	9.20728439e-07
0.871	8.59899471e-07
0.872	8.02653948e-07
0.873	7.48806950e-07
0.874	6.98181719e-07
0.875	6.50609356e-07
0.876	6.05928537e-07
0.877	5.63985230e-07
0.878	5.24632422e-07
0.879	4.87729857e-07
0.88	4.53143777e-07
0.881	4.20746677e-07
0.882	3.90417058e-07
0.883	3.62039197e-07
0.884	3.35502918e-07
0.885	3.10703373e-07
0.886	2.87540827e-07
0.887	2.65920455e-07
0.888	2.45752137e-07
0.889	2.26950270e-07
0.89	2.09433575e-07
0.891	1.93124921e-07
0.892	1.77951145e-07
0.893	1.63842887e-07
0.894	1.50734422e-07
0.895	1.38563505e-07
0.896	1.27271217e-07
0.897	1.16801817e-07
0.898	1.07102600e-07
0.899	9.81237619e-08
0.9	8.98182613e-08
0.901	8.21416981e-08
0.902	7.50521872e-08
0.903	6.85102406e-08
0.904	6.24786536e-08
0.905	5.69223945e-08
0.906	5.18084995e-08
0.907	4.71059708e-08
0.908	4.27856790e-08
0.909	3.88202697e-08
0.91	3.51840728e-08
0.911	3.18530168e-08
0.912	2.88045451e-08
0.913	2.60175372e-08
0.914	2.34722321e-08
0.915	2.11501552e-08
0.916	1.90340489e-08
0.917	1.71078054e-08
0.918	1.53564025e-08
0.919	1.37658431e-08
0.92	1.23230963e-08
0.921	1.10160420e-08
0.922	9.83341752e-09
0.923	8.76476673e-09
0.924	7.80039214e-09
0.925	6.93130864e-09
0.926	6.14919972e-09
0.927	5.44637586e-09
0.928	4.81573497e-09
0.929	4.25072478e-09
0.93	3.74530718e-09
0.931	3.29392443e-09
0.932	2.89146714e-09
0.933	2.53324388e-09
0.934	2.21495256e-09
0.935	1.93265331e-09
0.936	1.68274283e-09
0.937	1.46193031e-09
0.938	1.26721463e-09
0.939	1.09586294e-09
0.94	9.45390516e-10
0.941	8.13541782e-10
0.942	6.98272565e-10
0.943	5.97733406e-10
0.944	5.10253945e-10
0.945	4.34328320e-10
0.946	3.68601509e-10
0.947	3.11856600e-10
0.948	2.63002916e-10
0.949	2.21064971e-10
0.95	1.85172196e-10
0.951	1.54549417e-10
0.952	1.28508016e-10
0.953	1.06437767e-10
0.954	8.77992880e-11
0.955	7.21170793e-11
0.956	5.89731213e-11
0.957	4.80009875e-11
0.958	3.88804477e-11
0.959	3.13325291e-11
0.96	2.51150061e-11
0.961	2.00182904e-11
0.962	1.58616943e-11
0.963	1.24900431e-11
0.964	9.77060992e-12
0.965	7.59035078e-12
0.966	5.85341767e-12
0.967	4.47892786e-12
0.968	3.39896972e-12
0.969	2.55682589e-12
0.97	1.90539561e-12
0.971	1.40579937e-12
0.972	1.02614960e-12
0.973	7.40472360e-13
0.974	5.27765774e-13
0.975	3.71181932e-13
0.976	2.57319754e-13
0.977	1.75617270e-13
0.978	1.17832506e-13
0.979	7.76029943e-14
0.98	5.00746786e-14
0.981	3.15917402e-14
0.982	1.94395482e-14
0.983	1.16336486e-14
0.984	6.74834188e-15
0.985	3.77902440e-15
0.986	2.03306549e-15
0.987	1.04455054e-15
0.988	5.08756877e-16
0.989	2.32730119e-16
0.99	9.88000874e-17
0.991	3.83158420e-17
0.992	1.32875126e-17
0.993	3.99902153e-18
0.994	9.99700184e-19
0.995	1.93943511e-19
0.996	2.60568189e-20
0.997	1.95843239E-21
0.998	5.09944176e-23
0.999	9.96982700e-26
1	0

}{\hocsdataoneoften}


==> data/binom_hocs_data_4_10.tex <==
% Value at 0.4: 3.733746474
\pgfplotstableread{
proportion hocsratio
0	0
0.001	3.10735081e-09
0.002	4.94197550e-08
0.003	2.48687139e-07
0.004	7.81255978e-07
0.005	1.89590189e-06
0.006	3.90769505e-06
0.007	7.19589816e-06
0.008	1.22018965e-05
0.009	1.94271602e-05
0.01	2.94312376e-05
0.011	4.28297804e-05
0.012	6.02925996e-05
0.013	8.25417520e-05
0.014	0.00011035
0.015	0.000144537
0.016	0.000185972
0.017	0.000235567
0.018	0.000294277
0.019	0.0003631
0.02	0.000443071
0.021	0.000535267
0.022	0.000640798
0.023	0.00076081
0.024	0.000896481
0.025	0.001049023
0.026	0.001219676
0.027	0.001409709
0.028	0.001620418
0.029	0.001853125
0.03	0.002109176
0.031	0.002389939
0.032	0.002696804
0.033	0.003031182
0.034	0.0033945
0.035	0.003788204
0.036	0.004213758
0.037	0.004672636
0.038	0.00516633
0.039	0.005696343
0.04	0.006264187
0.041	0.006871387
0.042	0.007519476
0.043	0.008209993
0.044	0.008944487
0.045	0.009724508
0.046	0.010551615
0.047	0.011427367
0.048	0.012353329
0.049	0.013331063
0.05	0.014362135
0.051	0.015448109
0.052	0.016590549
0.053	0.017791014
0.054	0.019051063
0.055	0.020372249
0.056	0.021756119
0.057	0.023204218
0.058	0.024718081
0.059	0.026299237
0.06	0.027949206
0.061	0.029669502
0.062	0.031461625
0.063	0.033327067
0.064	0.035267311
0.065	0.037283824
0.066	0.039378064
0.067	0.041551474
0.068	0.043805484
0.069	0.04614151
0.07	0.048560954
0.071	0.0510652
0.072	0.053655618
0.073	0.056333561
0.074	0.059100364
0.075	0.061957346
0.076	0.064905807
0.077	0.067947028
0.078	0.071082271
0.079	0.074312779
0.08	0.077639775
0.081	0.081064461
0.082	0.084588019
0.083	0.088211609
0.084	0.091936368
0.085	0.095763415
0.086	0.099693843
0.087	0.103728724
0.088	0.107869105
0.089	0.112116013
0.09	0.116470449
0.091	0.12093339
0.092	0.125505789
0.093	0.130188575
0.094	0.134982653
0.095	0.1398889
0.096	0.14490817
0.097	0.150041293
0.098	0.155289069
0.099	0.160652276
0.1	0.166131664
0.101	0.171727957
0.102	0.177441853
0.103	0.183274024
0.104	0.189225113
0.105	0.195295738
0.106	0.20148649
0.107	0.207797932
0.108	0.214230601
0.109	0.220785005
0.11	0.227461625
0.111	0.234260917
0.112	0.241183306
0.113	0.24822919
0.114	0.255398942
0.115	0.262692905
0.116	0.270111394
0.117	0.277654698
0.118	0.285323076
0.119	0.293116762
0.12	0.301035959
0.121	0.309080844
0.122	0.317251567
0.123	0.325548249
0.124	0.333970984
0.125	0.342519837
0.126	0.351194846
0.127	0.359996024
0.128	0.368923352
0.129	0.377976787
0.13	0.387156257
0.131	0.396461664
0.132	0.405892881
0.133	0.415449754
0.134	0.425132105
0.135	0.434939726
0.136	0.444872383
0.137	0.454929815
0.138	0.465111736
0.139	0.475417832
0.14	0.485847764
0.141	0.496401164
0.142	0.507077642
0.143	0.51787678
0.144	0.528798134
0.145	0.539841236
0.146	0.55100559
0.147	0.562290678
0.148	0.573695955
0.149	0.585220852
0.15	0.596864774
0.151	0.608627103
0.152	0.620507197
0.153	0.632504389
0.154	0.644617987
0.155	0.656847278
0.156	0.669191523
0.157	0.681649963
0.158	0.694221812
0.159	0.706906264
0.16	0.719702489
0.161	0.732609637
0.162	0.745626832
0.163	0.758753179
0.164	0.77198776
0.165	0.785329638
0.166	0.798777851
0.167	0.812331419
0.168	0.82598934
0.169	0.839750593
0.17	0.853614134
0.171	0.867578903
0.172	0.881643817
0.173	0.895807775
0.174	0.910069658
0.175	0.924428325
0.176	0.938882619
0.177	0.953431365
0.178	0.968073367
0.179	0.982807415
0.18	0.997632279
0.181	1.012546712
0.182	1.027549452
0.183	1.042639217
0.184	1.057814711
0.185	1.073074622
0.186	1.088417621
0.187	1.103842364
0.188	1.119347492
0.189	1.13493163
0.19	1.150593391
0.191	1.16633137
0.192	1.18214415
0.193	1.1980303
0.194	1.213988376
0.195	1.23001692
0.196	1.24611446
0.197	1.262279515
0.198	1.278510587
0.199	1.294806169
0.2	1.311164743
0.201	1.327584776
0.202	1.344064727
0.203	1.360603043
0.204	1.377198161
0.205	1.393848506
0.206	1.410552497
0.207	1.427308538
0.208	1.444115027
0.209	1.460970354
0.21	1.477872897
0.211	1.494821027
0.212	1.511813108
0.213	1.528847494
0.214	1.545922533
0.215	1.563036566
0.216	1.580187924
0.217	1.597374936
0.218	1.61459592
0.219	1.631849191
0.22	1.649133057
0.221	1.666445821
0.222	1.683785781
0.223	1.701151228
0.224	1.71854045
0.225	1.735951732
0.226	1.753383351
0.227	1.770833585
0.228	1.788300706
0.229	1.805782981
0.23	1.823278677
0.231	1.840786058
0.232	1.858303384
0.233	1.875828914
0.234	1.893360905
0.235	1.910897613
0.236	1.928437292
0.237	1.945978195
0.238	1.963518575
0.239	1.981056685
0.24	1.998590775
0.241	2.016119098
0.242	2.033639907
0.243	2.051151454
0.244	2.068651994
0.245	2.086139783
0.246	2.103613075
0.247	2.12107013
0.248	2.138509209
0.249	2.155928573
0.25	2.173326487
0.251	2.19070122
0.252	2.208051041
0.253	2.225374224
0.254	2.242669048
0.255	2.259933792
0.256	2.277166742
0.257	2.294366188
0.258	2.311530421
0.259	2.328657742
0.26	2.345746452
0.261	2.362794861
0.262	2.379801282
0.263	2.396764034
0.264	2.413681443
0.265	2.430551839
0.266	2.44737356
0.267	2.464144951
0.268	2.480864361
0.269	2.49753015
0.27	2.51414068
0.271	2.530694326
0.272	2.547189465
0.273	2.563624487
0.274	2.579997787
0.275	2.596307767
0.276	2.612552842
0.277	2.628731431
0.278	2.644841964
0.279	2.66088288
0.28	2.676852626
0.281	2.69274966
0.282	2.708572449
0.283	2.724319469
0.284	2.739989206
0.285	2.755580157
0.286	2.771090829
0.287	2.78651974
0.288	2.801865416
0.289	2.817126398
0.29	2.832301235
0.291	2.847388489
0.292	2.86238673
0.293	2.877294543
0.294	2.892110524
0.295	2.90683328
0.296	2.92146143
0.297	2.935993605
0.298	2.950428449
0.299	2.964764617
0.3	2.979000779
0.301	2.993135616
0.302	3.007167821
0.303	3.021096102
0.304	3.034919178
0.305	3.048635783
0.306	3.062244664
0.307	3.075744581
0.308	3.089134307
0.309	3.102412631
0.31	3.115578353
0.311	3.128630289
0.312	3.141567268
0.313	3.154388134
0.314	3.167091746
0.315	3.179676975
0.316	3.192142708
0.317	3.204487847
0.318	3.216711308
0.319	3.228812022
0.32	3.240788935
0.321	3.252641009
0.322	3.264367218
0.323	3.275966555
0.324	3.287438026
0.325	3.298780653
0.326	3.309993473
0.327	3.321075539
0.328	3.332025919
0.329	3.342843698
0.33	3.353527975
0.331	3.364077866
0.332	3.374492503
0.333	3.384771031
0.334	3.394912616
0.335	3.404916436
0.336	3.414781687
0.337	3.42450758
0.338	3.434093343
0.339	3.44353822
0.34	3.452841472
0.341	3.462002375
0.342	3.471020222
0.343	3.479894322
0.344	3.488624002
0.345	3.497208604
0.346	3.505647486
0.347	3.513940024
0.348	3.522085611
0.349	3.530083654
0.35	3.537933578
0.351	3.545634827
0.352	3.553186857
0.353	3.560589145
0.354	3.567841181
0.355	3.574942475
0.356	3.581892552
0.357	3.588690953
0.358	3.595337238
0.359	3.601830981
0.36	3.608171775
0.361	3.614359228
0.362	3.620392965
0.363	3.62627263
0.364	3.63199788
0.365	3.637568392
0.366	3.642983857
0.367	3.648243984
0.368	3.653348499
0.369	3.658297144
0.37	3.663089677
0.371	3.667725874
0.372	3.672205526
0.373	3.676528442
0.374	3.680694447
0.375	3.684703381
0.376	3.688555103
0.377	3.692249486
0.378	3.69578642
0.379	3.699165814
0.38	3.702387588
0.381	3.705451683
0.382	3.708358054
0.383	3.711106673
0.384	3.713697526
0.385	3.716130618
0.386	3.718405968
0.387	3.720523612
0.388	3.722483601
0.389	3.724286001
0.39	3.725930898
0.391	3.727418387
0.392	3.728748585
0.393	3.729921621
0.394	3.73093764
0.395	3.731796803
0.396	3.732499286
0.397	3.73304528
0.398	3.733434993
0.399	3.733668645
0.4	3.733746474
0.401	3.733668732
0.402	3.733435684
0.403	3.733047614
0.404	3.732504816
0.405	3.731807603
0.406	3.730956298
0.407	3.729951244
0.408	3.728792794
0.409	3.727481316
0.41	3.726017194
0.411	3.724400824
0.412	3.722632619
0.413	3.720713003
0.414	3.718642414
0.415	3.716421306
0.416	3.714050145
0.417	3.711529411
0.418	3.708859597
0.419	3.706041209
0.42	3.703074768
0.421	3.699960806
0.422	3.69669987
0.423	3.693292519
0.424	3.689739324
0.425	3.68604087
0.426	3.682197753
0.427	3.678210584
0.428	3.674079985
0.429	3.669806589
0.43	3.665391043
0.431	3.660834005
0.432	3.656136145
0.433	3.651298146
0.434	3.646320701
0.435	3.641204515
0.436	3.635950306
0.437	3.6305588
0.438	3.625030737
0.439	3.619366867
0.44	3.613567952
0.441	3.607634763
0.442	3.601568083
0.443	3.595368704
0.444	3.589037432
0.445	3.582575079
0.446	3.57598247
0.447	3.569260438
0.448	3.562409828
0.449	3.555431493
0.45	3.548326298
0.451	3.541095114
0.452	3.533738825
0.453	3.526258321
0.454	3.518654503
0.455	3.510928282
0.456	3.503080575
0.457	3.49511231
0.458	3.487024423
0.459	3.478817857
0.46	3.470493566
0.461	3.462052509
0.462	3.453495656
0.463	3.444823984
0.464	3.436038476
0.465	3.427140124
0.466	3.418129928
0.467	3.409008894
0.468	3.399778037
0.469	3.390438377
0.47	3.380990942
0.471	3.371436767
0.472	3.361776892
0.473	3.352012366
0.474	3.342144242
0.475	3.332173581
0.476	3.322101449
0.477	3.311928918
0.478	3.301657066
0.479	3.291286977
0.48	3.280819739
0.481	3.270256447
0.482	3.2595982
0.483	3.248846103
0.484	3.238001266
0.485	3.227064803
0.486	3.216037832
0.487	3.204921477
0.488	3.193716866
0.489	3.18242513
0.49	3.171047406
0.491	3.159584833
0.492	3.148038555
0.493	3.136409719
0.494	3.124699476
0.495	3.11290898
0.496	3.101039388
0.497	3.089091861
0.498	3.077067561
0.499	3.064967654
0.5	3.05279331
0.501	3.040545698
0.502	3.028225994
0.503	3.015835371
0.504	3.003375008
0.505	2.990846085
0.506	2.978249783
0.507	2.965587284
0.508	2.952859774
0.509	2.940068438
0.51	2.927214464
0.511	2.91429904
0.512	2.901323354
0.513	2.888288597
0.514	2.875195959
0.515	2.862046633
0.516	2.848841809
0.517	2.835582679
0.518	2.822270435
0.519	2.80890627
0.52	2.795491375
0.521	2.782026942
0.522	2.768514163
0.523	2.754954227
0.524	2.741348326
0.525	2.727697648
0.526	2.714003382
0.527	2.700266715
0.528	2.686488834
0.529	2.672670923
0.53	2.658814165
0.531	2.644919744
0.532	2.630988838
0.533	2.617022626
0.534	2.603022285
0.535	2.588988989
0.536	2.57492391
0.537	2.560828219
0.538	2.546703082
0.539	2.532549665
0.54	2.518369131
0.541	2.504162638
0.542	2.489931343
0.543	2.4756764
0.544	2.461398959
0.545	2.447100169
0.546	2.432781171
0.547	2.418443107
0.548	2.404087114
0.549	2.389714325
0.55	2.375325869
0.551	2.360922871
0.552	2.346506453
0.553	2.332077731
0.554	2.317637819
0.555	2.303187826
0.556	2.288728855
0.557	2.274262005
0.558	2.259788373
0.559	2.245309047
0.56	2.230825113
0.561	2.216337651
0.562	2.201847737
0.563	2.18735644
0.564	2.172864825
0.565	2.158373951
0.566	2.143884872
0.567	2.129398636
0.568	2.114916286
0.569	2.10043886
0.57	2.085967386
0.571	2.071502892
0.572	2.057046396
0.573	2.04259891
0.574	2.028161443
0.575	2.013734993
0.576	1.999320556
0.577	1.984919118
0.578	1.970531662
0.579	1.956159161
0.58	1.941802583
0.581	1.92746289
0.582	1.913141036
0.583	1.898837967
0.584	1.884554624
0.585	1.870291941
0.586	1.856050843
0.587	1.841832249
0.588	1.82763707
0.589	1.813466212
0.59	1.79932057
0.591	1.785201033
0.592	1.771108484
0.593	1.757043795
0.594	1.743007835
0.595	1.72900146
0.596	1.715025523
0.597	1.701080865
0.598	1.687168321
0.599	1.673288719
0.6	1.659442877
0.601	1.645631607
0.602	1.63185571
0.603	1.618115981
0.604	1.604413206
0.605	1.590748163
0.606	1.577121621
0.607	1.563534341
0.608	1.549987076
0.609	1.536480571
0.61	1.523015559
0.611	1.509592769
0.612	1.496212918
0.613	1.482876716
0.614	1.469584865
0.615	1.456338055
0.616	1.443136971
0.617	1.429982287
0.618	1.416874668
0.619	1.403814772
0.62	1.390803246
0.621	1.377840729
0.622	1.364927851
0.623	1.352065234
0.624	1.339253488
0.625	1.326493217
0.626	1.313785015
0.627	1.301129466
0.628	1.288527145
0.629	1.27597862
0.63	1.263484446
0.631	1.251045174
0.632	1.23866134
0.633	1.226333476
0.634	1.2140621
0.635	1.201847725
0.636	1.189690853
0.637	1.177591975
0.638	1.165551576
0.639	1.15357013
0.64	1.141648101
0.641	1.129785944
0.642	1.117984108
0.643	1.106243027
0.644	1.09456313
0.645	1.082944836
0.646	1.071388553
0.647	1.059894681
0.648	1.048463612
0.649	1.037095725
0.65	1.025791393
0.651	1.014550978
0.652	1.003374835
0.653	0.992263307
0.654	0.981216729
0.655	0.970235427
0.656	0.959319717
0.657	0.948469907
0.658	0.937686295
0.659	0.92696917
0.66	0.916318811
0.661	0.905735489
0.662	0.895219466
0.663	0.884770995
0.664	0.874390317
0.665	0.864077669
0.666	0.853833274
0.667	0.84365735
0.668	0.833550104
0.669	0.823511734
0.67	0.813542429
0.671	0.803642371
0.672	0.79381173
0.673	0.784050671
0.674	0.774359346
0.675	0.764737902
0.676	0.755186474
0.677	0.745705192
0.678	0.736294173
0.679	0.726953529
0.68	0.717683363
0.681	0.708483767
0.682	0.699354826
0.683	0.690296618
0.684	0.681309211
0.685	0.672392664
0.686	0.663547029
0.687	0.65477235
0.688	0.646068661
0.689	0.637435989
0.69	0.628874353
0.691	0.620383765
0.692	0.611964226
0.693	0.603615731
0.694	0.595338267
0.695	0.587131812
0.696	0.578996339
0.697	0.570931811
0.698	0.562938182
0.699	0.555015401
0.7	0.547163408
0.701	0.539382137
0.702	0.531671512
0.703	0.524031452
0.704	0.516461867
0.705	0.50896266
0.706	0.501533728
0.707	0.494174959
0.708	0.486886236
0.709	0.479667432
0.71	0.472518417
0.711	0.46543905
0.712	0.458429186
0.713	0.451488671
0.714	0.444617348
0.715	0.437815049
0.716	0.431081601
0.717	0.424416827
0.718	0.417820539
0.719	0.411292546
0.72	0.40483265
0.721	0.398440647
0.722	0.392116325
0.723	0.385859468
0.724	0.379669854
0.725	0.373547253
0.726	0.367491432
0.727	0.361502149
0.728	0.35557916
0.729	0.349722212
0.73	0.343931048
0.731	0.338205406
0.732	0.332545018
0.733	0.326949611
0.734	0.321418905
0.735	0.315952618
0.736	0.31055046
0.737	0.305212137
0.738	0.299937352
0.739	0.2947258
0.74	0.289577173
0.741	0.284491159
0.742	0.279467439
0.743	0.274505691
0.744	0.26960559
0.745	0.264766803
0.746	0.259988996
0.747	0.25527183
0.748	0.250614961
0.749	0.246018042
0.75	0.241480721
0.751	0.237002643
0.752	0.232583448
0.753	0.228222775
0.754	0.223920257
0.755	0.219675524
0.756	0.215488202
0.757	0.211357916
0.758	0.207284284
0.759	0.203266925
0.76	0.199305451
0.761	0.195399474
0.762	0.191548602
0.763	0.187752438
0.764	0.184010587
0.765	0.180322646
0.766	0.176688214
0.767	0.173106884
0.768	0.169578249
0.769	0.166101899
0.77	0.162677419
0.771	0.159304397
0.772	0.155982415
0.773	0.152711055
0.774	0.149489895
0.775	0.146318512
0.776	0.143196483
0.777	0.140123382
0.778	0.137098781
0.779	0.13412225
0.78	0.13119336
0.781	0.128311677
0.782	0.12547677
0.783	0.122688204
0.784	0.119945543
0.785	0.117248351
0.786	0.114596191
0.787	0.111988624
0.788	0.109425211
0.789	0.106905513
0.79	0.104429089
0.791	0.101995499
0.792	0.099604301
0.793	0.097255054
0.794	0.094947315
0.795	0.092680643
0.796	0.090454595
0.797	0.088268729
0.798	0.086122601
0.799	0.084015771
0.8	0.081947796
0.801	0.079918234
0.802	0.077926644
0.803	0.075972584
0.804	0.074055613
0.805	0.072175292
0.806	0.07033118
0.807	0.068522839
0.808	0.066749831
0.809	0.065011719
0.81	0.063308065
0.811	0.061638434
0.812	0.060002393
0.813	0.058399507
0.814	0.056829344
0.815	0.055291473
0.816	0.053785465
0.817	0.052310892
0.818	0.050867325
0.819	0.04945434
0.82	0.048071514
0.821	0.046718423
0.822	0.045394647
0.823	0.044099767
0.824	0.042833367
0.825	0.04159503
0.826	0.040384344
0.827	0.039200898
0.828	0.038044281
0.829	0.036914088
0.83	0.035809912
0.831	0.034731351
0.832	0.033678005
0.833	0.032649474
0.834	0.031645364
0.835	0.030665279
0.836	0.02970883
0.837	0.028775628
0.838	0.027865287
0.839	0.026977423
0.84	0.026111655
0.841	0.025267605
0.842	0.024444899
0.843	0.023643163
0.844	0.022862027
0.845	0.022101125
0.846	0.021360093
0.847	0.020638569
0.848	0.019936196
0.849	0.019252618
0.85	0.018587484
0.851	0.017940445
0.852	0.017311154
0.853	0.01669927
0.854	0.016104453
0.855	0.015526366
0.856	0.014964678
0.857	0.014419057
0.858	0.013889179
0.859	0.01337472
0.86	0.01287536
0.861	0.012390783
0.862	0.011920678
0.863	0.011464733
0.864	0.011022644
0.865	0.010594108
0.866	0.010178827
0.867	0.009776504
0.868	0.009386849
0.869	0.009009574
0.87	0.008644393
0.871	0.008291025
0.872	0.007949194
0.873	0.007618626
0.874	0.00729905
0.875	0.006990201
0.876	0.006691814
0.877	0.006403632
0.878	0.006125399
0.879	0.005856863
0.88	0.005597776
0.881	0.005347894
0.882	0.005106975
0.883	0.004874784
0.884	0.004651086
0.885	0.004435652
0.886	0.004228257
0.887	0.004028677
0.888	0.003836696
0.889	0.003652097
0.89	0.003474669
0.891	0.003304206
0.892	0.003140504
0.893	0.002983361
0.894	0.002832583
0.895	0.002687975
0.896	0.00254935
0.897	0.00241652
0.898	0.002289305
0.899	0.002167526
0.9	0.002051008
0.901	0.00193958
0.902	0.001833074
0.903	0.001731326
0.904	0.001634175
0.905	0.001541464
0.906	0.001453039
0.907	0.00136875
0.908	0.00128845
0.909	0.001211996
0.91	0.001139247
0.911	0.001070067
0.912	0.001004321
0.913	0.000941881
0.914	0.000882618
0.915	0.000826409
0.916	0.000773134
0.917	0.000722675
0.918	0.000674918
0.919	0.000629752
0.92	0.000587068
0.921	0.000546762
0.922	0.000508732
0.923	0.000472877
0.924	0.000439103
0.925	0.000407316
0.926	0.000377426
0.927	0.000349344
0.928	0.000322986
0.929	0.000298271
0.93	0.000275117
0.931	0.000253449
0.932	0.000233192
0.933	0.000214276
0.934	0.000196629
0.935	0.000180187
0.936	0.000164885
0.937	0.00015066
0.938	0.000137454
0.939	0.00012521
0.94	0.000113872
0.941	0.000103387
0.942	9.37063302e-05
0.943	8.47799708e-05
0.944	7.65620400e-05
0.945	6.90082046e-05
0.946	6.20761054e-05
0.947	5.57253097e-05
0.948	4.99172635e-05
0.949	4.46152431e-05
0.95	3.97843076e-05
0.951	3.53912503e-05
0.952	3.14045500e-05
0.953	2.77943235e-05
0.954	2.45322762e-05
0.955	2.15916547e-05
0.956	1.89471976e-05
0.957	1.65750879e-05
0.958	1.44529046e-05
0.959	1.25595745e-05
0.96	1.08753248e-05
0.961	9.38163539e-06
0.962	8.06119126e-06
0.963	6.89783578e-06
0.964	5.87652378e-06
0.965	4.98327526e-06
0.966	4.20512941e-06
0.967	3.53009906e-06
0.968	2.94712568e-06
0.969	2.44603478e-06
0.97	2.01749200e-06
0.971	1.65295969e-06
0.972	1.34465417e-06
0.973	1.08550368e-06
0.974	8.69107050e-07
0.975	6.89693086e-07
0.976	5.42080866e-07
0.977	4.21640800e-07
0.978	3.24256627e-07
0.979	2.46288363e-07
0.98	1.84536226e-07
0.981	1.36205609e-07
0.982	9.88731429e-08
0.983	7.04538868e-08
0.984	4.91697100e-08
0.985	3.35189058e-08
0.986	2.22470910e-08
0.987	1.43194415e-08
0.988	8.89431717e-09
0.989	5.29832549e-09
0.99	3.00288109e-09
0.991	1.60231180e-09
0.992	7.93567673e-10
0.993	3.57587716e-10
0.994	1.42380461e-10
0.995	4.78751014e-11
0.996	1.26006996e-11
0.997	2.25167403e-12
0.998	1.98472114e-13
0.999	3.11357485e-15
1	0

}{\hocsdatafouroften}


==> full_of_hope.tex <==
\input{preamble}

\title{Bounding Undefined Probabilities Through Meta Reasoning}
\author{Justus Isaiah Hibshman}
\date{April 2021}

\begin{document}

\maketitle

\begin{abstract}
Probability functions are often considered as numeric measures of confidence. We analyze how numeric confidences can operate when someone chooses to leave probabilities (confidences) undefined rather than picking prior distributions. We develop inequalities that allow a user to perform many Bayesian calculations without needing to parametrize models with prior distributions. Amongst other things, our results enable a new version of single hypothesis testing.
\end{abstract}

\section{Introduction}

% TODO: Search in LaTeX for "P(" that should be "P_<something>("

You know that $P$ is a probability function on a random variable $X$, where $X$ can take on one of $n$ possible values. Thus you know that $P$ is always non-negative and sums to 1. That is all you know about $P$. Or is it? Can you conclude anything else meaningful about $P(X)$ from the above information alone? We argue that if $P$ is interpreted as a measure of confidence, then yes, there is much more of interest you can conclude. In order to illustrate the meaning and significance of our results, we focus on our results' implications for single hypothesis testing.

As is probably well-known, people mean different things by the term ``probability.'' Some use the idea to refer to a frequency of occurrence. Sometimes this frequency is considered to be inherent to each occurrence of the underlying phenomenon (e.g. some interpretations of the collapse of quantum wave functions). Other times, this frequency is considered to be a more general pattern about trends across repeated occurrences (e.g. repeatedly rolling a die).

Other people understand probabilities in terms of a measure of a person's confidence that an event would/will/did happen or that something is true/false. For example, Cheeseman argues in favor of this interpretation \cite{cheeseman1985defense}. In this paper we consider probabilities in this light. In this paper we will use ``probability function'' and ``confidence function'' interchangeably. We note that viewing a probability as a confidence is not inherently contradictory with believing that some things operate according to frequencies; in fact, a person thinking of probabilities as confidences will usually believe that their confidence should correspond to that frequency when a frequency is a proper way to understand the underlying process.

Often, a person wishing to employ mathematical notions of confidence does not have clearly defined confidences (i.e. probabilities) for certain events. Single (``null'') hypothesis testing is a classic example of this phenomenon. In single hypothesis testing, an experimenter will define a ``null'' hypothesis and obtain an experimental result; then the experimenter wishes to determine whether the experimental result counts as evidence against the null hypothesis. However, to truly determine whether the result is evidence against the null, the experimenter needs to consider the null hypothesis vis-a-vis the alternative hypothesis (i.e. the hypothesis that the null hypothesis is false). Richard Royall argues cogently for this requirement \cite{royall1997statistical}. Unfortunately, while the null hypothesis (usually) defines a probability function over the experimental result space, the alternative hypothesis is usually too vague to actually define probabilities about experimental results. After all, what is, ``The probability of flipping a coin 20 times and obtaining 7 heads given that the coin is \emph{not} fair?'' Such a question has no answer, but \emph{some kind of answer} is needed in order to meaningfully compare the null hypothesis to the alternative.

Some people try to simply avoid or sidestep situations where probability functions are undefined. In the realm of single hypothesis testing, p-values are such an attempt, but this causes p-values to fail to be a valid measure of evidence. To see excellent exposition on why p-values fail to be a proper formulation of statistical evidence, consider reading work by Richard Royall \cite{royall1997statistical} or Wagenmakers \cite{wagenmakers2007practical}.

Rather than attempting to sidestep situations where probability functions (i.e. confidences) are undefined, others have suggested using certain ``natural'' confidences in the form of ``uninformative'' priors. For example, the uniform prior and the Jeffereys prior are considered to be potentially good options for ``uninformative'' priors \cite{jeffreys1998theory, price2002uninformative}. Unfortunately, the term ``uninformative prior'' is a bit of a misnomer, as use of an uninformative prior can seriously bias one's analysis. One can read about some problems with the use of uninformative priors in Lemoine \cite{lemoine2019moving}. We find the idea of uninformative priors to be somewhat suspect.

Rather than trying to sidestep undefined probabilities, and rather than simply choosing to use an ``uninformative'' prior, we analyze what one can mathematically derive simply by asserting that you have a confidence function. That's it; no assumptions or definition of the confidence function required. In particular, we find that in lieu of defined confidence functions, we can derive useful \emph{bounds} on one's confidence about particular events. In the context of single hypothesis testing, our results allow someone to derive a lower bound on an experimental result's strength as evidence against the null, \emph{all without assuming any priors to parametrize the alternative hypothesis}.

To our knowledge, noone else has analyzed probability functions in this fashion. Perhaps the closest project we are aware of is Walley's work on ``imprecise probabilities,'' which basically involves using an upper and lower bound(s) on a probability rather than a single value \cite{walley1991statistical, walley2000towards}. However, Walley does not offer ways to derive bounds like we do. Rather, he offers ways to use and combine bounds one already has. \textbf{TODO: Fact check that. Get his book.}

We first expound on what it means to interpret probabilities as confidences (or confidences as probabilities) in Section~\ref{sec:essential_concepts}. While doing so, we introduce new mathematical notation to account for phenomena which only occurs when confidences are allowed to be undefined; these concepts and notation are crucial for our results to make sense. Then we introduce and derive our core results in Sections~\ref{sec:idea_warmup}, through \ref{sec:hypothesis_testing_math}. Throughout those sections, we provide a concrete way of understanding the meaning of our results via the fictional ``Monty Hallways Gameshow'' (story in green boxes). Next, in Section~\ref{sec:single_hypothesis_testing} we discuss the application to single hypothesis testing. Lastly, in Section~\ref{sec:objections} we respond to some objections.

\section{Essential Concepts}\label{sec:essential_concepts}

In this section we briefly cover the conceptual ground needed to understand and apply our mathematical results. In the process, we consider what it means for a probability function to be undefined, what it means to interpret confidences as probabilities, and how conditional confidences become more complex when probability functions are allowed to be undefined.

\subsection{Being Undefined}

Many expressions in math are undefined. For instance, the fraction ``$\left(\frac{1}{0}\right)$'' is undefined; the expression ``$\left(\lim_{x \rightarrow 0} \frac{1}{x}\right)$'' is not. There are multiple ways for something to be undefined. In the case of $\frac{1}{0}$, the expression is simply outside the scope of what the division operation is defined on. Consider the following cases:

\begin{enumerate}
    \item If we write, ``Let $x$ be a variable.'' then the value of $x$ is undefined, $x$ could be anything, $2, 5, \{\{1\}, \{2, 3\}, \emptyset \}, \langle 0, 3, 7 \rangle$, etc.
    \item If we write, ``Let $x \in \mathbbm{R}$ be a variable.'' then $x$ is still undefined, but we know a bit more about $x$; we know that $x$ could be $\pi, 1, $ or $-365$ but $x$ cannot be $\{2, 4\}$.
    \item If we write, ``Let $x \in \mathbbm{R}$ where $0 \leq x \leq 100$.'' then once again $x$ is undefined, but we know even more about $x$.
    \item Yet again, if we write, ``Let $x \in \{1, 2, 3, 4, 5\}$.'' then the value of $x$ is undefined, but our possible values for $x$ are very limited.
\end{enumerate}

We could provide many, many more examples, but the basic idea should be clear. Importantly, there are many cases where the value of something can be undefined, yet we still have \emph{some} knowledge about it and can use that knowledge to derive other results. For instance, if we write, ``Let $x \in \{1, 2, 3\}$. Let $y = 4$.'' then we can conclude that $x < y$ even though the value of $x$ is undefined.

In the case of probabilities we can do the same thing. For example, if we are given, ``$(\Omega, \mathcal{F}, P)$ is a probability space where $\Omega = \{0, 1, 2\}$ and $\mathcal{F} = \{\emptyset, \{1\}, \{0, 2\}, \{0, 1, 2\}\}$.'' then we can conclude that $P$ is a function, and while the value of $P(\{1\})$ is undefined, we still know that $0 = P(\emptyset) \leq P(\{1\}) \leq P(\{0, 1, 2\} = 1$. Similarly, if we are given the additional information that $\cup_{E \in \mathcal{F}} \{P(E)\} = \{0, 0.3, 0.7, 1\}$, then while the value $P(\{1\})$ is still undefined, we know that $P(\{1\}) \in \{0, 0.3, 0.7, 1\}$.

In this paper, we explore how simply knowing that some function $f$ is a probability measure (or knowing some further details about that function) can allow us to reach useful conclusions even when $f$ is undefined.

\subsection{Probabilities as Confidences}

There are many different ways to interpret the idea of a ``probability.'' As we have already discussed, in this paper we consider probabilities as measures of confidence. Once we begin to work with probability functions which are mathematically undefined in certain ways, we find that two things which are usually treated as conceptually equivalent can sometimes come apart: ``$A$ and $B$ \emph{occur} independently.'' and ``Upon observing $B$, your confidence about $A$ does not change.'' Understanding what we mean by these things is crucial to working with undefined probability functions.

When a probability function $P$ from a probability space ($\Omega$, $\mathcal{F}$, $P$) is interpreted as representing confidences, $P$ effectively represents confidences and their relationships \textit{at a single epistemic state}. Confidence about an event $E \in \mathcal{F}$ is expressed as $P(E)$. Relationships between events $A, B \in \mathcal{F}$ are expressed via conditional probabilities, $P(A | B)$, $P(B | A)$. A conditional probability $P(A | B)$ can be understood in two ways, which we explore in the following section.

\subsection{Anticipatory Conditionals and Confidence Update Conditionals}

When probabilities represent confidences, we can think of conditional confidences in the following two ways:

\begin{itemize}
    \item \textbf{The Anticipatory Conditional: } Here $P(A | B)$ is understood to mean a confidence about what will/has happen(ed) if something else will/has happen(ed). That is, $P(A | B) = p$ means, ``I am $p$ confident that if $B$ will/has occur(ed), then $A$ will/has occur(ed).''
    \item \textbf{The Confidence Update Conditional: } Here $P(A | B)$ is understood to mean what a confidence will change to upon being given new information. That is, $P(A | B) = p$ means, ``In my current epistemic state I am $P(A)$ confident that $A$ will/has occur(ed). However, if I observe event $B$, then my confidence that $A$ will/has occur(ed) changes to $p$.''
\end{itemize}

We believe these two conceptual understandings to be mathematically equivalent. Both can be helpful ways of understanding conditionals.

The standard probability axioms (the Kolmogorov axioms) do not explicitly define conditional probabilities. A conditional probability $P(A | B)$ is usually defined to be shorthand for the quantity $\frac{P(A \cap B)}{P(B)}$. When probability functions are fully defined, this mathematical definition perfectly corresponds to the concepts of a conditional probability we discussed. \emph{However, } when you allow probability functions to be undefined in certain ways, this mathematical definition and the concepts begin to come apart. At a high level, this coming-apart occurs because when a probability function $P$ is undefined in certain ways, observing an event $B$ allows you to think in a ``meta'' way about ``what your confidence is that $P(B)$ was a specific confidence.''

We present a new mathematical definition of conditional probabilities - a definition which equals the standard definition when probability functions are fully defined, but which behaves in a more conceptually proper way when probability functions are undefined.

\subsection{Formalizing Undefined Probability Functions}

In this section, we present a way to model probability functions where those probability functions can be undefined.

Let $(\Omega, \mathcal{F}, P)$ be a probability space as defined by the standard Kolmogorov axioms.

We model the extent to which $P$ is defined via the set $\mathcal{P}_P$ which contains all the possible definitions of $P$. That is,

$$\mathcal{P}_P = \{P'\ |\ \text{``}P' \neq P\text{''} \text{ is not defined to be true}\}$$

Thus, for example, if we defined $P$ to be a normal distribution but not did not specify \emph{which} normal distribution, then $\mathcal{P}_P$ would be the set of all normal distributions.

We believe this definition to be extremely general. However, it can be generalized even further by considering confidences about confidences.

\subsubsection{Undefined Probabilities over Undefined Probabilities}

We began with the set $\mathcal{P}_P$ of possible probability functions over $\mathcal{F}$; we can also consider the set $\mathcal{P}_P^2$ of probability functions over $\mathcal{P}_P$ itself. More broadly, we can define sets $\mathcal{P}_P^i$ of these ``meta'' probabilities over the previous set $\mathcal{P}_P^{i - 1}$.

We note however that any probability function in $P^2 \in \mathcal{P}_P^2$ effectively corresponds to a probability function over $\mathcal{F}$, where for any event $E \in \mathcal{F}$,

$$P^2(E) = \sum_{P^1 \in \mathcal{P}_P} P^1(E) P^2(P^1)$$

Thus, any collection of meta probability functions $\mathcal{P}_P, \mathcal{P}_P^2, \mathcal{P}_P^3, ..., \mathcal{P}_P^n$ corresponds to some other set $\mathcal{P}_P'$ of probability functions over $\mathcal{F}$. We are unsure as of writing this paper whether generalizing to $\mathcal{P}_P^i$ offers any advantage over sticking with a single $\mathcal{P}_P$.

\textbf{CHECK BACK}

\subsection{Defining Conditionals}

In some senses, this section contains our main contribution, and the rest of the paper is an unfolding of this contribution. In this section we redefine conditional probabilities to something which makes sense \emph{both} when probability functions are defined and when they are undefined. Our new definition always equals the standard definition when probability functions are defined, but it is more complete when they are undefined.

Typically, a conditional probability for events $A$ and $B$ is defined to be $P(A | B) = \frac{P(A \cap B)}{P(B)}$. However, we define conditionals as:

\begin{equation}\label{eqn:conditional_def}
P(A | B) = \frac{P(A \cap B)}{P(B)} \frac{P(\langle B \rangle)}{P(B)}
\end{equation}

Where $\langle B \rangle$ denotes something we call ``the hindsight event of $B$'' and $P(\langle B \rangle)$ is ``the hindsight probability of $B$.'' The hindsight event is not, strictly speaking, an event. We define hindsight ``probabilities'' in the next section.

\subsection{Defining Hindsight}

Let $(\Omega, \mathcal{F}, P)$ be a probability space where $P$ is defined to be a member of some set $\mathcal{P}$ of probability measures over $\Sigma, \mathcal{F}$. Note that if $P$ is fully defined then $|\mathcal{P}| = 1$.

Let $m : 2^\mathcal{P} \times [0, 1] \rightarrow \mathbbm{N}_0$ be a function defined as

$$m(S, q) = \min_{P' \in S} \left\{ \left| \{ \omega\ |\ \omega \in \Omega, P'(\{\omega\}) = q\} \right| \right\}$$

That is, $m(S, q) = k$ means that if we restrict the values $P$ could have to some subset $S \subseteq \mathcal{P}$ (i.e. $P' \in S$ and $S \in 2^\mathcal{P}$), there are $k$ or more elementary events where $P'$ says those events are each $q$-likely; in particular, $k$ is the largest of such values where this holds true. Now we define a set of probability values which \textit{always} appear in a subset $S \subseteq \mathcal{P}$ (if any) to be:

$$A: 2^\mathcal{P} \rightarrow \mathcal{P}([0, 1]);\ A(S) = \{q\ |\ m(S, q) > 0\}$$

Similarly, we define all the probabilities potentially associated with an event $\omega \in \Omega$ to be:

$$C: 2^\mathcal{P} \times \Omega \rightarrow \mathcal{P}([0, 1]);\ C(S, \omega) = \{q\ |\ \exists P' \in \mathcal{P}.\ P'(\{\omega\}) = q\}$$

Next, define $l : 2^\mathcal{P} \times \Omega \rightarrow [0, 1]$ and $u : 2^\mathcal{P} \times \Omega \rightarrow [0, 1]$ as:

\begin{equation*}
l(S, \omega) =
\begin{cases}
\frac{\sum_{q \in C(S, \omega)} q^2 \cdot m(S, q)}{\sum_{p \in C(S, \omega)} p \cdot m(S, p)},& \text{ if } C(S, \omega) \subseteq A(S) \\
0,& \text{ otherwise}
\end{cases}
\end{equation*}

\begin{equation*}
u(S, \omega) =
\begin{cases}
\frac{\sum_{q \in C(S, \omega)} q^2 \cdot m(S, q)}{\sum_{p \in C(S, \omega)} p \cdot m(S, p)},& \text{ if } C(S, \omega) \subseteq A(S) \\
1,& \text{ otherwise}
\end{cases}
\end{equation*}

Let $\mathbbm{P}_\mathcal{P}$ be the set of all partitions of $\mathcal{P}$. Then we define the functions $L: \Omega \rightarrow [0, 1]$ and $U: \Omega \rightarrow [0, 1]$ as:

$$L(\omega) = \max_{H \in \mathbbm{P}_\mathcal{P}} \left\{ \min_{S \in H} \left\{ l(S, \omega) \right\} \right\}$$

$$U(\omega) = \min_{H \in \mathbbm{P}_\mathcal{P}} \left\{ \max_{S \in H} \left\{ u(S, \omega) \right\} \right\}$$

Last but not least, $\mathcal{L}: \mathcal{F} \rightarrow [0, 1]$ and $\mathcal{U}: \mathcal{F} \rightarrow [0, 1]$:

\begin{equation*}
\mathcal{L}(E) = \frac{1}{P(E)} \cdot \sum_{\omega \in E} P(\{\omega\}) \left( L(\omega) + \sum_{\omega' \in E \setminus \{\omega\}} \frac{P(\{\omega'\}) (1 - P(\{\omega'\})) }{1 - L(\omega')} \right)
\end{equation*}

\begin{equation*}
\mathcal{U}(E) = \frac{1}{P(E)} \cdot \sum_{\omega \in E} P(\{\omega\}) \left( U(\omega) + \sum_{\omega' \in E \setminus \{\omega\}} \frac{P(\{\omega'\}) (1 - P(\{\omega'\}))}{1 - U(\omega')} \right)
\end{equation*}

With all this in place, we finally get that:

\begin{equation}\label{eqn:hindsight_def}
\mathcal{L}(E) \leq P(\langle E \rangle) \leq \mathcal{U}(E)
\end{equation}

%\begin{equation}\label{eqn:hindsight_finite}
%\forall E \in \mathcal{F}.\ P(\langle \rangle | E) = \sum_{p \in \{q\ |\ \exists \omega \in \Omega.\ P(\{\omega\}) = q\}} p P(\boxed{P} = p | E)
%\end{equation}

%\begin{equation}\label{eqn:hindsight_finite}
%\forall E \in \mathcal{F}.\ P(\langle \rangle | E) = \sum_{\omega \in \Omega} P(\{\omega\}) P(\boxed{P} = P(\{\omega\}) | E)
%\end{equation}

%\begin{equation}\label{eqn:hindsight_finite}
%\forall E \in \mathcal{F}.\ P(\langle \rangle | E) = \sum_{\omega \in \Omega} P(\{\omega\}) \frac{P\left(\boxed{P} = P(\{\omega\})\ \cap\ E\right)}{P(E)}
%\end{equation}

%And last but not least we define conditional probabilities for $\boxed{P}$ as follows:

%\begin{equation}
%\forall E \in \mathcal{F}.\ P(\boxed{P} = p | E) = 
%\begin{cases}
%\frac{P\left(\boxed{P} = p\ \cap\ E\right)}{P(E)},& \text{if this quantity is defined} \\
%p,& \text{otherwise}
%\end{cases}
%\end{equation}

\textbf{TODO: Define hindsight for continuous cases.}

\subsection{Independence}

Independence is often expressed in terms of conditional probabilities. That is, given two events $A$ and $B$, independence is often defined as $P(A | B) = P(A)$. Independence is also commonly defined as $P(A \cap B) = P(A) P(B)$. Normally these are mathematically equivalent. With our definitions, these two remain equivalent \emph{until} $P$ becomes undefined in which case they can come apart. Independence is conceptually meant to convey that one event's chance of occurring is not ``dependant'' on the other event having occurred.

%\begin{equation}
%P(A | B) = \sum_{something} something\ else
%\end{equation}

\begin{figure}[b]
% The \phantomcaption allows for an invisible caption.
% \phantomcaption{}
\begin{tcolorbox}[colback=green!10!white,colframe=green!50!black,before upper={\parindent15pt},title=\textbf{The Monty Hallways Gameshow - Intro}]

Welcome! You are a contestant on the famous Monty Hallways Gameshow, a gameshow for statisticians to show their prowess. Today's episode is sponsored by the local dairies' ``Got half-and-half?'' campaign and the state's ``50-50 Entertainment-Learning'' initiative. If you pass all the challenges, you will win the prize collection of premium half-and-half products. Do you have what it takes?

\ 

(These story segments serve to illustrate the concepts presented in the paper.)
\end{tcolorbox}
\end{figure}

\section{Undefined Pairing Between Result Space and Probabilities}\label{sec:idea_warmup}

Consider sampling a distribution twice (independently), where the distribution is defined over a finite set of values $\mathcal{X}$. The random variable $X$ represents the first sampled value and the random variable $X'$ represents the second. The sampling of $X$ and $X'$ is performed according to the same distribution over $\mathcal{X}$. Let $P_\mathcal{X}$ be the probability function representing our confidences about the sampling process. In this case, $P_\mathcal{X}$ (i.e. our confidences about what values $X$ and $X'$ will take) will be undefined in the following manner:

\begin{itemize}
\item We know (define) the following about $P_\mathcal{X}$: We are given the multiset $M_{P_\mathcal{X}} = (S_{P_\mathcal{X}}, m_{P_\mathcal{X}})$, where $S$ is the support set defined to be $S = \{p\ |\ \exists x \in \mathcal{X}.\  P_\mathcal{X}(X = x) = p\}$ and where $m$ is the multiplicity function $m: S \rightarrow \mathbbm{N}$. The multiplicity function $m$ states how many different $x \in \mathcal{X}$ have a probability of $p$ for $p \in S$.

\item We are ignorant (leave $P_\mathcal{X}$ undefined) as follows: For any given $x \in \mathcal{X}$, we do not know $P_\mathcal{X}(X = x)$. In other words, we know the probabilities, but we do not know the bijection between those probabilities and the values $X$ (or $X'$ can take. This bijection exists implicitly in the very fact that $P_\mathcal{X}$ is defined to be a probability function.
\end{itemize}

Given a confidence $P_\mathcal{X}$ which is undefined in this way, if we observe the event $X = x_0$, we can then conclude the following about the chances that $x_0$ will be sampled again (i.e. our confidence that $X' = x_0$):

\begin{equation}\label{eqn:no_pairings}
P_\mathcal{X}(X' = x_0 | X = x_0) = \sum_{q \in M_{P_\mathcal{X}}} q^2
\end{equation}

We explain the meaning of this result and its derivation in the rest of this section. To get a more concrete understanding of what this result means, we recommend considering it in terms of the situation presented in the first challenge of The Monty Hallways Gameshow, where $X$ represents the first dairy product brought forth, $X'$ represents the second, the doors display the probabilities (i.e. $M_{P_\mathcal{X}}$) but the bijection between the dairy products and the doors is unknown. You observe a particular dairy product, Leonard's 2\% Milk, which corresponds to observing $X = x_0$. You are then asked about your confidence that if a door is opened again, it will bring forth Leonard's Milk again ($X' = x_0$).

\begin{figure}[t]
% The \phantomcaption allows for an invisible caption.
% \phantomcaption{}\label{fig:first_story_task}
\begin{tcolorbox}[colback=green!10!white,colframe=green!50!black,before upper={\parindent15pt},title=\textbf{The Monty Hallways Gameshow - First Challenge}]
For your first challenge, you are brought into a long hallway. On each door is a number. The gameshow host tells you these numbers form a probability distribution over the doors. You are told that each door is associated with a unique dairy product. A product will be sampled according to the distribution. You are blindfolded while this sampling occurs. The sampling is surprisingly quiet. Perhaps it is the velvety carpet. Upon having your blindfold removed, you see a gallon of Leonard's 2\% Milk on the table in front of you.

\

The gameshow host then asks you, ``What is your confidence that if we repeat this process, you would see another gallon of Leonard's 2\% Milk?'' You are given a pencil and paper and proceed to write down the numbers on the doors. After some thinking, you come up with an answer. (See Section~\ref{sec:idea_warmup} for mathematical details.) ``Well done! A true theorist!'' your host exclaims. ``On to the next hallway...''
\end{tcolorbox}
\end{figure}

In order to understand what we know about $P_\mathcal{X}$, we consider how confidences evolve as new information appears. Confidences change over time as new information becomes available. A particular confidence function (i.e. probability function) expresses confidences at a fixed time; a confidence function also expresses rules for updating one's confidences upon observing an event. The updated confidences (or a posteriori confidences) are written as conditional probabilities. For example, consider a probability function $P$, events $A$ and $B$, and Bayes' rule:

$$P(A | B) = \frac{P(B | A)P(A)}{P(B)}$$

The probability function $P$ gives us both a present confidence $P(A)$ that $A$ will/has occur(ed) \emph{as well as} giving us a new confidence value $P(A | B)$ that $A$ will/has occur(ed) upon observation of the event $B$.

Now, back to our situation with $X$, $X'$, and $P_\mathcal{X}$: Imagine that you observe the event $X = x_0$. This is analogous to observing the gallon of Leonard's 2\% Milk in the first challenge of our running example. \emph{Before} you observed $X = x_0$, you could speak of the probability that $X = x_0$ in terms of your confidence about whether that event would happen. \emph{After} you observe $X = x_0$, there is a sense in which your confidence about $X = x_0$ becomes 1; you no longer have any uncertainty about whether $X = x_0$. This is expressed in mathematical notation as the conditional probability $P_\mathcal{X}(X = x_0 | X = x_0) = 1$. However, you can also still think of what your confidence that $X = x_0$ \emph{was} before you observed it; this is expressed as $P_\mathcal{X}(X = x_0)$.

Consider our confidences about $X'$. We know that $X$ and $X'$ follow the same distribution: $\forall x \in \mathcal{X}.\ P_\mathcal{X}(X = x) = P_\mathcal{X}(X' = x)$. Remember that $P_\mathcal{X}(X' = x_0)$ is, in a sense, undefined; we are given the collection of relevant probabilities via multiset $M_{P_\mathcal{X}} = (S_{P_\mathcal{X}}, m_{P_\mathcal{X}}$, but we do not know the bijection between the probabilities in $M_{P_\mathcal{X}}$ and the values in $P_\mathcal{X}$. Since we know $M_{P_\mathcal{X}}$, we know that the value $x_0$ was sampled with one of the probabilities in $M_{P_\mathcal{X}}$. This means that we can consider the chances (i.e. our confidence) that the sampled value $x_0$ was sampled with a given probability $p \in S_{P_\mathcal{X}}$. That is, for any $p \in S_{P_\mathcal{X}}$, we can be $p\cdot m_{P_\mathcal{X}}(p)$ confident that the event $X = x_0$ had a chance $p$ of occurring. Put mathematically:

$$\forall p \in S_{P_\mathcal{X}}.\ P_\mathcal{X}\left(P_\mathcal{X}(X = x_0) = p | X = x_0\right) = p \cdot m_{P_\mathcal{X}}(p)$$

In terms of The Monty Hallways Gameshow, the event ``$P_\mathcal{X}(X = x_0) = p$'' is the event that a door was opened which had probability $p$ written on the door. Obtaining the equation above corresponds to counting all the doors with probability $p$ written on them ($m_{P_\mathcal{X}}(p)$ doors total) and then computing the chances of having opened one of those doors ($p \cdot m_{P_\mathcal{X}}(p)$).

Similarly, we can consider the chances that $X'$ will equal $x_0$ as conditioned on the event that $P_\mathcal{X}(X = x_0) = p$. Since $P_\mathcal{X}(X' = x_0) = P_\mathcal{X}(X = x_0)$, this just becomes:

$$P_\mathcal{X}(X' = x_0 | P_\mathcal{X}(X = x_0) = p) = p$$

Putting it all together, we can derive the following confidence:

\begin{align*}
P_\mathcal{X}(X' = x_0 | X = x_0) &= \sum_{p \in S_{P_\mathcal{X}}} P_\mathcal{X}(X' = x_0 | X = x_0, P_\mathcal{X}(X = x_0) = p) P_\mathcal{X}(P_\mathcal{X}(X = x_0) = p | X = x_0) \\
 &= \sum_{p \in S_{P_\mathcal{X}}} P_\mathcal{X}(X' = x_0 | X = x_0, P_\mathcal{X}(X = x_0) = p) \cdot p \cdot m_{P_\mathcal{X}}(p) \\
 &= \sum_{p \in S_{P_\mathcal{X}}} p^2 \cdot m_{P_\mathcal{X}}(p) \\
 &= \sum_{q \in M_{P_\mathcal{X}}} q^2
\end{align*}

Thus, \emph{even though} we do not know which probabilities in $M_{P_\mathcal{X}}$ correspond to which values in $\mathcal{X}$, after observing a value $x_0$ be sampled we arrive at a particular confidence that $x_0$ will be sampled again. The sheer fact that $x_0$ had to have been sampled via \emph{one of} the probabilities in $M_{P_\mathcal{X}}$ gives us a confidence that $x_0$ will be sampled again.

Remember that the sampling of $X$ and $X'$ occur independently. Statisticians typically work with fully defined probability functions. When probability functions are fully defined, receiving information about the state of one random variable does not provide any information about another independent random variable. However, in this case, seeing the event $X = x_0$ moved our confidence in the event $X' = x_0$ from being undefined to being the exact value $\sum_{q \in M_{P_\mathcal{X}}} q^2$. That is, $P_\mathcal{X}(X' = x_0 | X = x_0) \neq P_\mathcal{X}(X' = x_0)$. This \emph{should not} be taken as saying $X$ and $X'$ are not independent. Rather, in this case the conditioning on an event (the event $X = x_0$) does something conditioning normally does not do; here the conditioning gives more information about $P_\mathcal{X}$ itself. This distinction is crucial to a proper interpretation of these results.

This result serves as the conceptual foundation for results when even less is known about $P_\mathcal{X}$. That is, the concepts in this section allow us to say things about our confidence when our confidence is even less defined than $P_\mathcal{X}$.

\section{Completely Undefined Probabilities}\label{sec:completely_undefined_probs}

We just explored in Section~\ref{sec:idea_warmup} how in \emph{some cases} we can define a probability even when certain aspects of the probability distribution are undefined. Here we extend those results to a case where \emph{nothing} about the probability function is defined beyond the fact that it is a probability function.

\begin{figure}
% The \phantomcaption allows for an invisible caption.
% \phantomcaption{}\label{fig:second_story_task}
\begin{tcolorbox}[colback=green!10!white,colframe=green!50!black,before upper={\parindent15pt},title=\textbf{The Monty Hallways Gameshow - Second Challenge}]
For your next challenge, you are once again brought into a long hallway. This time the doors are completely blank. Your host assures you that each door corresponds to a unique dairy product and that there is a probability distribution over the doors; the probabilities are hidden. The collection of relevant dairy products is pictured on one of the walls. Before anything occurs, the host points at the image of Dillard's Half-and-Half, asking, ``What is your confidence you'll see Dillard's come from a door in this hallway?''

You reply, ``Well, my confidence is rather undefined at the moment.''

``Of course! Of course!'' says your energetic host, ``How about a minimum confidence?''

``A minimum confidence? Is that like a lower bound on my confidence?''

``Indeed.''

``I'm afraid I cannot lower-bound my confidence above zero.'' you say.

``Well done! You're properly cautious. Now for the big question.''

You are temporarily blindfolded; when un-blindfolded, you see a box of Harriet's Best cream cheese. The gameshow host says, ``Tell me, what is your minimum confidence that if this process were to be repeated, the product would be Harriet's Best cream cheese again?'' Your brow furrows. You spend a while in thought and then come up with an answer. ``Wonderful!'' exclaims the host, ``Only two challenges remain...''

\ 

(The math behind this case is presented in Section~\ref{sec:completely_undefined_probs}.)
\end{tcolorbox}
\end{figure}

Our setup mirrors the situation in Section~\ref{sec:idea_warmup}. This time we sample twice independently from a finite set $\mathcal{Y}$. The random variables $Y$ and $Y'$ represent the first and second samples respectively. The sampling of $Y$ and $Y'$ is performed according to the same distribution over $\mathcal{Y}$. We represent our confidence about which values will be sampled via the confidence function $P_\mathcal{Y}$. In this case, we leave our confidence function \emph{completely} undefined. We are not even given a multiset similar to $M_{P_\mathcal{X}}$ from Section~\ref{sec:idea_warmup}. We observe the event $Y = y_0$ for some $y_0 \in \mathcal{Y}$. In this case we do not have enough information to get an exact confidence that $y_0$ will be sampled again. However, we \emph{can} consider a worst case application of Equation~\ref{eqn:no_pairings} and use that worst case to lower-bound our confidence that $y_0$ will be sampled again as follows:

\begin{equation}\label{eqn:total_ignorance_bound}
P_\mathcal{Y}(Y' = y_0 | Y = y_0) \geq \frac{1}{|\mathcal{Y}|}
\end{equation}

We explain the meaning and derivation of this result in the rest of this section. For a more concrete version of this problem, check out the second challenge of The Monty Hallways Gameshow story. In the gameshow story, the event $Y = y_0$ corresponds to seeing Harriet's Best cream cheese, and the event $Y' = y_0$ represents seeing the cream cheese again. In the story, you know that there is \emph{some} probability distribution governing the sampling process, but you know nothing about that distribution.

Key to this result is the shift from having an undefined or exact confidence to having a lower bound on a confidence. Conceptually, a lower bound of $\alpha$ on a confidence can be understood in several ways. We list two:

\begin{enumerate}
    \item If your confidence is a measure of your belief about a rate of occurrence, then the lower bound of $\alpha$ corresponds to thinking the event is at least $\alpha$-likely to occur.
    \item If your confidence is solely a measure of how much you believe some event $E$ will/has occur(ed) with no reference to an underlying probabilistic mechanism behind $E$, then the meaning of the lower bound is less easy to define. When confidences are understood as ``amounts of belief,'' then a specific numeric confidence corresponds to a specific amount of belief and a completely undefined confidence corresponds to some kind of state of total agnosticism. In this light, a confidence lower bound would correspond to something like an agnosticism which is \emph{restricted} to a particular range of amounts of belief.
\end{enumerate}

We do not claim this is an exhaustive list of the ways to interpret lower bounds on confidences. Our goal here is simply to ballpark ways of interpreting the mathematical results such that the math meaningfully corresponds to the realities probabilities-as-confidences are meant to model.

Given these notions of a bound on a confidence, how did we obtain the bound in Equation~\ref{eqn:total_ignorance_bound}? We did so via an extension of the results contained in Equation~\ref{eqn:no_pairings}. For Equation~\ref{eqn:no_pairings}, we were given the multiset of probabilities associated with the sampling process. In this context, we no longer have that multiset. However, we can consider all possible multisets of probabilities and see if our confidence would always be at least certain amount no matter which multiset was applied. If so, then we can conclude that even without the knowledge/confidence contained in $M_{P_\mathcal{X}}$ from Section~\ref{sec:idea_warmup}, we know that \emph{whatever} that knowledge/confidence is, if we had it and our confidence would be at least $\alpha$, then our confidence can be at least $\alpha$. This can be formalized as follows:

Like $M_{P_\mathcal{X}}$ from Section~\ref{sec:idea_warmup}, let $M_{P_\mathcal{Y}} = (S_{P_\mathcal{Y}}, m_{P_\mathcal{Y}})$ be the multiset of probabilities (our confidences) that values of $\mathcal{Y}$ will be sampled. That is, $S_{P_\mathcal{Y}} = \{p\ |\ \exists y \in \mathcal{Y}.\ P_\mathcal{Y}(Y = y) = p \}$ and $m_{P_\mathcal{Y}}$ is the multiplicity function of those probabilities. In Section~\ref{sec:idea_warmup}, we were \emph{given} (or defined) $M_{P_\mathcal{X}}$ and by doing so partially defined $P_\mathcal{X}$. In this case, we \emph{are not} given (or do not define) $M_{P_\mathcal{Y}}$. Rather, we just defined the relationship between $M_{P_\mathcal{Y}}$ and $P_\mathcal{Y}$. We know from Equation~\ref{eqn:no_pairings} that $P_\mathcal{Y}(Y' = y_0 | Y = y_0) = \sum_{q \in M_{P_\mathcal{Y}}} q^2$. In this case, because $M_{P_\mathcal{Y}}$ is undefined, this value is also undefined.

Fortunately, we can still apply a worst case analysis. Let $\mathcal{M}^{P_\mathcal{Y}}$ be the set of all possible values for $M_{P_\mathcal{Y}}$. That is let:

$$\mathcal{M}^{P_\mathcal{Y}} = \left\{M = (S, m)\ |\ |M| = |\mathcal{Y}| \land \left(\forall p \in S.\ p \geq 0.\right) \land \sum_{p \in S} p \cdot m(p) = 1 \right\}$$

Then with this definition of $\mathcal{M}^{P_\mathcal{Y}}$, we can derive the bound in Equation~\ref{eqn:total_ignorance_bound} as follows.

\begin{align*}
P_\mathcal{Y}(Y' = y_0 | Y = y_0) &= \sum_{q \in M_{P_\mathcal{Y}}} q^2 \\
&\geq \min_{M \in \mathcal{M}^{P_\mathcal{Y}}} \left\{ \sum_{q \in M} q^2 \right\} = \sum_{i = 1}^{|\mathcal{Y}|} \left(\frac{1}{|\mathcal{Y}|}\right)^2 = \frac{1}{|\mathcal{Y}|}
\end{align*}

In other words, the value for $M_{P_\mathcal{Y}}$ that minimizes Equation~\ref{eqn:no_pairings} is $M_{P_\mathcal{Y}} = \left\{\frac{1}{|\mathcal{Y}|}, \frac{1}{|\mathcal{Y}|}, ..., \frac{1}{|\mathcal{Y}|}\right\}$ which would yield a confidence of $\frac{1}{|\mathcal{Y}|}$. Thus this becomes the lower bound.

Having established this method for obtaining confidence lower bounds, we now turn to lower-bounding confidences in more complex scenarios.

\section{Multiple Distributions - One Undefined}\label{sec:hypothesis_testing_math}

In Section~\ref{sec:completely_undefined_probs} we introduced a way to obtain a lower bound on a confidence that a result would repeat when our confidence function was a completely undefined probability function. However, sometimes a person is presented with a context where their model for what occurs is a mix of defined and undefined probability functions. Single hypothesis testing is a classic example of this situation, where the null hypothesis' probability function over the result space is (usually) completely defined but the alternative hypothesis (usually) leaves the probabilities over the result space undefined. In this section we move our analysis toward more complex situations, including that of null hypothesis testing.

As usual, we consider sampling twice from a set. This time we sample from the finite set $\mathcal{Z}$. We represent our uncertainty about sampling with the probability function $P_\mathcal{Z}$. In this case we actually have \emph{two different} distributions with which to sample from $\mathcal{Z}$, the ``heads distribution'' and the ``tails distribution.'' Each time we sample from $\mathcal{Z}$, we first flip a coin to choose which distribution to sample with. The coin is biased and flips heads (event $H$ the first time, $H'$ the second time) with probability $P_\mathcal{Z}(H) = P_\mathcal{Z}(H')$ and tails (events $T$, $T'$) with probability $P_\mathcal{Z}(T) = P_\mathcal{Z}(T') = 1 - P_\mathcal{Z}(H)$. Let $Z$ be the random variable representing our first sample and $Z'$ represent the second.

In this section we let the distribution associated with flipping heads be completely defined. That is, $P_\mathcal{Z}(Z | H)$ and $P_\mathcal{Z}(Z' | H)$ are completely defined. However, we will leave $P_\mathcal{Z}(Z | T)$ and $P_\mathcal{Z}(Z' | T)$ completely undefined like in Section~\ref{sec:completely_undefined_probs}. Under this setup, we obtain our first sample, \emph{but} we do not get to see the coin; we just observe the event $Z = z_0$. Having observed $Z = z_0$, we can obtain the following confidence bound:

\begin{equation}\label{eqn:hype_basis}
P_\mathcal{Z}(Z' = z_0 | Z = z_0) \geq P_\mathcal{Z}(Z' = z_0 | H)P_\mathcal{Z}(H') + \frac{1}{|\mathcal{Z}|}P_\mathcal{Z}(T')^2
\end{equation}

We proceed to explain and derive this result in the rest of this section. To understand the above bound more concretely, consider the example in the third challenge of the Monty Hallways Gameshow. Here heads corresponds to the distribution over the blue doors in the example, and tails corresponds to the yellow doors. The event $Z = z_0$ represents seeing the first block of Grover's Cheddar.

\begin{figure}
% The \phantomcaption allows for an invisible caption.
% \phantomcaption{}\label{fig:third_story_task}
\begin{tcolorbox}[colback=green!10!white,colframe=green!50!black,before upper={\parindent15pt},title=\textbf{The Monty Hallways Gameshow - Third Challenge}]
You are brought to the third and final challenge of today's show. This time there are two sets of doors, colored blue and yellow. On the blue doors, both probabilities and pictures of the dairy products are visible. The yellow doors are completely blank, but your host assures you that for every product shown on a blue door there is a corresponding yellow door and that the yellow doors have some other probability distribution associated with them. To sample a product, your host will first (fairly) flip a fair coin; one side is blue - the other, yellow. The color of the coin flip will determine which set of doors (and thus which distribution) is used to select a dairy product.

\ 

You are blindfolded and neither see the result of the coin flip nor which door opens. When unblindfolded, you see a block of Grover's Cheddar. ``Now...'' the host asks you, ``You must tell me, what is your minimum confidence that if we use the same set of doors (blue or yellow, you do not know) and sample a product again, we'll get another block of Grover's Cheddar?'' This one takes you a while, but after some careful calculations, you offer your answer. Your host is thrilled. ``Congratulations! Someone get this winner their half-and-half!''

\ 

(The math behind this case is presented in Section~\ref{sec:hypothesis_testing_math}.)
\end{tcolorbox}
\end{figure}

Equation~\ref{eqn:hype_basis} appears to use something like our bound from Section~\ref{sec:completely_undefined_probs}. Perhaps the most surprising thing about Equation~\ref{eqn:hype_basis} is that $P_\mathcal{Z}(T')$ is squared. While we use the same sort of reasoning we used in Section~\ref{sec:completely_undefined_probs}, here in Equation~\ref{eqn:hype_basis} we square $P_\mathcal{Z}(T')$ because there's only a $P_\mathcal{Z}(T') = P_\mathcal{Z}(T)$ chance that the result $Z = z_0$ was actually sampled using $P_\mathcal{Z}(\cdot | T)$. In other words,

\section{Application to Single Hypothesis Testing}\label{sec:single_hypothesis_testing}

We now turn to the direct application of our results to single (i.e. null) hypothesis testing. Often, a researcher wishes to test a \emph{single}, ``null,'' hypothesis, such as ``the coin is fair'' or ``the treatment is more than 70\% effective.'' The researcher runs an experiment and wishes to determine whether the result counts as evidence against the null hypothesis and, if so, quantify how strong the evidence is. There are presently two major ways to get numeric results for this sort of hypothesis testing: p-values and Bayes factor analysis. That is, when a researcher wants to quantitatively judge whether an experimental result counts as evidence against a null hypothesis, they will employ either some kind of p-value-granting statistical test or obtain a Bayes factor. However, both p-values and standard Bayes factor analysis techniques have serious conceptual issues.

\subsection{Defining Statistical Evidence}

Usually, researchers are not intending to rely solely on their one experiment to determine their beliefs on a subject. Rather, they intend to use that experimental result as one piece of \emph{evidence} amidst a wider collection of other pieces of evidence - perhaps some of which will only be acquired in the future.

The best mathematical, probabilistic interpretation of what it means for a result $R$ to count as \emph{evidence} (and how strong that evidence is), is how much the result $R$ increases or decreases one's confidence that the null hypothesis is true. Expressed mathematically, this means the following: Let $N$ denote the event that the null hypothesis is true. Then result $R$ should be understood as evidence in the following sense: Let $P(N)$ and $P(\bar{N}) = 1 - P(N)$ be a person's confidences that the null hypothesis is true/false respectively \emph{before} they see the experimental result. Let $P(N | R)$ and $P(\bar{N} | R) = 1 - P(N | R)$ be that person's confidences that the null hypothesis is true/false \emph{after} they see the experimental result. Then $R$ is considered to have been evidence according to the factor by which it changed the person's confidence:

$$\text{evidence for/against }N = \left ( \frac{P(N | R)}{P(\bar{N} | R)} \middle /  \frac{P(N)}{P(\bar{N})} \right ) = \frac{P(R | N)}{P(R | \bar{N})}$$

This is to say, if we are going to try to treat evidence as a matter of mathematics and probabilities, then the evidence for/against $N$ is best understood as the ``Likelihood Ratio,'' $\frac{P(R | N)}{P(R | \bar{N})}$, because the likelihood ratio quantifies how much the result $R$ would change a person's numeric confidence in $N$. This viewpoint is cogently and thoroughly argued in Richard Royall's book \emph{Statistical Evidence: A Likelihood Paradigm} \cite{royall1997statistical}. A curious or suspicious reader may find Royall's book valuable; however, for the purposes of this paper, it should be sufficient for the reader to keep in mind our stated reason for using likelihood ratios as a valid numeric quantification of evidence: the likelihood ratio quantifies how much a person's numeric confidence would change given the experimental result.

\subsection{If Likelihood Ratios are the Answer, What is the Rest of this Paper For?}

We, along with others, believe that likelihood ratios are the best mathematical formulation of evidence in a probabilistic context. \emph{\textbf{However}, as far as we are aware, before this paper there was no good way to acquire a likelihood ratio when using only a single (null) hypothesis.} This is because a likelihood ratio in single-hypothesis testing requires both a probability of the result $R$ given the null hypothesis ($P(R | N)$) \emph{and} a probability of the result $R$ given that the null hypothesis is false ($P(R | \bar{N})$). Usually, however, the alternative hypothesis $\bar{N}$ is too vague to provide this latter probability. For example, consider the question, ``What is the probability of flipping a coin ten times and getting two heads given that the coin is \emph{not} a fair 50-50 coin?'' This question has no answer.

Bayes factor analysis purports to provide an answer via its use of prior probabilities over the parameters of the coin in the event that the coin is not 50-50. We and many others find this technique suspect.

Rather than directly attempting to provide an answer, we create a generalization of the likelihood ratio and use our results from earlier in the paper to \emph{lower-bound} this generalization's expression of the strength of evidence against the null. First though, we must cover some conceptual ground behind interpreting probabilities as confidences; applying our mathematical results to hypothesis testing only makes sense under certain philosophic views of confidences.

\subsection{Our Requirements for Interpretation of Probabilities as Confidences}

In order to derive our mathematical results in Sections~\ref{sec:idea_warmup} through~\ref{sec:hypothesis_testing_math}, it was sufficient to require that 

As we have already alluded to 

\subsection{Introducting the ``Repeat Ratio'' as Evidence}

When probability functions are undefined, the likelihood ratio is also undefined - even bounds on the likelihood ratio are undefined. In this section we introduce a generalization of the likelihood ratio that equals the likelihood ratio when probability functions are defined, but which can be lower/upper bounded when the functions are undefined. Due to the close conceptual link between the likelihood ratio and our alternative, we suggest that our alternative be treated as a valid expression of mathematical evidence.

To obtain this generalization, we revisit the idea of repeating a result. Throughout the paper so far, we have been considering confidences about an event ``repeating'' if the process could be done over again. We have modeled this as sampling twice (independently) from the same distribution. In this section, given an event $E$, we use $E'$ as shorthand for ``$E$ occurs when the trial is independently repeated.'' \textbf{TODO: More philosophically (and mathematically) formalize what I mean by an event repeating INDEPENDENTLY.} \textbf{Model as sampling with replacement.}

Importantly, when a probability function $P$ is fully defined, then $P(E' | E) = P(E') = P(E)$. Thus, when a probability function is fully defined for two hypotheses $H_1$ and $H_2$, the likelihood ratio $\frac{P(E | H_1)}{P(E | H_2)}$ equals the expression $\frac{P(E' | E, H_1)}{P(E' | E, H_2)}$. We call this latter ratio the ``Repeat Ratio.'' When working with defined probability functions, a person could use the repeat ratio instead of the likelihood ratio and get the exact same results. However, when working with undefined probability functions, a person cannot get likelihood ratios or even bounds on the likelihood ratios, but they \emph{can} get bounds on the repeat ratio.

\textbf{TODO: Workshop a better name than ``repeat ratio.''}

\section{Answering Objections}\label{sec:objections}

\section{Conclusion}

\bibliography{references}
\bibliographystyle{ieeetr}

\begin{appendices}

\section{Partially Undefined Probabilities}\label{sec:partially_undefined_probs}

\textbf{TODO: write about when the blue pairing is unknown.}

\end{appendices}

%\section{Introduction Part 2 - The Monty Hallways Gameshow}

%You are a participant in The Monty Hallways Gameshow - a challenge for statisticians sponsored by the local dairies' ``Got half-and-half?'' campaign. You will need to perform a series of statistical tasks adequately in order to win the prize - a collection of premium half-and-half products.

%\textbf{TODO: Replace 20-sided die with a coin.}

%Being led into yet another hallway, you observe that there are two kinds of doors. Half the doors are blue and half are yellow. The blue doors have probabilities on them. Your host tells you that on the back side of each yellow door is a number corresponding to some other probability distribution. Thus there are two distributions, the blue and the yellow. None of the doors have the product pictures. The host tells you that each product is associated with both a blue door and a yellow door. On a table in the middle of the hallway is a 20-sided die, where 8 faces are yellow and 12 are blue. The host tells you that he will roll the die; the color of the face will determine which of the two probability distributions (yellow or blue) is used to decide which door to open.

%With the stage set, the sixth task begins. Once again you are blindfolded. The die is rolled, a door is opened, and a block of Grover's Cheddar is brought forth. The host hides the die from you, and then you are unblindfolded. ``Now...'' the host asks you, ``You must tell me, what is your minimum confidence that if we re-roll the die and open a door again, we'll get another block of Grover's Cheddar?'' This one takes you a while, but after some careful calculations, you offer your answer. ``Excellent!'' your host exclaims, ``I have one final question for you. The blue door for Grover's Cheddar is this one over here...'' the host says as he points at a particular blue door, ``Do you wish to change your minimum confidence?'' With this new information in mind, you ponder the chances and come up with a new minimum confidence. Your host is thrilled. ``Congratulations! Someone get this winner their half-and-half!''

%What were your answers to tasks three, five, and six? This paper explores the math behind those answers. In the process we reveal that even when your probability function is completely undefined (e.g. no numbers on doors and no assumed priors) there are still cases where you can reasonably have certain minimum confidences. Furthermore, the techniques we present in this paper enable a new form of single-hypothesis testing, which we discuss in the latter half of the paper.

%\section{Related Work}

%Perhaps the most famous distribution which is undefined in some sense is the Cauchy Distribution \cite{poisson1827probabilite, cauchy1853resultats}; the Cauchy Distribution has a defined pdf, but its mean and variance are undefined.

%A related project is the attempt to argue for the use of certain ``uninformative'' priors when someone does not have a particular reason to use other priors. For example, the uniform prior and the Jeffereys prior are considered to be potentially good options for ``uninformative'' priors \cite{jeffreys1998theory, price2002uninformative}.

%Perhaps the closest project to ours is that of ``imprecise probabilities,'' which basically involves using an upper and lower bound(s) on a probability rather than a single value \cite{walley1991statistical, walley2000towards}.

%\section{Our Methodology - Answering the Monty Hallways Problems}

%To introduce and explain our results, we will discuss the tasks from the Monty Hallways Gameshow described in Section~\ref{sec:main_gameshow_segment} one by one.

%\subsection{Task Number Three}

%As a recap, in this task you had the probabilities on the doors, but not the pictures. Thus you did know which door the gallon of milk came from. You were asked how confident you were that the same product would appear again if the process were repeated.

%Let $n$ be the number of doors and $p_1$, $p_2$, ..., $p_n$ be the probabilities on the doors. You know that the door with probability $p_1$ had a chance of $p_1$ of being opened. Thus, you are $p_1$ confident that the milk came from door one. This means that you are $p_1$ confident that the chance the milk will be brought forth again is $p_1$. The same applies to each door. You are $p_i$ confident that the milk came from door $i$, meaning that you are $p_i$ confident that the milk has a chance of $p_i$ of appearing.

%Let $LM$ be the event you already observed, namely the event that Leonard's 2\% Milk was brought forth. Let $LM'$ be the event that Leonard's 2\% Milk would be brought forth again if the process were repeated. Lastly, let $D_i$ be the event that the milk came from door $i$. Then you can express your confidence the milk will re-appear as conditioned on the door the milk came from:

%$$P(LM' | LM) = \sum_{i = 1}^n P(LM' | D_i) P(D_i) = \sum_{i = 1}^n p_i^2$$

%Consequently, \emph{even though} you did not know which door Leonard's Milk came from, the sheer fact that you observed it being brought forth was enough to give you a \emph{particular} confidence that Leonard's Milk would appear again.

%\subsubsection{Generalized Version}

%This result generalizes directly as follows: Let $X$ be a random variable which will take on one of $n$ values. Let $p_1, p_2, ... p_n$ be the probabilities of those values, but where you do not know which probability is for which value. In terms of the task three analogy, $X$ corresponds to ``the product'' which will be one of the $n$ specific products. Let $X'$ be a random variable whose distribution is identical to $X$. In terms of the analogy, assigning $X'$ a value corresponds to bringing forth a second product. Given these definitions, if you observe the event $X = x$ (e.g. ``the product'' = Leonard's 2\%), your confidence that $X'$ will take on value $x$ becomes:

%\begin{equation}
%P(X' = x | X = x) = \sum_{i = 1}^n p_i^2
%\end{equation}

%This result informs the process for answering tasks five and six.

%\subsection{Task Number Five}

%To recap, in this task the doors had probabilities associated with them, but you did know those probabilities. You got to see which product was brought forth (a box of Harriet's Best cream cheese), and were asked to give a minimum confidence (a lower bound on your confidence) that the same cream cheese would be brought out if the process were repeated.

%This task is effectively equivalent to task three \emph{except} that you do not know the set of probabilities. However, you know that there \emph{were} a total of $n$ probabilities $p_1, p_2, ..., p_n$ and the chance that the $i$th door opened (event $D_i$) was $p_i$. If you knew the $p_i$'s, you could simply calculate as you did in task three: sum the squares of the probabilities.

%Fortunately, you were only asked for a \emph{lower bound} on your confidence. Thus, you ask yourself the question, ``If an adversary was allowed to assign the values $p_1, p_2, ..., p_n$, would there still be a minimum value to the sum of the squares?'' You realize that the sum of squares is minimized when each $p_i = \frac{1}{n}$. Therefore, \emph{no matter what} the distribution was, if you were allowed to perform your confidence calculation from task three on that distribution, your confidence would be at least $n \cdot \left(\frac{1}{n}\right)^2 = \frac{1}{n}$. Thus, given that you observed Harriet's Best cream cheese the first time (event $HB$) you can be at least $\frac{1}{n}$ confident that the same would brought out if the process were repeated (event $HB'$): $P(HB' | HB) \geq \frac{1}{n}$.

%\subsubsection{Generalized Version}

%This result generalizes as follows: Let $X$ be a random variable which can take on one of $n$ values and $P$ be the probability function which governs $X$, but which is unknown to you. That is, your confidence about which values $X$ will take is simply undefined; $P$ is mathematically undefined other than that is restricted to being probability function. This is equivalent to not knowing the numbers on the doors in task five. Let $X'$ be another random variable just like $X$; that is, $X'$ takes on a value from the same set as $X$ with the same probabilities.

%Now, upon observing $X$ take on a value $x$, you can set a minimum confidence:

%\begin{equation}
%P(X' = x | X = x) \geq \frac{1}{n} 
%\end{equation}

%Just like the technique from task three helped solve task five, this technique helps solve task six.

%\subsection{Task Number Six - Part 1}

%In the sixth task, you knew that there were two probability distributions. You knew the blue distribution but not the yellow distribution. The host chose which distribution was sampled from by rolling a 20-sided die. In this case there was an $\frac{8}{20}$ chance of drawing from the yellow distribution and a $\frac{12}{20}$ chance of drawing from the blue distribution. Let $B$ be the event that the host drew from the blue distribution (i.e. opened a blue door), and let $B'$ be the event that a blue door will be opened if the process is repeated. Let $Y$ and $Y'$ be the same respective events for yellow. Then we have the $P(B) = P(B') = \frac{12}{20} = \frac{3}{5}$ and $P(Y) = P(Y') = 1 - P(B) = \frac{2}{5}$.

%Let $b_1, b_2, ..., b_n$ be the blue probabilities for the $n$ blue doors and $y_1, y_2, ..., y_n$ be the yellow probabilities for the $n$ yellow doors. In this setting, you will use the convention that if the $i$th blue door corresponds to certain dairy product then the $i$th yellow door corresponds to that same product. Using this convention does not change the mathematical results; it simply helps express them. Given this defintion of the $b_i$'s and $y_i$'s, you know that for the $i$th product, the probability $p_i$ of getting that product is equal to $b_i P(B') + y_i P(Y')$.

%You observed a block of Grover's Cheddar (event $GC$) and are asked for a minimum confidence you would observe Grover's Cheddar again if the process were repeated (event $GC'$). Let $D_{b_i}$ be the event that the $i$th blue door was opened and $D_{y_i}$ be the event that the $i$th yellow door was opened. As with tasks three and five, you can think of your confidence as the sum of the squares of the $p_i$'s. We derive this as follows:

%\begin{align*}
%P(GC' | GC) &= \sum_{i = 1}^n P(GC' | D_{b_i} \cup D_{y_i}, GC) P(D_{b_i} \cup D_{y_i}| GC) \\
% &= \sum_{i = 1}^n (P(GC' | B', D_{b_i} \cup D_{y_i}, GC) P(B' | D_{b_i} \cup D_{y_i}, GC) \\
% & \ \ \ \ \ \ \ \ \ \ \ + P(GC' | Y', D_{b_i} \cup D_{y_i}, GC) P(Y' | D_{b_i} \cup D_{y_i}, GC) ) \\
% & \ \ \ \ \ \ \ \ \ \cdot (b_i P(B) + y_i P(Y)) \\
% &= \sum_{i = 1}^n (P(GC' | B', D_{b_i} \cup D_{y_i}, GC) P(B') + P(GC' | Y', D_{b_i} \cup D_{y_i}, GC) P(Y') ) \\
% & \ \ \ \ \ \ \ \ \ \cdot (b_i P(B) + y_i P(Y)) \\
% &= \sum_{i = 1}^n (b_i P(B') + y_i P(Y')) (b_i P(B) + y_i P(Y)) \\
% &= \sum_{i = 1}^n (b_i P(B) + y_i P(Y))^2 
%\end{align*}

%Like in task five, this sum is undefined. In task five you obtained a minimum confidence by thinking of the values an adversary could choose for the $p_i$'s that would minimize the sum of squares. Here the $b_i$'s are defined, so the adversary has fewer options, but you can still think of values for the $y_i$'s an adversary would choose that minimizes the sum of squared $p_i$'s. In other words, you solve the minimization problem:

%$$P(GC' | GC) \geq \min_{\vec{y} \in \mathbb{R}^n} \left\{ \sum_{i = 1}^n \left(b_i P(B) + y_i P(Y)\right)^2 \right\}	$$

%This expression is minimized by satisfying the following constraints for the probability distribution $y_1, y_2, ..., y_n$:

%$$\forall i, j \in \{1, 2, ..., n\}.\ b_i \geq b_j \rightarrow \left(y_i = 0 \lor y_j P(Y) + b_j P(B) = y_i P(Y) + b_i P(B)\right).$$

%These constraints can be satisfied with a simple $O(n \log n)$ algorithm, and perhaps some faster algorithm of which we are not aware.

%\subsection{Task Number Six - Part 2}

%After you found your confidence for the first part of task six, your gameshow host told you which blue door corresponds to Grover's Cheddar. Thus you gained some new information. Then the host asked you if you would like to change your minimum confidence that if the process were repeated Grover's Cheddar would be brought forth again.

%Once you know the blue door (say it's door $j$), then you know the blue probability of getting Grover's Cheddar ($b_j$). However, you still do not know which yellow door is the yellow door for Grover's Cheddar. Let $D_{y_i}$ be the event that a product came forth from yellow door $i$. Recall that $P(B) = \frac{3}{5}$ represents the chance of rolling a blue face on the 20-sided die and $P(Y) = 1 - P(B) = \frac{2}{5}$ represents the chance of rolling a yellow face. Then you can express your confidence as follows:

%\textbf{TODO: Finish Math}

\end{document}


==> old_excerpts.tex <==
\input{preamble}

\title{Undefined Probability Functions - Old Excerpts}
\author{Justus Isaiah Hibshman}
\date{May 2021}

\begin{document}

\maketitle

\section{Hellinger Content}

\subsection{Intro to Statistical Metrics}

We have two front-runners for consideration, the Total Variance metric and the Hellinger metric.

We use our metric for two things: Defining Borel $\sigma$-algebras over credal sets, and formulating a notion of a ``uniform'' distribution which we use specifically for an important conjecture.

When it comes to the first purpose, our choice does not matter, because Total Variance and Hellinger create the same Borel $\sigma$-algebras. \textbf{TODO: Get citation from something over than online lecture notes.} When it comes to our central conjecture, we find for finite simulations both the Total Variance metric and the Hellinger metric give us the same results; we are uncertain about the infinite case (hence the conjecture). \textbf{TODO: Revisit -- True?} However, Hellinger seems more appropriate for our conjecture because it creates a unique, privileged definition of ``uniform'' that Total Variance seems to fail to provide. \textbf{$\leftarrow$ Revisit that too.}

\subsubsection{The Hellinger Metric}

While the total variance metric is effectively a generalization of the $L_1$ distance metric (i.e. ``Manhattan distance''), the Hellinger metric is akin to a generalization of the $L_2$ distance metric (i.e. ordinary, everyday, Euclidean distance).

Formally, given probability spaces ($\Omega$, $\mathcal{F}$, $P_A$) and ($\Omega$, $\mathcal{F}$, $P_B$), as well as a third measure $\mu$ which is absolutely continuous with both $P_A$ and $P_B$, the Hellinger distance between $P_A$ and $P_B$ is defined to be:

$$H(P_A, P_B) = \sqrt{\frac{1}{2} \int_\Omega \left(\sqrt{\frac{\text{d}P_A}{\text{d}\mu}} - \sqrt{\frac{\text{d}P_B}{\text{d}\mu}} \right)^2 \text{d}\mu}$$

Due to the way it is defined, the Hellinger metric is independent of the choice of $\mu$. We define a notion of ``uniformity'' in a similar fashion later in Section~\ref{sec:uniformity}.

When our sample space $\Omega$ is finite, a probability function can be thought of as a $|\Omega|$-dimensional vector, summing to 1. In this case, the Hellinger metric corresponds to shifting the probability functions from the $L_1$ simplex to the $L_2$ simplex by taking the square root of each vector component, then taking the Euclidean distance between the two new vectors.

\subsection{Intro to Uniformity}

In this paper, we will define uniformity over $\mathcal{C}$ with respect to some distance metric $d$, and will focus on when $d$ is the Hellinger metric $H$ because, like the Euclidean metric for $\mathbbm{R}^n$, the Hellinger metric leaves our uniform measure unaffected by our choice of parametrization.

\subsection{Main Conjecture}

Let $d$ be a distance metric for probability functions which produces the same uniform distribution for any simple parametrization (e.g. Hellinger). All claims in this section which implicitly reference a distance metric shall be understood to reference $d$.

\section{Higher Order Uniformity :(}

Because we can define a uniform distribution over our first order credal set $\mathcal{C}^1$ using some (any) $n$-dimensional simple parametrization, then it follows that we can define a uniform measure for \emph{all} our higher order credal sets. Let $d$ be our distance metric of choice. We can obtain our higher order uniform distributions inductively in the following fashion:

\begin{enumerate}
    \item Assume we have a simple parametrization $p^i : I_1^i \times ... \times I_n^i \rightarrow \mathcal{C}^i$. Then we can think of any probability function $P^{i+1} \in \mathcal{C}^{i + 1}$ as being a probability function over our parametrization space $I_1^i \times ... \times I_n^i$ via $(p^i)^{-1}$.
	\item We can order the points in $(p^i)^{-1}(\mathcal{C}^i) = I_1^i \times ... \times I_n^i$ via the ordering $\precsim_{p^i}$ defined such that:
    $$
	\begin{aligned}
	 & \langle x_1, x_2, ..., x_n \rangle \precsim_{p^i} \langle y_1, y_2, ..., y_n \rangle \\
	 & \ \ \leftrightarrow x_1 \geq y_1 \land \left(\forall 2 \leq i \leq n.\ x_i < y_i. \rightarrow \exists 1 \leq j < i.\ x_j > y_j \right)
	\end{aligned}
	$$
	\item This ordering of $(p^i)^{-1}(\mathcal{C}^i)$ allows us to order the cumulative distribution functions (``cdfs'') of the elements of $\mathcal{C}^{i+1}$.
    \item We can then order these $(i+1)$th order cdfs with a transitive ordering $\precsim_{\mathcal{C}^{i+1}}$ defined such that:

\begin{equation*}
\begin{aligned}
    \forall P_A, P_B \in \mathcal{C}^{i+1}.\ \left(P_A \precsim_{\mathcal{C}^{i+1}} P_B \right) \leftrightarrow & (\forall y \in (p^i)^{-1}(\mathcal{C}^i).\ \text{CDF}_{P_A}(y) < \text{CDF}_{P_B}(y) \\
 & \rightarrow ( \exists x \in (p^i)^{-1}(\mathcal{C}^i).\ (x \precsim_{p^i} y.\ \\ 
 & \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \land \text{CDF}_{P_A}(x) > \text{CDF}_{P_B}(x) ) ) )
\end{aligned}
\end{equation*}
    \item A transitive ordering on our set $\mathcal{C}^{i+1}$ of cardinality $|\mathbbm{R}|$ corresponds to a family of injections from $\mathcal{C}^{i+1}$ to $\mathbbm{R}$ where for each injection $f: \mathcal{C}^{i+1} \rightarrow \mathbbm{R}$, $f(\mathcal{C}^{i+1})$ is an continuous interval (possibly $(-\infty, \infty)$) and $P_A \precsim_{\mathcal{C}^{i+1}} P_B \leftrightarrow f(P_A) \leq f(P_B)$. Crucially, due to the way that $\precsim_{\mathcal{C}^{i+1}}$ orders cdfs, each $f$ is a one-dimensional parametrization of $\mathcal{C}^{i+1}$ which is continuous in terms of $d$.
\end{enumerate}

As discussed in Section~\ref{sec:defining_uniformity_over_credal_sets}, because these parametrizations exist, uniform distributions over our credal sets also exist. We denote the uniform distribution over the $i$th order credal set with $U_d^{i + 1}$.

...

$$\lim_{i \rightarrow \infty} U_d^{i+1}\left(\left\{P^i\ |\ P^i \in \mathcal{C}^i \land \exists E \in \mathcal{F}.\ P^i(E) \neq U_d^2(E)\right\}\right) = 0$$

\section{Misc I}


You are a participant in The Monty Hallways Gameshow - a challenge for statisticians sponsored by the local dairies' ``Got half-and-half?'' campaign. You will need to perform a series of statistical tasks adequately in order to win the prize - a collection of premium half-and-half products.

\textbf{TODO: Replace 20-sided die with a coin.}

Being led into yet another hallway, you observe that there are two kinds of doors. Half the doors are blue and half are yellow. The blue doors have probabilities on them. Your host tells you that on the back side of each yellow door is a number corresponding to some other probability distribution. Thus there are two distributions, the blue and the yellow. None of the doors have the product pictures. The host tells you that each product is associated with both a blue door and a yellow door. On a table in the middle of the hallway is a 20-sided die, where 8 faces are yellow and 12 are blue. The host tells you that he will roll the die; the color of the face will determine which of the two probability distributions (yellow or blue) is used to decide which door to open.

With the stage set, the sixth task begins. Once again you are blindfolded. The die is rolled, a door is opened, and a block of Grover's Cheddar is brought forth. The host hides the die from you, and then you are unblindfolded. ``Now...'' the host asks you, ``You must tell me, what is your minimum confidence that if we re-roll the die and open a door again, we'll get another block of Grover's Cheddar?'' This one takes you a while, but after some careful calculations, you offer your answer. ``Excellent!'' your host exclaims, ``I have one final question for you. The blue door for Grover's Cheddar is this one over here...'' the host says as he points at a particular blue door, ``Do you wish to change your minimum confidence?'' With this new information in mind, you ponder the chances and come up with a new minimum confidence. Your host is thrilled. ``Congratulations! Someone get this winner their half-and-half!''

What were your answers to tasks three, five, and six? This paper explores the math behind those answers. In the process we reveal that even when your probability function is completely undefined (e.g. no numbers on doors and no assumed priors) there are still cases where you can reasonably have certain minimum confidences. Furthermore, the techniques we present in this paper enable a new form of single-hypothesis testing, which we discuss in the latter half of the paper.

\section{Old Related Work}

Perhaps the most famous distribution which is undefined in some sense is the Cauchy Distribution \cite{poisson1827probabilite, cauchy1853resultats}; the Cauchy Distribution has a defined pdf, but its mean and variance are undefined.

A related project is the attempt to argue for the use of certain ``uninformative'' priors when someone does not have a particular reason to use other priors. For example, the uniform prior and the Jeffereys prior are considered to be potentially good options for ``uninformative'' priors \cite{jeffreys1998theory, price2002uninformative}.

Perhaps the closest project to ours is that of ``imprecise probabilities,'' which basically involves using an upper and lower bound(s) on a probability rather than a single value \cite{walley1991statistical, walley2000towards}.

\section{Our Methodology - Answering the Monty Hallways Problems}

To introduce and explain our results, we will discuss the tasks from the Monty Hallways Gameshow described in Section~\ref{sec:main_gameshow_segment} one by one.

\subsection{Task Number Three}

As a recap, in this task you had the probabilities on the doors, but not the pictures. Thus you did know which door the gallon of milk came from. You were asked how confident you were that the same product would appear again if the process were repeated.

Let $n$ be the number of doors and $p_1$, $p_2$, ..., $p_n$ be the probabilities on the doors. You know that the door with probability $p_1$ had a chance of $p_1$ of being opened. Thus, you are $p_1$ confident that the milk came from door one. This means that you are $p_1$ confident that the chance the milk will be brought forth again is $p_1$. The same applies to each door. You are $p_i$ confident that the milk came from door $i$, meaning that you are $p_i$ confident that the milk has a chance of $p_i$ of appearing.

Let $LM$ be the event you already observed, namely the event that Leonard's 2\% Milk was brought forth. Let $LM'$ be the event that Leonard's 2\% Milk would be brought forth again if the process were repeated. Lastly, let $D_i$ be the event that the milk came from door $i$. Then you can express your confidence the milk will re-appear as conditioned on the door the milk came from:

$$P(LM' | LM) = \sum_{i = 1}^n P(LM' | D_i) P(D_i) = \sum_{i = 1}^n p_i^2$$

Consequently, \emph{even though} you did not know which door Leonard's Milk came from, the sheer fact that you observed it being brought forth was enough to give you a \emph{particular} confidence that Leonard's Milk would appear again.

\subsubsection{Generalized Version}

This result generalizes directly as follows: Let $X$ be a random variable which will take on one of $n$ values. Let $p_1, p_2, ... p_n$ be the probabilities of those values, but where you do not know which probability is for which value. In terms of the task three analogy, $X$ corresponds to ``the product'' which will be one of the $n$ specific products. Let $X'$ be a random variable whose distribution is identical to $X$. In terms of the analogy, assigning $X'$ a value corresponds to bringing forth a second product. Given these definitions, if you observe the event $X = x$ (e.g. ``the product'' = Leonard's 2\%), your confidence that $X'$ will take on value $x$ becomes:

\begin{equation}
P(X' = x | X = x) = \sum_{i = 1}^n p_i^2
\end{equation}

This result informs the process for answering tasks five and six.

\subsection{Task Number Five}

To recap, in this task the doors had probabilities associated with them, but you did know those probabilities. You got to see which product was brought forth (a box of Harriet's Best cream cheese), and were asked to give a minimum confidence (a lower bound on your confidence) that the same cream cheese would be brought out if the process were repeated.

This task is effectively equivalent to task three \emph{except} that you do not know the set of probabilities. However, you know that there \emph{were} a total of $n$ probabilities $p_1, p_2, ..., p_n$ and the chance that the $i$th door opened (event $D_i$) was $p_i$. If you knew the $p_i$'s, you could simply calculate as you did in task three: sum the squares of the probabilities.

Fortunately, you were only asked for a \emph{lower bound} on your confidence. Thus, you ask yourself the question, ``If an adversary was allowed to assign the values $p_1, p_2, ..., p_n$, would there still be a minimum value to the sum of the squares?'' You realize that the sum of squares is minimized when each $p_i = \frac{1}{n}$. Therefore, \emph{no matter what} the distribution was, if you were allowed to perform your confidence calculation from task three on that distribution, your confidence would be at least $n \cdot \left(\frac{1}{n}\right)^2 = \frac{1}{n}$. Thus, given that you observed Harriet's Best cream cheese the first time (event $HB$) you can be at least $\frac{1}{n}$ confident that the same would brought out if the process were repeated (event $HB'$): $P(HB' | HB) \geq \frac{1}{n}$.

\subsubsection{Generalized Version}

This result generalizes as follows: Let $X$ be a random variable which can take on one of $n$ values and $P$ be the probability function which governs $X$, but which is unknown to you. That is, your confidence about which values $X$ will take is simply undefined; $P$ is mathematically undefined other than that is restricted to being probability function. This is equivalent to not knowing the numbers on the doors in task five. Let $X'$ be another random variable just like $X$; that is, $X'$ takes on a value from the same set as $X$ with the same probabilities.

Now, upon observing $X$ take on a value $x$, you can set a minimum confidence:

\begin{equation}
P(X' = x | X = x) \geq \frac{1}{n} 
\end{equation}

Just like the technique from task three helped solve task five, this technique helps solve task six.

\subsection{Task Number Six - Part 1}

In the sixth task, you knew that there were two probability distributions. You knew the blue distribution but not the yellow distribution. The host chose which distribution was sampled from by rolling a 20-sided die. In this case there was an $\frac{8}{20}$ chance of drawing from the yellow distribution and a $\frac{12}{20}$ chance of drawing from the blue distribution. Let $B$ be the event that the host drew from the blue distribution (i.e. opened a blue door), and let $B'$ be the event that a blue door will be opened if the process is repeated. Let $Y$ and $Y'$ be the same respective events for yellow. Then we have the $P(B) = P(B') = \frac{12}{20} = \frac{3}{5}$ and $P(Y) = P(Y') = 1 - P(B) = \frac{2}{5}$.

Let $b_1, b_2, ..., b_n$ be the blue probabilities for the $n$ blue doors and $y_1, y_2, ..., y_n$ be the yellow probabilities for the $n$ yellow doors. In this setting, you will use the convention that if the $i$th blue door corresponds to certain dairy product then the $i$th yellow door corresponds to that same product. Using this convention does not change the mathematical results; it simply helps express them. Given this defintion of the $b_i$'s and $y_i$'s, you know that for the $i$th product, the probability $p_i$ of getting that product is equal to $b_i P(B') + y_i P(Y')$.

You observed a block of Grover's Cheddar (event $GC$) and are asked for a minimum confidence you would observe Grover's Cheddar again if the process were repeated (event $GC'$). Let $D_{b_i}$ be the event that the $i$th blue door was opened and $D_{y_i}$ be the event that the $i$th yellow door was opened. As with tasks three and five, you can think of your confidence as the sum of the squares of the $p_i$'s. We derive this as follows:

\begin{align*}
P(GC' | GC) &= \sum_{i = 1}^n P(GC' | D_{b_i} \cup D_{y_i}, GC) P(D_{b_i} \cup D_{y_i}| GC) \\
 &= \sum_{i = 1}^n (P(GC' | B', D_{b_i} \cup D_{y_i}, GC) P(B' | D_{b_i} \cup D_{y_i}, GC) \\
 & \ \ \ \ \ \ \ \ \ \ \ + P(GC' | Y', D_{b_i} \cup D_{y_i}, GC) P(Y' | D_{b_i} \cup D_{y_i}, GC) ) \\
 & \ \ \ \ \ \ \ \ \ \cdot (b_i P(B) + y_i P(Y)) \\
 &= \sum_{i = 1}^n (P(GC' | B', D_{b_i} \cup D_{y_i}, GC) P(B') + P(GC' | Y', D_{b_i} \cup D_{y_i}, GC) P(Y') ) \\
 & \ \ \ \ \ \ \ \ \ \cdot (b_i P(B) + y_i P(Y)) \\
 &= \sum_{i = 1}^n (b_i P(B') + y_i P(Y')) (b_i P(B) + y_i P(Y)) \\
 &= \sum_{i = 1}^n (b_i P(B) + y_i P(Y))^2 
\end{align*}

Like in task five, this sum is undefined. In task five you obtained a minimum confidence by thinking of the values an adversary could choose for the $p_i$'s that would minimize the sum of squares. Here the $b_i$'s are defined, so the adversary has fewer options, but you can still think of values for the $y_i$'s an adversary would choose that minimizes the sum of squared $p_i$'s. In other words, you solve the minimization problem:

$$P(GC' | GC) \geq \min_{\vec{y} \in \mathbb{R}^n} \left\{ \sum_{i = 1}^n \left(b_i P(B) + y_i P(Y)\right)^2 \right\}	$$

This expression is minimized by satisfying the following constraints for the probability distribution $y_1, y_2, ..., y_n$:

$$\forall i, j \in \{1, 2, ..., n\}.\ b_i \geq b_j \rightarrow \left(y_i = 0 \lor y_j P(Y) + b_j P(B) = y_i P(Y) + b_i P(B)\right).$$

These constraints can be satisfied with a simple $O(n \log n)$ algorithm, and perhaps some faster algorithm of which we are not aware.

\subsection{Task Number Six - Part 2}

After you found your confidence for the first part of task six, your gameshow host told you which blue door corresponds to Grover's Cheddar. Thus you gained some new information. Then the host asked you if you would like to change your minimum confidence that if the process were repeated Grover's Cheddar would be brought forth again.

Once you know the blue door (say it's door $j$), then you know the blue probability of getting Grover's Cheddar ($b_j$). However, you still do not know which yellow door is the yellow door for Grover's Cheddar. Let $D_{y_i}$ be the event that a product came forth from yellow door $i$. Recall that $P(B) = \frac{3}{5}$ represents the chance of rolling a blue face on the 20-sided die and $P(Y) = 1 - P(B) = \frac{2}{5}$ represents the chance of rolling a yellow face. Then you can express your confidence as follows:

\section{Response to Sample Space Objection}

\subsection{Sample Space Representation Worries}

Depending on how we represent the sample and event spaces, we will obtain different values for the probability of the result given the null hypothesis. This ``problem'' affects almost all 

\textbf{TODO Update/Fill Out}

%In the section above we outlined mathematical limitations on when the techniques presented in this paper apply. In this section we further discuss those limitations. In particular, we saw above that the only kind of alternative hypothesis our bound works for (at present) is the completely agnostic alternative hypothesis - i.e. the hypothesis which includes all (and only) distinct distributions over the random variable. This raises two important questions:

%\begin{itemize}
%    \item What is the proper random variable to use when testing a null hypothesis $H$?
%    \item When does it make sense to use the ``completely agnostic'' alternative hypothesis? 
%\end{itemize}

%Our answer to these questions takes the form of the following two principles which we believe are intuitively true:

\begin{itemize}
     \item \textbf{Principle 1:} Use the question being asked to determine the relevant space of precise hypotheses. Specifically, given what is assumed, consider all possible alternatives to the null hypothesis. For example, imagine a machine which spits out bits. If we assume the bits are independent and have the null hypothesis ``The proportion of 1's produced by the machine is $p$.'' then the relevant space of hypotheses are well-defined hypotheses about other proportions. If, by contrast we do not assume independence and our null hypothesis is ``Each bit is produced independently an 1's occur with probability $p$.'' then the relevant space of hypotheses includes all possible correlations/relationships over the output bits.
     \item \textbf{Principle 2:} Use the space of relevant hypotheses being considered to determine the relevant random variable. In particular, use \emph{all} and \emph{only} the information in the experimental result relevant to distinguishing between fully-defined hypotheses. We can formalize this as:

Let $\mathcal{H}$ be the space of hypotheses obtained from Principle 1, expressed as probability functions. We know that our null hypothesis $P_N$ will be one of the elements of $\mathcal{H}$ and our alternative hypothesis $P_{\bar{N}}$ will have $\mathcal{V}(P_{\bar{N}}) = \mathcal{H} \setminus \{P_N\}$. Let $\Omega$ and $\mathcal{F}$ be the sample and event spaces on which the hypotheses are defined. We can partition the event space into the relevant outcomes as follows. Define equivalence classes on elements of $\Omega$ via the function $C : \Omega \rightarrow \mathbbm{R}$ where $C$ is defined such that:

$$\forall \omega_1, \omega_2 \in \Omega.\ \left( C(\omega_1) = C(\omega_2) \leftrightarrow \forall P \in \mathcal{H}.\ P(\{\omega_1\}) = P(\{\omega_2\}) \right)$$

Then $C$ is the relevant random variable for use in the hindsight ratio. In other words, $C$ groups elementary outcomes together if those outcomes are effectively the same according to the space of relevant hypotheses. We then use these groups as the relevant events.

\end{itemize}

These two principles tell an experimenter what random variable and alternative hypothesis to use. Sometimes following these principles allows the experimenter to use our bounds, sometimes they do not. We believe that if these two principles are followed, then \textbf{FILL IN} represents evidence against the null.

We believe that Principles 1 and 2 should be applied to \emph{all} statistical tests - not just the kinds of tests presented in this paper. These principles present a \emph{unique}, \emph{natural} way to represent experimental results. Having a natural, privileged way of representing statistical results deals with the issues and objections people raise surrounding methods which are affected by the size of the sample space (e.g. Royall~\cite{royall1997statistical}) or other objections based on result representation (e.g. Fitelson and Osherson~\cite{fitelson2012remarks}, and Pratt~\cite{pratt1961testing}).

Lastly, we note that a hindsight ratio, as with a likelihood ratio, expresses the evidence for/against one hypothesis vis-a-vis another hypothesis. To have evidence for/against a \emph{single} hypothesis, the second hypothesis needs to be the negation of the first. The hindsight ratios we present in this paper are not \emph{exactly} ``null hypothesis vs. the alternative hypothesis'' ratios; rather, because our ``completely agnostic'' hypothesis must include the null hypothesis itself as a possibility, our results \emph{approach} being a bound on the alternative hypothesis, but are technically a bound on something slightly different. We believe that the difference is practically negligible; after all, in the contexts where we apply our bounds: $\mathcal{V}(P_\text{Completely-Agnostic-Hypothesis}) = \mathcal{V}(P_\text{Alternative-Hypothesis}) \cup \{P_\text{Null-Hypothesis}\}$ and $|\mathcal{V}(P_\text{Alternative-Hypothesis})| = |\mathbbm{R}|$. Thus, our bound is effectively a bound on the evidence against the null hypothesis.

\section{Old Content for Hypothesis Testing}

\subsection{Introducing the ``Hindsight Ratio'' as Evidence}

When probability functions are undefined, the likelihood ratio is also undefined - even bounds on the likelihood ratio are usually undefined. In this section we introduce a generalization of the likelihood ratio that equals the likelihood ratio when probability functions are defined, but which more naturally corresponds to belief update mathematics when probability functions are undefined. Our generalized version, the ``hindsight ratio,'' can be lower/upper bounded when one of the probability functions is undefined, thereby allowing it to be used in single hypothesis testing.

To do a confidence update for two competing hypotheses $H_1$ and $H_2$, we normally take how likely an event seemed under $H_1$ vs. how likely it seemed under $H_2$ and use that ratio and Bayes' rule to update our confidences in $H_1$ and $H_2$. When probability functions are fully defined, ``How likely the result seemed under $H_1$'' just means $P(\text{result}\ |\ H_1)$. However, as we have seen in this paper, when probability functions can be undefined, ``How likely the result seemed under $H_1$'' is expressed by the hindsight probability $P(\langle \text{result} \rangle | H_1)$. That \emph{is} effectively the definition of a hindsight probability. Further, as we have seen, hindsight probabilities equal standard probabilities when the probability function is defined. Consequently, we suggest that it makes the most sense to update confidences via:

\begin{equation*}
\begin{aligned}
\frac{\text{New Confidence in }H_1}{\text{New Confidence in }H_2} &= \frac{\text{Old Confidence in }H_1}{\text{Old Confidence in }H_2} \cdot \frac{\text{How Likely the Result was Under }H_1}{\text{How Likely the Result was Under }H_2} \\
&= \frac{P(H_1)}{P(H_2)} \cdot \frac{P(\langle \text{Result} \rangle | H_1)}{P(\langle \text{Result} \rangle | H_2)}
\end{aligned}
\end{equation*}

Hence the hindsight ratio $\frac{P(\langle \text{Result} \rangle | H_1)}{P(\langle \text{Result} \rangle | H_2)}$ becomes the expression of evidence for/against $H_1$ relative to $H_2$.

% Let ($\Omega_e, \mathcal{F}_e, P_e$) be a probability space with events $N, \bar{N} \in \mathcal{F}$ being events representing a null hypothesis being true/false respectively. If the alternative hypothesis leaves probabilities undefined - as is usually the case - then $P_e$ itself will be undefined. However, we can consider two other probability spaces, ($\Omega_e, \mathcal{F}_e, P_{e,N}$) and ($\Omega_e, \mathcal{F}_e, P_{e,\bar{N}}$) where $P_{e,N}(E) = P_e(E | N)$ and $P_{e,\bar{N}}(E) = P_e(E | \bar{N})$. Then we find that $P_{e,N}$ is (usually) fully defined, while $P_{e,\bar{N}}$ is not.

\subsection{Application}

Given the limited techniques in this paper, we cannot directly obtain a hindsight ratio in the context of single hypothesis testing. Rather, we can obtain a \emph{bound} on the hindsight ratio \emph{in some cases}. In particular, consider a random variable $R$ which represents an experimental result, where $R$ takes on some value from the set $S_R$. We can directly obtain the hindsight probability under the null hypothesis as $P(\langle R = r \rangle\ |\ N) = P(R = r\ |\ N)$ because probabilities under the null hypothesis (i.e. $P(\cdot | N)$) are fully defined. Then, ideally, we can \emph{lower-bound} the hindsight probability for the alternative hypothesis. At the moment, given the techniques in this paper, we can only lower-bound $P(\langle R = r \rangle\ |\ \bar{N})$ when the alternative hypothesis meets the criterion for the bound in Section~\ref{sec:combined_lower_bound}. When those criterion are met, we obtain that:

\begin{equation}\label{eqn:our_hindsight_ratio_bound}
\text{Strength of Evidence Against the Null } = \frac{P(\langle R = r \rangle | \bar{N})}{P(\langle R = r \rangle | N)} \geq \frac{\frac{1}{|S_R|}}{P(R = r | N)}
\end{equation}

Thus, for \emph{some} alternative hypotheses, we have a way to obtain a lower bound on the strength of evidence an experimental result provides against the null hypothesis, all based on reasoning about undefined probability functions - no prior probability assumptions needed. We now revisit our discussion from Section~\ref{sec:combined_lower_bound} to see when this bound on the hindsight ratio applies and what limitations this presents for hypothesis testing.

\subsection{Limitations}\label{sec:limitations}

We begin this section by re-iterating the criterion for using Equation~\ref{eqn:our_hindsight_ratio_bound} as a lower-bound on statistical evidence. We then proceed to discuss what this means practically for testing.

Let $(\Omega_f, \mathcal{F}_f, P_f)$ be a probability space where two events $N, \bar{N}$ represent the null hypothesis being true/false respectively; $\bar{N} = \Omega_f \setminus N$. We can think of $P_f(\cdot | N)$ and $P_f(\cdot | \bar{N})$ as distinct probability functions, each with their own set of possible values, $\mathcal{V}(P_f(\cdot | N))$ and $\mathcal{V}(P_f(\cdot | \bar{N}))$. Let $X_f$ be a random variable representing our experimental result, where $X_f$ takes on a value from the set $S_{X_f}$; that is, $S_{X_f} = \{v\ |\ \exists \omega \in \Omega_f.\ X_f(\omega) = v\}$. We can use Equation~\ref{eqn:our_hindsight_ratio_bound} when the following criterion are met:

\begin{enumerate}
    \item $P_f(\cdot | N)$ is fully defined.
    \item $\mathcal{V}(P_f(\cdot | \bar{N}))$ contains all and only distinct probability functions with respect to $X_f$. That is:
    \begin{enumerate}
        \item All: $\forall P'.\ \left( (\Omega_f, \mathcal{F}_f, P') \text{ is a probability space with } P'(\bar{N}) = 1\right)$ $\rightarrow$\\ $\left(\exists P'' \in \mathcal{V}(P_f(\cdot | \bar{N})).\ \forall x \in S_{X_f}.\ P'(X_f = x) = P''(X_f = x) \right)$
        \item Only: $\forall P_1, P_2 \in \mathcal{V}(P_f(\cdot | \bar{N})).\ \left( P_1 \neq P_2 \rightarrow \left( \exists x \in S_{X_f}.\ P_1(X_f = x) \neq P_2(X_f = x). \right) \right)$
    \end{enumerate}
\end{enumerate}

Technically, these constraints could be a little looser. However, these are typically the relevant constraints.

Practically, what this means is that the hypothesis tester cannot constrain the space of possible alternatives to the null hypothesis. Thus, for example, if the experimenter is flipping a coin and testing for evidence against 50-50 randomness, the experimenter cannot use our bound while constraining the space of hypotheses to be binomial hypotheses. The alternative hypothesis must allow for \emph{every} possible distribution over the result variable $X_f$ (including the null distribution!); the alternative hypothesis must be what we call ``completely agnostic'' with respect to $X_f$.

To continue with a coin-flipping example, this means that if the experimenter wishes to test for 50-50 randomness, they must take great care in defining the probability space and result variable $X_f$. If they define the result variable $X_f$ to represent the full sequence of coin flips, then the alternative hypothesis must include all (and only) distinct probability distributions over coin flip sequences - not just hypotheses which assume independent flips. Similarly, if the experimenter wishes to define $X_f$ as the number of heads tossed, then the alternative hypothesis must include all (and only) distinct probability distributions over the number of heads. This does not always make conceptual sense. Thus, applying the techniques provided in this paper will not always make conceptual sense, and consequently the techniques simply \emph{should not be used} in many cases.

We continue our discussion of proper use of our bound in the next section. We also note that some of these limitations are not due to the concept of a hindsight probability but rather due to our current techniques for reasoning about repeat/hindsight probabilities. We hope and expect that there are more situations in which hindsight probabilities can be calculated in a well-defined manner, thereby opening up new lower-bounding opportunities via our generalized lower-bounding technique from Section~\ref{sec:confidence_bounding_principle}.


\section{Main Results}\label{sec:main_results}

\begin{figure}[b]
% The \phantomcaption allows for an invisible caption.
% \phantomcaption{}
\begin{tcolorbox}[colback=green!10!white,colframe=green!50!black,before upper={\parindent15pt},title=\textbf{The Monty Hallways Gameshow - Intro}]

Welcome! You are a contestant on the famous Monty Hallways Gameshow, a gameshow for statisticians to show their prowess. Today's episode is sponsored by the local dairies' ``Got half-and-half?'' campaign and the state's ``50-50 Entertainment-Learning'' initiative. If you pass all the challenges, you will win the prize collection of premium half-and-half products. Do you have what it takes?

\ 

(These story segments serve to illustrate the concepts presented in the paper.)
\end{tcolorbox}
\end{figure}

%This section contains our main contributions. Here we consider various kinds of ``meta'' reasoning one can do about confidences when one's confidences are not completely defined. In particular, we focus on a kind of confidence we call the ``hindsight'' or ``repeat'' confidence, which effectively represents how confident someone would be that an event would repeat if things could be done over again (or, perhaps more succinctly, how likely something seems to have been given hindsight).

This notion of a repeat confidence then enables us to suggest an alternative way of quantifying statistical evidence, which we discuss beginning in Section~\ref{sec:hypothesis_testing}.

\subsection{Introducing Repeat (or ``Hindsight'') Confidences}\label{sec:introducting_repeat_hindsight}

\begin{definition}[Repeat/Hindsight Confidences]\label{def:hindsight}
Let $(\Omega, \mathcal{F}, P)$ be a probability space and $X$ be a random variable on that space where $X$ takes on a value from the set $S_X$. Let $P' \in \mathcal{V}(P)$ be some possible value for $P$ (thus $\mathcal{V}(P') = \mathcal{V}(P)$). Define a sampling process on an urn of colored balls with one color for each of the possible values for $X$. That is, consider $S_X$ to be the set of different colors. In this sampling process the proportion of each color $c \in S_X$ in the urn is determined by $P'(X = c)$. Imagine that an idealized agent observes some ball of color $c$. The agent's Repeat Confidence (aka Hindsight Confidence) for the event $X = c$, denoted as $P(\langle X = c \rangle)$, is the agent's confidence that if they sampled the urn a second time with replacement they would get the same color ball.
\end{definition}

This definition corresponds to ``how likely something seems to have been'' after observing it and ``how likely something seems to be to repeat'' if a process could be repeated with indeterminism. Given this definition, the agent's repeat confidences will depend on how defined/undefined $P$ is. For example, if $P$ is fully defined, then $|\mathcal{V}(P)| = 1$ and the hypothetical distribution $P'$ governing the hypothetical urn sampling is defined to be $P' = P$; in that case $P'(X = x)$ is defined for any random variable $X$ defined on the space, and the agent's repeat confidence $P(\langle X = x \rangle)$ will just be $P'(X = x) = P(X = x)$. If however $P$ is undefined, then the agent may use certain forms of ``meta'' reasoning to still obtain a hindsight confidence. We analyze some of the kinds of reasoning that can be done and thus obtain ways of getting hindsight confidences in certain situations.

This notion of a repeat confidence expressed in terms of repeated sampling from an urn is related to the work of Couso et. al. on different kinds of independence~\cite{couso2000survey}. In particular, our urn model used in defining repeat/hindsight confidence contains the kind of independence Couso et. al. refer to as ``Repitition Independence.''

\subsection{Warmup Example - Undefined Deterministic ``Distributions''}

Let $(\Omega_a = \{1, 2, 3, 4\}, \mathcal{F}_a = \mathcal{P}(\Omega_a), P_a)$ be a probability space where $P_a$ is defined to be an element of the set $\mathcal{V}(P_a) = \{(1:1, 2:0, 3:0, 4:0),$ $(1:0, 2:1, 3:0, 4:0),$ $(1:0, 2:0, 3:1, 4:0),$ $(1:0, 2:0, 3:0, 4:1)\}$ - where a four-tuple of $a:b$ pairs indicates a probability distribution which assigns probability $b$ to elementary event $\{a\}$.  That is, $P_a = (1:1, 2:0, 3:0, 4:0)$ means $P_a(\{1\}) = 1$ and $P_a(\{2, 3, 4\}) = 0$; $P_a = (1:0.25, 2:0.25, 3:0.25, 4:0.25)$ would be a uniform distribution over $\Omega_a$. Etc.

\begin{figure}[t]
% The \phantomcaption allows for an invisible caption.
% \phantomcaption{}\label{fig:first_story_task}
\begin{tcolorbox}[colback=green!10!white,colframe=green!50!black,before upper={\parindent15pt},title=\textbf{The Monty Hallways Gameshow - First Challenge}]
For your first challenge, you are brought into a long hallway. On each door is a number. The gameshow host tells you these numbers form a probability distribution over the doors. You are told that behind each door is a shelf stocked with a dairy product - a different dairy product for each door. A product will be sampled according to the probability distribution on the doors. The strange thing about this ``distribution'' is that all the doors have zeros except for one door, which has the number 1 on it. You quickly realize that this means the door with the 1 is the only door that can open, and thus whatever dairy product is associated with that door is the product you will see.

\

You are blindfolded while this ``sampling'' occurs. The sampling is surprisingly quiet. Perhaps it is the velvety carpet. Upon having your blindfold removed, you see a box of Harriet's Best Cream Cheese on the table in front of you. Your gameshow host asks you, ``How confident are you that if we sample this distribution again, we will get another box of Harriet's Best Cream Cheese?'' Using the reasoning described above, you confidently answer that you are 100\% confident. Easy. You are correct and proceed to the next challenge.
\end{tcolorbox}
\end{figure}

We define a simple random variable $X: \Omega \rightarrow \mathbbm{R}$ where $X(\omega) = \omega$. In this scenario, what is $P_a(\langle X = 3 \rangle)$? We represent this kind of question in story-form in the ``First Challenge'' segment of our Monty Hallways Gameshow extras. In the story, sampling a second time from the same underlying probability distribution depicted on the doors corresponds to sampling a second time from the hypothetical urn. The doors specify that \emph{one} of the products will be sampled 100\% of the time, but not which one. This is analogous to $\mathcal{V}(P_a)$ = $\{(1:1, 2:0, 3:0, 4:0), (1:0, 2:1, 3:0, 4:0), (1:0, 2:0, 3:1, 4:0), (1:0, 2:0, 3:0, 4:1)\}$.

To calculate $P_a(\langle X = 3 \rangle)$, we consider sampling from an urn with one of the distributions of colors contained in $\mathcal{V}(P_a)$. We note that whatever distribution is chosen, the urn will be composed of balls of entirely one color; we simply do not know which color. However, \emph{if} we observe the ``color'' 3 in the first urn sample, then we know that if we sample the urn again we shall get the same color. Thus our repeat/hindsight confidence is $P_a(\langle X = 3 \rangle) = 1$.

\subsection{One Kind of Hindsight - Numbered Doors in Hallways}\label{sec:numbered_doors_hindsight}

Let $(\Omega_b, \mathcal{F}_b, P_b)$ be a probability space, where $P_b \in \mathcal{V}(P_b)$ is undefined. Let $X_b$ be a random variable defined on the space where $X_b$ can take on a value from the set $S_{X_b}$. For any probability function $P_b' \in \mathcal{V}(P_b)$, define the multiset $M_{P_b'} = (C_{P_b'}, m_{P_b'})$ to be the multiset of probabilities that $P_b'$ ascribes to the possible values for $X_b$. The set $C_{P_b'} = \{p\ |\ \exists x \in S_{X_b}.\ P_b'(X_b = x) = p\}$ and $m_{P_b'}$ is the multiplicity function.

\begin{figure}[t]
% The \phantomcaption allows for an invisible caption.
% \phantomcaption{}\label{fig:first_story_task}
\begin{tcolorbox}[colback=green!10!white,colframe=green!50!black,before upper={\parindent15pt},title=\textbf{The Monty Hallways Gameshow - Second Challenge}]
For your second challenge, you are brought into another long hallway. Once again the doors have a probability distribution over them, but this time the distribution is non-trivial. Once again each door is associated with a unique dairy product. A product will be sampled according to the distribution. You are blindfolded while this sampling occurs. Upon having your blindfold removed, you see a gallon of Leonard's 2\% Milk on the table in front of you.

\

The gameshow host asks you, ``What is your confidence that if we repeat this process, you would see another gallon of Leonard's 2\% Milk?'' You are given a pencil and paper and proceed to write down the numbers on the doors. After some thinking, you come up with an answer. (See Section~\ref{sec:numbered_doors_hindsight} for mathematical details.) ``Well done! A true theorist!'' your host exclaims. ``On to the next hallway...''
\end{tcolorbox}
\end{figure}

For the kind of reasoning we do in this section, we need that the following three criterion to be met: the collection of probability values over $X_b$ is the same for all probability functions in $\mathcal{V}(P)$, all possible permutations of these probabilities over the values for $X_b$ are present, and none of the possible probability functions are identical with respect to $X_b$. We express these criterion formally as:

$$\text{1: } \forall P_{b_1}', P_{b_2}' \in \mathcal{V}(P_b).\ M_{P_{b_1}'} = M_{P_{b_2}'}.$$

$$\text{2: } \forall \text{ orderings } \precsim \text{ of } S_{X_b}.\ \exists P_b' \in \mathcal{V}(P_b).\ \forall x_1, x_2 \in S_{X_b}.\ x_1 \precsim x_2 \rightarrow P_b'(X_b = x_1) \leq P_b'(X_b = x_2).$$

$$\text{3: }\forall P_{b_1}', P_{b_2}' \in \mathcal{V}(P_b).\ \exists x \in S_{X_b}.\ P_{b_1}'(X_b = x) \neq P_{b_2}'(X_b = x).$$

If these criterion are met, then we can reason as follows. We can conclude from criterion 1 that \emph{no matter which} $P_b' \in \mathcal{V}(P_b)$ is chosen, the multiset of probabilities in the urn will be the same ($M_{P_b'}$). We simply will not know which probabilities are associated with which colors. Further, we know that any assignment of probabilities in $M_{P_b'}$ over the colors in the urn is possible (criterion 2). Lastly, we know that there are no ``duplicate'' possibilities for $P_b'$ which specify the same distribution of colors in the urn (criterion 3); thus we do not need to consider any one assignment of probabilities to colors to be special for occurring more often than the others.

WLOG call the color of the first ball we observe ``red.'' At this point, we do not know which probability is associated with the color red. However, we know that the chance we had of sampling red was one of the values in $M_{P_b'} = (C_{P_b'}, m_{P_b'})$. This is analogous to knowing the numbers on the doors but not the mapping between the doors and the products in the second challenge of the Monty Hallways Gameshow story. We can now reason that, ``Our confidence that the chance of drawing red was $c \in C_{P_b'}$ given that we observed red is $c \cdot m_{P_b'}$.'' Then we can express our confidence that we will draw red again as:

$$
\begin{aligned}
P_b(\text{Draw red again}) &= \sum_{c \in C_{P_b'} } P_b(\text{Draw red given chance of drawing red is }c) \\
 &\ \ \ \ \ \ \ \ \ \ \ \ \ \ \cdot P_b(\text{Chance of drawing red was }c\ given\ \text{Observed red}) \\
 &= \sum_{c \in C_{P_b'} } c \cdot c \cdot m_{P_b'}(c)
\end{aligned}
$$

Thus even though $P_b$ is undefined, we have the right kind of information about $P_b$ to do the above kind of meta reasoning and obtain a hindsight confidence:

$$P_b(\langle X = x \rangle) = \sum_{c \in C_{P_b'} } c^2 \cdot m_{P_b'}(c)$$

Note that our definition here applies to finite cases only. However, as far as we can tell, the reasoning contained in this section should naturally extend to the limiting case, and thus a continuous version of this kind of confidence should be obtainable via taking the limit (i.e. via an integral). We present a simple example of applying the result from this section before moving on to other ways to obtain hindsight confidences.

\subsubsection{A Simple Walkthrough Example}

As a simple example, consider the case where $\Omega_b = \{\omega_1, \omega_2, \omega_3, \omega_4\}$. We will express a probability distribution as a 4-tuple of probabilities for the elementary events. In our scenario, let $\mathcal{V}(P_b) = \{(0.2, 0.2, 0.4, 0.2), (0.2, 0.6, 0.1, 0.1), (0.6, 0.2, 0.05, 0.15)\}$. Consider the random variable $X_b$ to be defined such that $X_b(\omega_1) = 1$, $X_b(\omega_2) = 2$, and $X_b(\omega_3) = X_b(\omega_4) = 3$. In this case $S_{X_b} = \{1, 2, 3\}$. We find that no matter which of the three distributions are chosen from $\mathcal{V}(P_b)$, the collection of probabilities for the events $X_b = 1$, $X_b = 2$, and $X_b = 3$ will be the same: 0.2, 0.2, and 0.6. In one case it's 0.2 for $X_b = 1$, 0.2 for $X_b = 2$, and 0.4 + 0.2 = 0.6 for $X_b = 3$; in another it's 0.2 for $X_b = 1$, 0.6 for $X_b = 2$, and 0.1 + 0.1 = 0.2 for $X_b = 3$; in the last case it's 0.6 for $X_b = 1$, 0.2 for $X_b = 2$, and 0.05 + 0.15 = 0.2 for $X_b = 3$. Thus criterion 1 and 2 are met. We also find that there are no duplicate probability functions with respect to $X_b$; therefore criterion 3 is met and we can apply our equation.

Since this case meets the conditions, we can define the hindsight probabilities of the possible events involving $X_b$ to be $P(\langle X_b = 1 \rangle) = P(\langle X_b = 2 \rangle) = P(\langle X_b = 3 \rangle) = 0.2^2 \cdot 2 + 0.6^2 \cdot 1 = 0.4$.

Note that hindsight confidences do not typically form a probability distribution unless the original distribution is fully defined. In this example, the hindsight confidences sum to more than 1.

\subsection{The Confidence-Refinement Bounding Principle}\label{sec:confidence_bounding_principle}

So far, we have considered two ways to obtain a hindsight confidence. The first is when a probability function $P$ is fully defined; then the hindsight confidence for an event $E$ is just $P(\langle E \rangle) = P(E)$. The second way has more complex prerequisites, and thus can only be applied in some cases.

In this section we offer a principle that can be used to \emph{bound} hindsight confidences, regardless of whatever other ways a person can obtain a hindsight confidence. Recall that a hindsight confidence is defined to be what an idealized agent would conclude (see Definition~\ref{def:hindsight} for a reminder if need be). As of writing this paper, we are not aware of all the ways an idealized agent could perform meta-reasoning about probabilities in order to obtain a hindsight confidence; we only know what sort of reasoning such an agent would perform in certain situations. Ideally, we will eventually be able to offer a more generalized mathematical formalism for hindsight. However, even though we do not know exactly what an idealized agent would conclude in all cases, we can obtain \emph{bounds} on their hindsight confidences.

How do these bounds work? Our bounds operate by considering different kinds of information gains. Let $(\Omega_c, \mathcal{F}_c, P_c)$ be a probability space. Recall that $\mathcal{V}(P_c)$ contains the possible values for $P_c'$, the distribution governing the hypothetical urn sampling process. In other words, $\mathcal{V}(P_c)$ expresses the current constraints on what the urn's distribution might be. If, however, we received information which removed some elements from $\mathcal{V}(P_c)$, our confidences would be refined. We call the information that told us which elements to discard from $\mathcal{V}(P_c)$ ``refinement information.'' We can then consider the various ``kinds'' of refinement information. We define a ``kind of refinement information'' $K$ to be a partition of $\mathcal{V}(P_c)$. That is, a \emph{kind} of refinement information is equivalent to a collection of cells, where the information we get of that kind will tell us which cell to refine $\mathcal{V}(P_c)$ to.

Let $X_c : \Omega_c \rightarrow \mathbbm{R}$ be a random variable defined on our probability space, where $X_c$ takes on a value from the set $S_{X_c}$. Let $L : S_{X_c} \times \mathcal{P}(\mathcal{V}(P_c)) \rightarrow [0, 1]$ and $U: S_{X_c} \times \mathcal{P}(\mathcal{V}(P_c)) \rightarrow [0, 1]$ represent whatever techniques we have available to define upper and lower bounds on our repeat/hindsight confidence for the event $X_c = x \in S_{X_c}$ given a collection of possible confidences functions $C \subseteq \mathcal{V}(P_c)$ governing the urn sampling process (i.e. $C \in \mathcal{P}(\mathcal{V}(P_c))$). Let $\mathcal{K}(\mathcal{V}(P_c))$ denote all the non-trivial partitions of $\mathcal{V}(P_c)$ (i.e. all the kinds of confidence refinement information). Then we can upper- and lower-bound our hindsight confidence as:

\begin{equation}\label{eqn:bounding_principle}
\max_{K \in \mathcal{K}(\mathcal{V}(P_c))} \left\{ \min_{C \in K} \left\{ L(x, C) \right\} \right\} \leq P_c(\langle X_c = x \rangle) \leq \min_{K \in \mathcal{K}(\mathcal{V}(P_c))} \left\{ \max_{C \in K} \left\{ U(x, C) \right\} \right\}
\end{equation}

What does this bound represent conceptually? It means that if we think of some \emph{kind} of information refinement $K$ where for each different information refinement associated with that kind (i.e. each different cell $C \in K$), our hindsight confidence is lower-/upper-bounded by $\alpha$, then we can lower-/upper-bound our overall hindsight confidence by $\alpha$.

This principle sounds more obvious when an analogy is used: Imagine you can learn one piece of information about Jones - his age, height, or weight; these three represent different kinds of confidence refinements. Further, imagine that regardless of which age Jones is, upon learning his age you can calculate his income. If, for every age, your calculation comes out to be at least \$10 a month, then you can lower-bound Jones' income by \$10 a month even without knowing his age.

\subsection{Combining These Results}\label{sec:combined_lower_bound}

In Section~\ref{sec:numbered_doors_hindsight} we discussed a way to calculate a repeat confidence when certain conditions were met. Then in Section~\ref{sec:confidence_bounding_principle} we discussed a fully general method to take whatever specific, situational techniques we have and use them to obtain lower- or upper-bounds on our hindsight confidence. In the worst case, these bounds are trivial, a lower bound of zero and an upper bound of 1. However, sometimes we can do better. In this section we explore cases where the technique in Section~\ref{sec:numbered_doors_hindsight} can combine with the principle in Section~\ref{sec:confidence_bounding_principle}.

Let $(\Omega_d, \mathcal{F}_d, P_d)$ be a probability space where $P_d \in \mathcal{V}(P_d)$. Let $X_d$ be a random variable defined on that space, where $X_d$ takes on a value from the set $S_{X_d}$. Let $L_d : S_{X_d} \times \mathcal{P}(\mathcal{V}(P)) \rightarrow [0, 1]$ and $U_d : S_{X_d} \times \mathcal{P}(\mathcal{V}(P)) \rightarrow [0, 1]$ represent the technique we have available from Section~\ref{sec:numbered_doors_hindsight} for upper- and lower-bounding confidences. That is, given a value $x \in S_{X_d}$ and collection $C \subseteq \mathcal{V}(P_d)$ of possible probability distributions for the hypothetical urn, $L_d$ and $U_d$ are defined as:

\begin{equation*}
L_d(x, C) = \begin{cases}
\text{Calculation from Section~\ref{sec:numbered_doors_hindsight}. } & \text{ if }C\text{ meets the criterion with respect to }X_d \\
0\ & \text{ otherwise}
\end{cases}
\end{equation*}

\begin{equation*}
U_d(x, C) = \begin{cases}
\text{Calculation from Section~\ref{sec:numbered_doors_hindsight}. } & \text{ if }C\text{ meets the criterion with respect to }X_d \\
1\ & \text{ otherwise}
\end{cases}
\end{equation*}

Basically, $L_d$ and $U_d$ perform the calculation from Section~\ref{sec:numbered_doors_hindsight} if it applies and otherwise provide the trivial lower-/upper-bound of 0/1. Let $\mathcal{K}(\mathcal{V}(P_d))$ be the set of all non-trivial partitions of $\mathcal{V}(P_d)$, and let $x$ be any value $X_d$ can take on (i.e. $x \in S_{X_d}$). Recall that:

$$
\max_{K \in \mathcal{K}(\mathcal{V}(P_d))} \left\{ \min_{C \in K} \left\{ L_d(x, C) \right\} \right\} \leq P_d(\langle X_d = x \rangle) \leq \min_{K \in \mathcal{K}(\mathcal{V}(P_d))} \left\{ \max_{C \in K} \left\{ U_d(x, C) \right\} \right\}
$$

\begin{figure}[t]
% The \phantomcaption allows for an invisible caption.
% \phantomcaption{}\label{fig:second_story_task}
\begin{tcolorbox}[colback=green!10!white,colframe=green!50!black,before upper={\parindent15pt},title=\textbf{The Monty Hallways Gameshow - Third Challenge}]
For your third and final challenge, you are once again brought into a long hallway. This time the doors are completely blank. Your host assures you that each door corresponds to a unique dairy product and that there is a probability distribution over the doors; the probabilities are hidden. The collection of relevant dairy products is pictured on one of the walls. Before anything occurs, the host points at the image of Dillard's Half-and-Half, asking, ``What is your confidence you'll see Dillard's come from a door in this hallway?''

You reply, ``Well, my confidence is rather undefined at the moment.''

``Of course! Of course!'' says your energetic host, ``How about a minimum confidence?''

``A minimum confidence? Is that like a lower bound on my confidence?''

``Indeed.''

``I'm afraid I cannot lower-bound my confidence above zero.'' you say.

``Well done! You're properly cautious. Now for the big question...''

You are temporarily blindfolded while the distribution is sampled; when un-blindfolded, you see a stick of Pleasant Valley butter. The gameshow host says, ``Tell me, what is your minimum confidence that if this process were to be repeated, the product would be Pleasant Valley butter again?'' Your brow furrows. You spend a while in thought and then come up with an answer: 1 over the number of doors. ``Wonderful!'' exclaims the host, ``Someone get this winner their half-n-half!''

\ 

(The math behind this case is presented in Section~\ref{sec:combined_lower_bound}.)
\end{tcolorbox}
\end{figure}

\emph{If} $\mathcal{V}(P_d)$ contains all (and only) distinct probability functions with respect to $X_d$, then we can define a partition $K$ of $\mathcal{V}(P_d)$ that allows us to obtain a lower bound on hindsight confidences involving $X_d$. In particular, consider the partition $K \in K(\mathcal{V}(P_d))$ where every cell $C \in K$ has all and only the probability functions which yeild the same multiset of probabilities over the events $X_d = x.$ for $x \in S_{X_d}$. For any cell $C \in K$, label the multiset of probabilities for $X_d$ associated with $C$ as $M_{X_d,C} = (S_{X_d, C}, m_{X_d, C})$. Then we get that for any value $x$ that $X_d$ can take on:

$$\min_{C' \in K} \left\{ \sum_{p \in S_{X_d, C'}} p^2 \cdot m_{X_d, C'}(p) \right\} \leq P_d(\langle X_d = x \rangle) \leq \max_{C' \in K} \left\{ \sum_{p \in S_{X_d, C'}} p^2 \cdot m_{C'}(p) \right\}$$

Solving for the min and max yeilds that $\frac{1}{|S_{X_d}|} \leq P_d(\langle X_d = x \rangle) \leq 1$. Consequently, while $P_d(X_d = x)$ is completely undefined, our hindsight confidence for $X_d = x$ is at least $\frac{1}{|S_{X_d}|}$.

Note that if $P_d$ was more precisely defined, $\mathcal{V}(P_d)$ will have fewer values, and we might not be able to partition $\mathcal{V}(P_d)$ into cells which all meet the requirements in order to apply the calculation from Section~\ref{sec:numbered_doors_hindsight}. Thus, we cannot always obtain that $P_d(\langle X_d = x \rangle) \geq \frac{1}{|S_{X_d}|}$. One trivial example of this fact is when $|\mathcal{V}(P)| = 1$ (i.e. when $P_d$ is fully defined); then there is no room or need for meta-reasoning: then $P_d(\langle X_d = x \rangle) = P_d(X_d = x)$, and $P_d(X_d = x)$ could be less than $\frac{1}{|S_{X_d}|}$.

This kind of reasoning is analogous to the reasoning used in the third challenge of the Monty Hallways Gameshow story. In the \emph{second} challenge of the story, you were able to use the numbers on the doors as the multiset of probabilities needed for the calculation in Section~\ref{sec:numbered_doors_hindsight}. In the \emph{third} challenge, you did not even know the numbers on the doors; you knew absolutely nothing about the distribution over the dairy products (the distribution over $X_d$). Thus you were able to consider the \emph{kind} of information gain corresponding to the partitioning of possible distributions into the possible multisets of probabilities. That is, you could consider partitioning over the possible number arrangements on doors. Under this partition, you found that no matter which multiset of probabilities the doors were labeled with, your hindsight confidence would come out to be at least one over the number of doors (1 over $|S_{X_d}|$).

\section{Philosophical Intro Excerpts}

Probabilistic models of beliefs and confidences tend to be Bayesian. Bayesian statistical methods assume that agents have precise probability assignments. That is, they assume that agents assign exact confidences concerning every event/parameter being considered. Peter Walley refers to this as ``the Bayesian dogma of precision,''~\cite{walley1991statistical} stating:

\begin{blockquote}
A central assumption of the Bayesian theory is that uncertainty should always be measured by a single (additive) probability measure, and values should always be measured by a precise utility function. This assumption will be called the \textbf{Bayesian dogma of precision}.
\end{blockquote} % From page 3 of his book. Page 241 has further discussion.

Walley's work, along with the work of many others, helps to explain why modeling an agent's confidences with precise probabilities is insufficient to handle various kinds of uncertainty. We provide just two examples in this introduction:

\begin{itemize}
    \item Under the dogma of precision, one cannot distinguish between degrees of epistemic uncertainty about underlying frequencies (i.e. different ``epistemic probabilities'' about ``aleatory probabilities''). For example, consider flipping a coin. Rigorous evidence that the coin is being flipped fairly would lead to a well-informed confidence of $\frac{1}{2}$ that the next flip will be a heads. However, if we have no evidence the coin will be tossed fairly and are very uncertain about the chance it will flip heads, we would likely still choose a confidence of $\frac{1}{2}$ to represent our ignorance. These numbers are identical yet they represent very different kinds of confidences. As Walley expresses it, ``Imprecision in probabilities is needed to reflect the amount of information on which they are based.''~\cite{walley1991statistical}
    \item Requiring precise probabilities means requiring precise priors. These priors are often insufficiently motivated. Some have suggested the use of ``uninformative priors,'' such as the Jefferys prior or the max-entropy prior~\cite{jeffreys1998theory, jaynes1957information, jaynes1982rationale, price2002uninformative}. However, even ``uninformative priors'' for model parameters actually carry significant information~\cite{walley1991statistical}. For example they are not ``uninformative'' under reparametrization~\cite{walley1991statistical, lemoine2019moving}.
\end{itemize}

While more criticisms could be raised, we proceed to the fact that people have developed powerful, imprecise alternatives. One alternative is to work with upper and lower bounds on confidences~\cite{walley1991statistical, walley2000towards}; in this case confidences are effectively intervals - the smaller the interval the more precise the confidence. Another, more general alternative is to use \emph{sets} of probability functions rather than a single (and therefore precise) probability distribution~\cite{kyburg1977randomness, levi1975indeterminate, joyce2010defense, bradley2019imprecise}. In this paper we focus on this last option; we model uncertainty via a \emph{set} of probability functions rather than a single probability function.

When modeling imprecise confidences via a set of probability functions, two important questions arise:

\begin{itemize}
    \item \textbf{Question 1:} Upon observing an event $E$, how should we update our confidences?
    \item \textbf{Question 2:} What \emph{evidence} does an event $E$ provide about a hypothesis $H$?
\end{itemize}

These two questions are related but distinct. They both have fairly straightforward ``answers'' in Bayesian statistics - use Bayes' rule and the likelihood ratio (with ``uninformative priors'') for questions 1 and 2 respectively. However, as we have already mentioned, Bayesian statistics suffers from issues which imprecise probabilities address.

We do not answer questions 1 or 2 in entirety. Rather, we provide answers for particular cases which we expect can be generalized to a full theory someday. The crucial insight of our paper is the following: Given a set $\mathcal{C}$ of probability functions which represents our confidences, observing an event $E$ \emph{not only} tells us what each individual probability function in $\mathcal{C}$ says conditioned on $E$; observing $E$ \emph{also tells us} which probability functions within $\mathcal{C}$ served as better models of what happened - thereby telling us which elements of $\mathcal{C}$ we should favor in the future. We formalize this idea more in Section~\ref{sec:main_results}.

In effect, this paper accomplishes three things:

\begin{enumerate}
    \item We consider repeated sampling from an urn and thereby reveal an issue with the ``Confirmational Conditionalization'' method for updating imprecise confidences~\cite{levi1975indeterminate, joyce2010defense}.
    \item We use the ``crucial insight'' mentioned above to provide an alternative, ``meta'' way to reason with imprecise confidences which illuminates information not considered during the process of confirmational conditionalization.
    \item We develop this extra information into a promising basis for upper- and lower-bounding the evidence that observing an event provides about a \emph{single} hypothesis - something previously argued impossible by excellent theorists such as Royall~\cite{royall1997statistical}.
\end{enumerate}

Along the way, our analysis also suggests a solution to the ``problem'' of dilation~\cite{seidenfeld1993dilation}.

\section{Pre-Imprecise Intro Excerpts}

You know that $P$ is a probability function on a random variable $X$, where $X$ can take on one of $n$ possible values. Thus you know that $P$ is always non-negative and sums to 1. That is all you know about $P$. Or is it? Can you reason about $P(X)$ to conclude anything meaningful? We argue that if $P$ is interpreted as a certain kind of confidence measure, then yes, there is much more of interest you can conclude. In this paper we open up a new way to think about probabilistic reasoning, and we focus on its application to single hypothesis testing.

---

In this paper we consider probabilities in both lights. Sometimes, we think of probabilities specifically as a kind of confidence where a confidence of $c$ that event $E$ will occur is a belief that $E$ has an inherent chance $c$ of occuring; we call these ``chance confidences.'' Other times, we consider probabilities as confidences more broadly; we call these ``full confidences.'' We elaborate more on this way of thinking in Section~\ref{sec:probs_as_confidences}. The reader does not necessarily need to think of probabilities in this fashion in order to find our results useful; however, we found this conception of probabilities to be the most natural one in which to reason about ``meta'' confidences - confidences about confidences.

---

we analyze what one can mathematically derive simply by asserting that you have a confidence function. That is all; no assumptions or definition of the confidence function required. In particular, we find that in lieu of defined confidence functions, we can sometimes derive \emph{bounds} on one's confidence about particular kinds of events. In the context of single hypothesis testing, our results contribute toward enabling someone to derive a lower bound on an experimental result's strength as evidence against the null, \emph{all without assuming any priors to parametrize the alternative hypothesis}.

To our knowledge, noone else has analyzed probability functions in the exact fashion that we do. The closest works we are aware of are the systems of Kyburg and Levi for representing epistemic states via \emph{sets} of probability functions~\cite{kyburg1977randomness, levi1975indeterminate}. We also represent undefined/imprecise confidences through sets of probability functions. However, we use these sets differently from both Kyburg and Levi. Overall, our approach is more akin to Kyburg's project than Levi's. Sometimes, when confidences are analyzed this way, a fascinating phenomenon called ``Dilation'' occurs; Seidenfeld and Wasserman have done an in-depth analysis on dilation \cite{seidenfeld1993dilation}. While dilation is not immediately relevant to this paper, we believe that the kind of reasoning we do in this paper can be extended to analyze dilation cases. More recently, people such as Joyce have defended the usefulness of the sets-of-probability-functions model for analyzing imprecise (``undefined'') confidences over and against other methodologies~\cite{joyce2010defense}. \textbf{TODO: Read Bradley's Summary \cite{bradley2019imprecise}} \textbf{-- TODO: Check out who also cites Joyce}

In this work we consider bounds on confidences one can obtain via analyzing vague/undefined probabilities. The idea of bounds on probabilities is well established. The work of Peter Walley on ``imprecise probabilities'' is an excellent specimen of working with upper and lower probability bounds rather than single precise probabilities~\cite{walley1991statistical, walley2000towards}. In this paper we explore what we believe to be new ways to obtain such bounds.

\section{Second Question for Dan}

I want to sample an element ``uniformly'' from the set of all probability functions over $n$ discrete elements. This corresponds to selecting a point from the unit simplex. For more discussion, see \href{https://cs.stackexchange.com/questions/3227/uniform-sampling-from-a-simplex}{https://cs.stackexchange.com/questions/3227/uniform-sampling-from-a-simplex}.

However, the algorithms I am aware of for sampling ``uniformly'' from the simplex are uniform across the space \emph{with respect to the L2 distance metric}. I want to sample uniformly with respect to the L1 distance metric. Questions:

\begin{enumerate}
    \item Do you know how (or if) L1 would change things?
    \item Do you know of keywords I should search?
\end{enumerate}


\section{First Question for Dan}

Let the set $\Omega$ be our sample space and  $\sigma$-algebra $\mathcal{F}$ over $\Omega$ be our event space. Let $\mathcal{P}^1$ be some set of probability functions, where ``$\forall P^1 \in \mathcal{P}^1.\ (\Omega, \mathcal{F}, P^1)$ is a probability space.''

Let $\mathcal{P}^2$ be the set of \emph{all} probability functions over $\mathcal{P}^1$. That is to say:

$$\mathcal{P}^2 = \{P^2\ |\ (\mathcal{P}^1, 2^{\mathcal{P}^1}, P^2) \text{ is a probability space}\}$$

We can note that any $P^2 \in \mathcal{P}^2$ implicitly defines a probability function over $\mathcal{F}$, where:

$$\forall E \in \mathcal{F}.\ P^2(E) \text{ ``=''} \int_{\mathcal{P}^1} P(E)\ P^2(P) \ dP$$

We can generalize this to $\mathcal{P}^i$ where for all $i > 1$:

$$\mathcal{P}^i = \{P^i\ |\ (\mathcal{P}^{i-1}, 2^{\mathcal{P}^{i-1}}, P^i) \text{ is a probability space}\}$$

and:

$$\forall E \in \mathcal{F}.\ P^i(E) \text{ ``=''} \int_{\mathcal{P}^{i-1}} P(E)\ P^i(P) \ dP$$

Let $P^* \in \mathcal{P}^2$ be the uniform distribution over $\mathcal{P}^1$.

Now for the question(s): Is the following true/false for a rigorous definition of ``almost all,'' and if so what is a proof?

$$\text{As }i \rightarrow \infty, \text{ for ``\emph{almost all}'' } P^i \in \mathcal{P}^i \text{ we get that } \forall E \in \mathcal{F}.\ P^i(E) = P^*(E).$$

\section{Explanation that you can always have elementary events}

Let $(\Omega, \mathcal{F}, P)$ be a probability space. Without loss of generality (``WLOG''), we assume that all the elementary events ($\{\omega\}$ where $\omega \in \Omega$) are in our event space $\mathcal{F}$. This is WLOG because any probability space has a mathematically equivalent probability space wherein elements $\omega_1, \omega_2$ of $\Omega$ that are always found together (i.e. $\forall E \in \mathcal{F}.\ \omega_1 \in E \leftrightarrow \omega_2 \in E$) can be merged into a single element, and because probabilities for unions of events in $\mathcal{F}$ entail probabilities for intersections: $P(A \cup B) = P(A) + P(B) - P(A \cap B)$. From here through the rest of the paper, we assume that all the elementary events are in an event space.

Further, because $P(A \cap B) = \emptyset$ when $A$ and $B$ are elementary events, fixing the probabilities $P$ assigns to the elementary events fixes the probabilities $P$ assigns to all the events in the event space. Thus, in this paper we can represent a probability function by stating what probabilities it assigns to the elementary events. Lastly, when $\mathcal{F}$ contains all the elementary events, $\mathcal{F}$ is the power set of $\Omega$, which we write as $\mathcal{F} = \mathcal{P}(\Omega)$.

\section{``Chance Confidences''}

\begin{definition}[Confidence]
A ``Confidence'' is a quantification of how strongly an agent believes some proposition $p$ (e.g. that an event $E$ will/has occurr(ed)).
\end{definition}

\begin{definition}[Chance Confidence]\label{def:chance_confidence}
A ``Chance Confidence'' is a particular kind of confidence. A chance confidence is an agent's belief that some event $E$ has/had a chance $c$ of occurring, where that chance is understood to be inherently probabilistic (i.e. non-deterministic and obeying a probability distribution function $P$ that specifies $P(E) = c$).
\end{definition}

Given this definition, when interpreted as a chance confidence, ``$P(E) = c$'' means \emph{both} that, ``You are $c$ confident that $E$ will/has occur(ed).'' and that, ``You believe $E$ has/had an inherently probabilistic chance $c$ of occuring.''

\section{Isomorphisms incl. Believed Isomorphism}

\subsection{Isomorphic Probability Spaces}\label{sec:isomorphic_spaces}

We use the notion of isomorphic probability spaces for some of our analysis, so we review the concept here and extend it to probability spaces with undefined probability functions. The notion of isomorphic probability spaces helps us to consider reasoning about a single probability space in terms of two ``equivalent'' spaces.

Let $(\Omega_1, \mathcal{F}_1, P_1)$ and $(\Omega_2, \mathcal{F}_2, P_2)$ be probability spaces. $(\Omega_1, \mathcal{F}_1, P_1)$ and $(\Omega_2, \mathcal{F}_2, P_2)$ are ``Isomorphic'' if there exists a bijection $f: \Omega_1 \rightarrow \Omega_2$ such that $E_1 \in \mathcal{F}_1 \leftrightarrow f(E_1) \in \mathcal{F}_2$ and $\forall E_1 \in \mathcal{F}_1.\ P_1(E_1) = P_2(f(E_1))$.

In other words, probability spaces are isomorphic when there's a way of looking at them such that there's a one-to-one correspondence between the (event, probability) pairs in the two spaces.

When we allow probability spaces to have probability measures which are undefined (i.e. $P_1 \in \mathcal{V}(P_1)$ and $P_2 \in \mathcal{V}(P_2)$), then our definition of an isomorphism changes slightly and we actually get two kinds of isomorphism.

\begin{definition}[Isomorphism]\label{def:isomorphism}
Two probability spaces $(\Omega_1, \mathcal{F}_1, P_1)$ and $(\Omega_2, \mathcal{F}_2, P_2)$ have an ``Isomorphism'' (i.e. are isomorphic) if there exist bijections $f: \Omega_1 \rightarrow \Omega_2$ and $g: \mathcal{V}(P_1) \rightarrow \mathcal{V}(P_2)$ such that $E_1 \in \mathcal{F}_1 \leftrightarrow f(E_1) \in \mathcal{F}_2$, and:

$$\forall P_1' \in \mathcal{V}(P_1).\ \forall E_1 \in \mathcal{F}_1.\ P_1'(E_1) = g(P_1')(f(E_1))$$
\end{definition}

This definition collapses to the standard definition of an isomorphism when the probability functions are fully defined (i.e. when $|\mathcal{V}(P_1)| = |\mathcal{V}(P_2)| = 1$). In addition to this definition, we define a stronger kind of isomorphism, the ``believed isomorphism'' as follows:

\begin{definition}[Believed Isomorphism]\label{def:believed_isomorphism}
Two probability spaces $(\Omega_1, \mathcal{F}_1, P_1)$ and $(\Omega_2, \mathcal{F}_2, P_2)$ have a ``Believed Isomorphism'' if they have an isomorphism defined by functions $f: \Omega_1 \rightarrow \Omega_2, g: \mathcal{V}(P_1) \rightarrow \mathcal{V}(P_2)$ and if for that isomorphism $P_1(E)$ is defined to be equal to $P_2(f(E))$ for all $E \in \mathcal{F}_1$.
\end{definition}

In a \emph{believed} isomorphism, an agent has defined their confidences over the two spaces to be linked. That is, the agent believes $E \in \mathcal{F}_1$ is as likely as $f(E) \in \mathcal{F}_2$ to occur \emph{even if} the agent has not fully defined their confidence $P_1(E)$. When an agent has a believed isomorphism between spaces, they may be able to use what occurs in one space as a way to refine their confidences about the second space; that is the chief idea we explore later in this paper.

Mathematically, when $(\Omega_1, \mathcal{F}_1, P_1)$ and $(\Omega_2, \mathcal{F}_2, P_2)$ have a believed isomorphism $f, g$, then $\mathcal{V}(P_1)$ is not equivalent with the definition of $P_1$. Rather, $\mathcal{V}(P_1)$ contains all the values $P_1$ could have, but the full definition of $P_1$ is that $(P_1, P_2) \in \mathcal{V}((P_1, P_2)) = \{(h_1, g(h_1))\ |\ h_1 \in \mathcal{V}(P_1)\}$.

With these background concepts established, we can now turn to our main considerations.

\section{Introducing Repeat (or ``Hindsight'') Confidences In Terms of Believed Isomorphism}

\begin{definition}[Repeat/Hindsight Confidences]\label{def:repeat_hindsight_v2}
Let $S_1 = (\Omega_1, \mathcal{F}_1, P_1)$ and $S_2 = (\Omega_2, \mathcal{F}_2, P_2)$ be probability spaces an agent has about two phenomenon, where the confidences over the spaces are interpreted as chance confidences (see Definition~\ref{def:chance_confidence}). In particular, consider the agent to have a believed isomorphism $f: \Omega_1 \rightarrow \Omega_2$ and $g : \mathcal{V}(P_1) \rightarrow \mathcal{V}(P_2)$ (see Definition~\ref{def:believed_isomorphism}) between the probability spaces. For any event $E \in \mathcal{F}_1$, the agent's ``Repeat Confidence'' (or ``Hindsight Confidence'') is denoted as ``$P_1(\langle E \rangle)$'' and is defined to be how confident the agent will be that $f(E) \in \mathcal{F}_2$ will occur in the second probability space if they observed $E$ in the first probability space.
\end{definition}

This definition corresponds to ``how likely something seems to have been'' after observing it and ``how likely something seems to be to repeat'' if a process could be repeated with indeterminism. For example, if you were to sample colored balls from an urn with replacement and represented the first and second sampling as believed-isomorphic probability spaces, then a repeat/hindsight confidence for the color red would represent how confident you are that you will sample a red ball the second time \emph{if} you sampled a red ball the first time.

Given this definition, the agent's repeat confidences will depend on how defined/undefined $P_1$ is. For example, if $P_1$ is fully defined, then $P_1(E_1)$ is defined for any event $E_1 \in \mathcal{F}_1$, and the agent's repeat confidence $P_1(\langle E_1 \rangle)$ will just be $P_1(E_1) = P_2(f(E_1))$. If however $P_1$ is undefined, then the agent may use certain forms of ``meta'' reasoning to still obtain a hindsight confidence. We analyze some of the kinds of reasoning that can be done and thus obtain ways of getting hindsight confidences in certain situations.

Importantly, we note that the second probability space can be purely conceptual. We can still consider a hindsight confidence when working with only one probability space by mathematically considering an isomorphic space.

\section{Failed Attempt at Hindsight Definition}

\begin{definition}[Repeat/Hindsight Confidences Formulation 1]\label{def:repeat_hindsight_v1}
Let $(\Omega_1, \mathcal{F}_1, P_1)$ and $(\Omega_2, \mathcal{F}_2, P_2)$ be isomorphic probability spaces with the isomorphism function $f: \Omega_1 \rightarrow \Omega_2$ (and $g : \mathcal{V}(P_1) \rightarrow \mathcal{V}(P_2)$ if the probability functions are undefined). Let $E_1 \in \mathcal{F}_1$ be an event and $E_2 = f(E_1) \in \mathcal{F}_2$. The ``Repeat Confidence'' (or ``Hindsight Confidence'') for $E_1$ and $E_2$, denoted as ``$P_1(\langle E_1 \rangle)$'' or ``$P_2(\langle E_2 \rangle)$,'' represents how confident the agent would be that $E_2$ will/has occur(ed) in the second probability space given that the agent had the confidences defined by $P_1$ over $\mathcal{F}_1$, the confidences defined by $P_2$ over $\mathcal{F}_2$, \emph{and} the agent has observed $E_1$ in the first probability space.
\end{definition}

\section{Discussing Idea of Conditionals}

Later in the paper, we provide a new mathematical definition of conditional probabilities. To understand some of the intuition behind we would off a redifinition, we talk in this section about what conditional probabilities represent. When probabilities represent confidences, we can think of conditional confidences in the following two ways:

\begin{itemize}
    \item \textbf{The Anticipatory Conditional: } Here $P(A | B)$ is understood to mean a confidence about what will/has happen(ed) if something else will/has happen(ed). That is, $P(A | B) = p$ means, ``I am $p$ confident that if $B$ will/has occur(ed), then $A$ will/has occur(ed).''
    \item \textbf{The Confidence Update Conditional: } Here $P(A | B)$ is understood to mean what a confidence will change to upon being given new information. That is, $P(A | B) = p$ means, ``In my current epistemic state I am $P(A)$ confident that $A$ will/has occur(ed). However, if I observe event $B$, then my confidence that $A$ will/has occur(ed) changes to $p$.''
\end{itemize}

We believe these two conceptual understandings to be mathematically equivalent. Both can be helpful ways of understanding conditionals.

The standard probability axioms (the Kolmogorov axioms) do not explicitly define conditional probabilities. A conditional probability $P(A | B)$ is usually defined to be shorthand for the quantity $\frac{P(A \cap B)}{P(B)}$. When probability functions are fully defined, this mathematical definition perfectly corresponds to the concepts of a conditional probability we discussed. \emph{However, } when you allow probability functions to be undefined in certain ways, this mathematical definition and the concepts begin to come apart. At a high level, this coming-apart occurs because when a probability function $P$ is undefined in certain ways, observing an event $B$ allows you to think in a ``meta'' way about ``what your confidence is that $P(B)$ was a specific confidence.''

We present a new mathematical definition of conditional probabilities - a definition which equals the standard definition when probability functions are fully defined, but which behaves in a more conceptually proper way when probability functions are undefined. This new definition is detailed beginning in Section~\ref{sec:defining_conditionals}

\section{Idea of ``Effectively Elementary Events''}

Any ``singleton'' event $\{\omega\} \in \mathcal{F}$ where $\omega \in \Omega$ is also referred to as an ``elementary event.'' In this paper we only work with events which are ``effectively'' elementary events. In the future, we hope to generalize our definitions to apply to all events in $\mathcal{F}$. \textbf{CHECK BACK} We define an ``effectively elementary'' event as follows:

\textbf{DO I ACTUALLY NEED THIS BIT ABOUT ``EFFECTIVELY ELEMENTARY'' EVENTS?}

\begin{definition}[Effectively Elementary Event]
Let $E \in \mathcal{F}$ be an event. Then $E$ is considered to be ``Effectively Elementary'' iff:
$$\forall E' \in \mathcal{F}. \left(\left(E' \cap E \neq E \land E' \cap E \neq E' \right) \rightarrow P(E' \cap E) = P(E') P(E)\right)$$
\end{definition}

That is, an event $E$ is elementary if all other events which partially ``overlap'' with $E$ are independent of $E$. Note that this definition entails that any elementary event is automatically an effectively elementary event.

For any effectively elementary event $B$, and some other event $A$ we define the probability of $A$ conditioned on $B$ as:

$$P(A | B) = \frac{P(A \cap B)}{P(B)} \frac{P(\langle \rangle| B)}{P(B)}$$

Where $\langle \rangle$ is something we call the ``hindsight event.'' The hindsight event is not technically an event (it is not an element of $\mathcal{F}$). Rather, the hindsight event is a conceptual and notational tool. We define its conditionals as follows:

Let $\mathcal{E} \subseteq \mathcal{F}$ be the set of all effectively elementary events. Let 

\section{Definition of $\boxed{P}$}

Recall the definition of a random variable: A random variable is a measureable function $X : \Omega \rightarrow E$ where $E$ is some set. Typically $E = \mathbbm{R}$. The probability that $X$ takes on a value in a measurable set $S \subseteq E$ is $P(X \in S) = P(\{\omega \in \Omega | X(\omega) \in S\})$.

Consequently, the probability function $P$ \emph{is effectively} a random variable from $\Omega$ to $\mathbbm{R}$. Except, $P$ is defined on subsets of $\Omega$, not elements of $\Omega$. Therefore, $P$ implicitly defines a random variable $\boxed{P} : \Omega \rightarrow \mathbbm{R}$ where $\boxed{P}(\omega) = P(\{\omega\})$. The probability that $\boxed{P}$ takes on a value in a measurable set $S \subseteq \mathbbm{R}$ is just $P(\boxed{P} \in S) = P(\{\omega \in \Omega | \boxed{P}(\omega) \in S\})$.

\section{Another Incorrect Hindsight Definition}

Thinking of $P$ as implicitly defining a random variable $\boxed{P}$ allows us to mathematically define conditional probabilities in a broader way. First, we consider whether or not two singleton events $\omega_1, \omega_2 \in \Omega$ have ``the same probability information about them.'' To do this, we define the set of values $P(\{\omega\})$ is restricted to be.

$$S_P : \Omega \rightarrow \mathcal{P}([0, 1]).\ S_P(\omega) = \left\{p\ |\ \text{``}\left(P(\{\omega\}) \neq p\right)\text{''} \text{ is not defined to be true}\right\}$$

We then define classes of values that all have the same $S_P$: $I(\omega) = \{\omega' | \omega' \in \Omega \land S_P(\omega') = S_P(\omega)\}$. We denote the set of all the $S_P$ classes as $\mathcal{I} = \{J | \exists \omega \in \Omega.\ J = I(\omega)\}$.

With these definitions, we can note that when an event $\omega \in \Omega$ occurs, from a probability perspective this was effectively the same as some other event $\omega' \in I(\omega)$ occuring. Using that intuition, we define something we call the ``conditional hindsight event'' which we denote as $\langle \rangle$ given some event $E$ (i.e. ``$\langle \rangle | E$''). The conditional hindsight event is not technically an event, but it represents ``whatever happened.'' For any event $E \in \mathcal{F}$ we choose to define the conditional probabilities for the hindsight event as:

\begin{equation}\label{eqn:hindsight_finite}
P(\langle \rangle | \{\omega\} \cup (E \setminus \{\omega\})) = 
\begin{cases}
\sum_{\omega' \in I(\omega)} P(\omega')^2,& \text{if }|E| = 1 \\
P(\langle \rangle | \{\omega\}) + P(\langle \rangle | E \setminus \{\omega\})(1 - P(\langle \rangle | \{\omega\})),& \text{otherwise}
\end{cases}
\end{equation}

\textbf{TODO: DOUBLE CHECK THIS}

Given two events $A, B \in \mathcal{F}$, the conditional probability $P(A | B)$ is defined to be:

\begin{equation}\label{eqn:conditional_prob}
P(A | B) = \frac{P(A \cap B)}{P(B)} \cdot \frac{P(\langle \rangle | B)}{P(B)}
\end{equation}

\section{Incorrect Infinity Case for Defining Hindsight}

Or, if the sum is not computable due to infinitely many probabilities.

\begin{equation}\label{eqn:hindsight_infinite}
P(\langle \rangle | B) = \int_0^1 p P(\boxed{P} = p | B) dp
\end{equation}

\section{Fancy Partition for $\Omega$ and Hindsight Prob Before I Assumed all Singletons of $\Omega$ are in $\mathcal{F}$}

Let $B \in \mathcal{F}$ be an event. Let $S_B \subseteq \mathcal{F}$ be a partition of $\Omega$ defined as follows:

$$\text{Partition Space } \mathcal{S}_B = \left\{S \subseteq \mathcal{F}\ |\ \left(\forall E_1, E_2 \in S.\ E_1 \cap E_2 = \emptyset \right) \land \left(\forall E \in S.\ E \subseteq B \lor B \cap E = \emptyset\right)\right\}$$

$$S_B = \argmax_{S \in \mathcal{S}_B} \left\{ |S| \right\}$$

\section{Explanation and Philosophy of ``Probability'' Meaning}

One way people can think of probability functions is as models describing the underlying mechanics of how reality operates. Usually, this is an oversimplification. For example, when a die is rolled, typically the result is already deterministically fixed before someone rolls the die; there is not actually an equal ``chance'' of each side being rolled \footnote{Free will may also play a role, but even then the die roll is not probabilistic according to our view. While we believe free will is neither deterministic nor probabilistic, arguments for such views are certainly outside the scope of this paper.}. By contrast, it seems that some aspects of quantum physics \emph{may actually} operate in an inherently probabilistic fashion, whereby wave functions (i.e. probability distributions) ``collapse'' to a single value randomly according to the distribution. Whether or not quantum mechanics actually operates in this inherently probabilistic fashion is a subject for debate among physicists and philosophers. Our point here is not to take a stance on that issue but rather to point out a way in which it is \emph{conceptually possible} for reality to act inherently probabilitistically, but that we apply probabilistic models to many other kinds of situations wherein the models do not perfectly correspond to the underlying mechanics of the situation. Modeling die-rolling and other such things with probabilities is a fiction not to be taken too literally; however this does not keep the models from being practically useful, and in some ways these models correspond to the truth.

Some people prefer to think of probability functions as models of confidences and \emph{not} as models of reality (except perhaps indirectly because a person's confidences are themselves a sort of model). Sometimes probability calculations (Bayesian ones especially) are put forth as a model for human confidences and confidence updates. This has some empirical backing \textbf{TODO: GET SOURCES}, although, similar to how the underlying mechanics of die-rolling is not inherently probabilistic, it appears that human confidence updates are also not inherently probabilistic \textbf{CITE}. At the very least, our minds do not operate according to idealized Bayesian probability calculations \textbf{MORE SOURCES}. Leaving humans aside, sometimes Bayesian probability calculations are presented as how an ideally rational agent would update their confidences. This is a fascinating assertion, because, at least understood naively, it suggests that an ideally rational agent would model the world in a way which does \emph{not} perfectly correspond to how the world actually behaves \footnote{We offer the caveat that deterministic phenomenon can still, in a sense, be modeled as probabilistic. It's just that the conditional probabilities would have to be 1's or 0's for those phenomenon. Thus, ignoring free will - a bad thing to ignore, but oh well - one \emph{could perfectly model} real die-rolling ``probabilistically,'' \emph{if} the model took into account many, many more events than die-rolling models usually do. Such a model would need to take into account all the relevant events for the physics calculation.}.

Typically, a conditional probability for events $A$ and $B$ is defined to be $P(A | B) = \frac{P(A \cap B)}{P(B)}$. However, we define conditionals as:

\begin{equation}\label{eqn:conditional_def}
P(A | B) = \frac{P(A \cap B)}{P(B)} \frac{P(\langle B \rangle)}{P(B)}
\end{equation}

Where $\langle B \rangle$ denotes something we call ``the hindsight event of $B$'' and $P(\langle B \rangle)$ is ``the hindsight probability of $B$.'' The hindsight event is not, strictly speaking, an event. We define hindsight ``probabilities'' in the next section.

\subsection{Defining Hindsight}

Let $(\Omega, \mathcal{F}, P)$ be a probability space where $P$ is defined to be a member of its values set $\mathcal{V}(P)$ of probability measures over $\Sigma, \mathcal{F}$. Note that if $P$ is fully defined then $|\mathcal{V}(P)| = 1$.

Let $m : \mathcal{P}(\mathcal{V}(P)) \times [0, 1] \rightarrow \mathbbm{N}_0$ be a function defined as

$$m(S, q) = \min_{P' \in S} \left\{ \left| \{ \omega\ |\ \omega \in \Omega, P'(\{\omega\}) = q\} \right| \right\}$$

That is, $m(S, q) = k$ means that if we restrict the values $P$ could have to some subset $S \subseteq \mathcal{V}(P)$ (i.e. $P' \in S$ and $S \in \mathcal{P}(\mathcal{V}(P))$), there are $k$ or more elementary events where $P'$ says those events are each $q$-likely; in particular, $k$ is the largest of such values where this holds true. Now we define a set of probability values which \textit{always} appear in a subset $S \subseteq \mathcal{P}$ (if any) to be:

$$A: \mathcal{P}(\mathcal{V}(P)) \rightarrow \mathcal{P}([0, 1]);\ A(S) = \{q\ |\ m(S, q) > 0\}$$

Similarly, we define all the probabilities potentially associated with an event $\omega \in \Omega$ to be:

$$C: \mathcal{P}(\mathcal{V}(P)) \times \Omega \rightarrow \mathcal{P}([0, 1]);\ C(S, \omega) = \{q\ |\ \exists P' \in \mathcal{V}(P).\ P'(\{\omega\}) = q\}$$

Next, define $l : \mathcal{P}(\mathcal{V}(P)) \times \Omega \rightarrow [0, 1]$ and $u : \mathcal{V}(P) \times \Omega \rightarrow [0, 1]$ as:

\begin{equation*}
l(S, \omega) =
\begin{cases}
\frac{\sum_{q \in C(S, \omega)} q^2 \cdot m(S, q)}{\sum_{p \in C(S, \omega)} p \cdot m(S, p)},& \text{ if } C(S, \omega) \subseteq A(S) \\
0,& \text{ otherwise}
\end{cases}
\end{equation*}

\begin{equation*}
u(S, \omega) =
\begin{cases}
\frac{\sum_{q \in C(S, \omega)} q^2 \cdot m(S, q)}{\sum_{p \in C(S, \omega)} p \cdot m(S, p)},& \text{ if } C(S, \omega) \subseteq A(S) \\
1,& \text{ otherwise}
\end{cases}
\end{equation*}

Let $\mathbbm{P}_{\mathcal{V}(P)}$ be the set of all partitions of $\mathcal{V}(P)$. Then we define the functions $L: \Omega \rightarrow [0, 1]$ and $U: \Omega \rightarrow [0, 1]$ as:

$$L(\omega) = \max_{H \in \mathbbm{P}_{\mathcal{V}(P)}} \left\{ \min_{S \in H} \left\{ l(S, \omega) \right\} \right\}$$

$$U(\omega) = \min_{H \in \mathbbm{P}_{\mathcal{V}(P)}} \left\{ \max_{S \in H} \left\{ u(S, \omega) \right\} \right\}$$

Last but not least, $\mathcal{L}: \mathcal{F} \rightarrow [0, 1]$ and $\mathcal{U}: \mathcal{F} \rightarrow [0, 1]$:

\begin{equation*}
\mathcal{L}(E) = \frac{1}{P(E)} \cdot \sum_{\omega \in E} P(\{\omega\}) \left( L(\omega) + \sum_{\omega' \in E \setminus \{\omega\}} \frac{P(\{\omega'\}) (1 - P(\{\omega'\})) }{1 - L(\omega')} \right)
\end{equation*}

\begin{equation*}
\mathcal{U}(E) = \frac{1}{P(E)} \cdot \sum_{\omega \in E} P(\{\omega\}) \left( U(\omega) + \sum_{\omega' \in E \setminus \{\omega\}} \frac{P(\{\omega'\}) (1 - P(\{\omega'\}))}{1 - U(\omega')} \right)
\end{equation*}

With all this in place, we finally get that:

\begin{equation}\label{eqn:hindsight_def}
\mathcal{L}(E) \leq P(\langle E \rangle) \leq \mathcal{U}(E)
\end{equation}

%\begin{equation}\label{eqn:hindsight_finite}
%\forall E \in \mathcal{F}.\ P(\langle \rangle | E) = \sum_{p \in \{q\ |\ \exists \omega \in \Omega.\ P(\{\omega\}) = q\}} p P(\boxed{P} = p | E)
%\end{equation}

%\begin{equation}\label{eqn:hindsight_finite}
%\forall E \in \mathcal{F}.\ P(\langle \rangle | E) = \sum_{\omega \in \Omega} P(\{\omega\}) P(\boxed{P} = P(\{\omega\}) | E)
%\end{equation}

%\begin{equation}\label{eqn:hindsight_finite}
%\forall E \in \mathcal{F}.\ P(\langle \rangle | E) = \sum_{\omega \in \Omega} P(\{\omega\}) \frac{P\left(\boxed{P} = P(\{\omega\})\ \cap\ E\right)}{P(E)}
%\end{equation}

%And last but not least we define conditional probabilities for $\boxed{P}$ as follows:

%\begin{equation}
%\forall E \in \mathcal{F}.\ P(\boxed{P} = p | E) = 
%\begin{cases}
%\frac{P\left(\boxed{P} = p\ \cap\ E\right)}{P(E)},& \text{if this quantity is defined} \\
%p,& \text{otherwise}
%\end{cases}
%\end{equation}

\textbf{TODO: Define hindsight for continuous cases.}

\subsection{Independence}

Independence is often expressed in terms of conditional probabilities. That is, given two events $A$ and $B$, independence is often defined as $P(A | B) = P(A)$. Independence is also commonly defined as $P(A \cap B) = P(A) P(B)$. Normally these are mathematically equivalent. With our definitions, these two remain equivalent \emph{until} $P$ becomes undefined in which case they can come apart. Independence is conceptually meant to convey that one event's chance of occurring is not ``dependant'' on the other event having occurred.

%\begin{equation}
%P(A | B) = \sum_{something} something\ else
%\end{equation}



\section{Undefined Pairing Between Result Space and Probabilities}\label{sec:idea_warmup}

Consider sampling a distribution twice (independently), where the distribution is defined over a finite set of values $\mathcal{X}$. The random variable $X$ represents the first sampled value and the random variable $X'$ represents the second. The sampling of $X$ and $X'$ is performed according to the same distribution over $\mathcal{X}$. Let $P_\mathcal{X}$ be the probability function representing our confidences about the sampling process. In this case, $P_\mathcal{X}$ (i.e. our confidences about what values $X$ and $X'$ will take) will be undefined in the following manner:

\begin{itemize}
\item We know (define) the following about $P_\mathcal{X}$: We are given the multiset $M_{P_\mathcal{X}} = (S_{P_\mathcal{X}}, m_{P_\mathcal{X}})$, where $S$ is the support set defined to be $S = \{p\ |\ \exists x \in \mathcal{X}.\  P_\mathcal{X}(X = x) = p\}$ and where $m$ is the multiplicity function $m: S \rightarrow \mathbbm{N}$. The multiplicity function $m$ states how many different $x \in \mathcal{X}$ have a probability of $p$ for $p \in S$.

\item We are ignorant (leave $P_\mathcal{X}$ undefined) as follows: For any given $x \in \mathcal{X}$, we do not know $P_\mathcal{X}(X = x)$. In other words, we know the probabilities, but we do not know the bijection between those probabilities and the values $X$ (or $X'$ can take. This bijection exists implicitly in the very fact that $P_\mathcal{X}$ is defined to be a probability function.
\end{itemize}

Given a confidence $P_\mathcal{X}$ which is undefined in this way, if we observe the event $X = x_0$, we can then conclude the following about the chances that $x_0$ will be sampled again (i.e. our confidence that $X' = x_0$):

\begin{equation}\label{eqn:no_pairings}
P_\mathcal{X}(X' = x_0 | X = x_0) = \sum_{q \in M_{P_\mathcal{X}}} q^2
\end{equation}

We explain the meaning of this result and its derivation in the rest of this section. To get a more concrete understanding of what this result means, we recommend considering it in terms of the situation presented in the first challenge of The Monty Hallways Gameshow, where $X$ represents the first dairy product brought forth, $X'$ represents the second, the doors display the probabilities (i.e. $M_{P_\mathcal{X}}$) but the bijection between the dairy products and the doors is unknown. You observe a particular dairy product, Leonard's 2\% Milk, which corresponds to observing $X = x_0$. You are then asked about your confidence that if a door is opened again, it will bring forth Leonard's Milk again ($X' = x_0$).



In order to understand what we know about $P_\mathcal{X}$, we consider how confidences evolve as new information appears. Confidences change over time as new information becomes available. A particular confidence function (i.e. probability function) expresses confidences at a fixed time; a confidence function also expresses rules for updating one's confidences upon observing an event. The updated confidences (or a posteriori confidences) are written as conditional probabilities. For example, consider a probability function $P$, events $A$ and $B$, and Bayes' rule:

$$P(A | B) = \frac{P(B | A)P(A)}{P(B)}$$

The probability function $P$ gives us both a present confidence $P(A)$ that $A$ will/has occur(ed) \emph{as well as} giving us a new confidence value $P(A | B)$ that $A$ will/has occur(ed) upon observation of the event $B$.

Now, back to our situation with $X$, $X'$, and $P_\mathcal{X}$: Imagine that you observe the event $X = x_0$. This is analogous to observing the gallon of Leonard's 2\% Milk in the first challenge of our running example. \emph{Before} you observed $X = x_0$, you could speak of the probability that $X = x_0$ in terms of your confidence about whether that event would happen. \emph{After} you observe $X = x_0$, there is a sense in which your confidence about $X = x_0$ becomes 1; you no longer have any uncertainty about whether $X = x_0$. This is expressed in mathematical notation as the conditional probability $P_\mathcal{X}(X = x_0 | X = x_0) = 1$. However, you can also still think of what your confidence that $X = x_0$ \emph{was} before you observed it; this is expressed as $P_\mathcal{X}(X = x_0)$.

Consider our confidences about $X'$. We know that $X$ and $X'$ follow the same distribution: $\forall x \in \mathcal{X}.\ P_\mathcal{X}(X = x) = P_\mathcal{X}(X' = x)$. Remember that $P_\mathcal{X}(X' = x_0)$ is, in a sense, undefined; we are given the collection of relevant probabilities via multiset $M_{P_\mathcal{X}} = (S_{P_\mathcal{X}}, m_{P_\mathcal{X}}$, but we do not know the bijection between the probabilities in $M_{P_\mathcal{X}}$ and the values in $P_\mathcal{X}$. Since we know $M_{P_\mathcal{X}}$, we know that the value $x_0$ was sampled with one of the probabilities in $M_{P_\mathcal{X}}$. This means that we can consider the chances (i.e. our confidence) that the sampled value $x_0$ was sampled with a given probability $p \in S_{P_\mathcal{X}}$. That is, for any $p \in S_{P_\mathcal{X}}$, we can be $p\cdot m_{P_\mathcal{X}}(p)$ confident that the event $X = x_0$ had a chance $p$ of occurring. Put mathematically:

$$\forall p \in S_{P_\mathcal{X}}.\ P_\mathcal{X}\left(P_\mathcal{X}(X = x_0) = p | X = x_0\right) = p \cdot m_{P_\mathcal{X}}(p)$$

In terms of The Monty Hallways Gameshow, the event ``$P_\mathcal{X}(X = x_0) = p$'' is the event that a door was opened which had probability $p$ written on the door. Obtaining the equation above corresponds to counting all the doors with probability $p$ written on them ($m_{P_\mathcal{X}}(p)$ doors total) and then computing the chances of having opened one of those doors ($p \cdot m_{P_\mathcal{X}}(p)$).

Similarly, we can consider the chances that $X'$ will equal $x_0$ as conditioned on the event that $P_\mathcal{X}(X = x_0) = p$. Since $P_\mathcal{X}(X' = x_0) = P_\mathcal{X}(X = x_0)$, this just becomes:

$$P_\mathcal{X}(X' = x_0 | P_\mathcal{X}(X = x_0) = p) = p$$

Putting it all together, we can derive the following confidence:

\begin{align*}
P_\mathcal{X}(X' = x_0 | X = x_0) &= \sum_{p \in S_{P_\mathcal{X}}} P_\mathcal{X}(X' = x_0 | X = x_0, P_\mathcal{X}(X = x_0) = p) P_\mathcal{X}(P_\mathcal{X}(X = x_0) = p | X = x_0) \\
 &= \sum_{p \in S_{P_\mathcal{X}}} P_\mathcal{X}(X' = x_0 | X = x_0, P_\mathcal{X}(X = x_0) = p) \cdot p \cdot m_{P_\mathcal{X}}(p) \\
 &= \sum_{p \in S_{P_\mathcal{X}}} p^2 \cdot m_{P_\mathcal{X}}(p) \\
 &= \sum_{q \in M_{P_\mathcal{X}}} q^2
\end{align*}

Thus, \emph{even though} we do not know which probabilities in $M_{P_\mathcal{X}}$ correspond to which values in $\mathcal{X}$, after observing a value $x_0$ be sampled we arrive at a particular confidence that $x_0$ will be sampled again. The sheer fact that $x_0$ had to have been sampled via \emph{one of} the probabilities in $M_{P_\mathcal{X}}$ gives us a confidence that $x_0$ will be sampled again.

Remember that the sampling of $X$ and $X'$ occur independently. Statisticians typically work with fully defined probability functions. When probability functions are fully defined, receiving information about the state of one random variable does not provide any information about another independent random variable. However, in this case, seeing the event $X = x_0$ moved our confidence in the event $X' = x_0$ from being undefined to being the exact value $\sum_{q \in M_{P_\mathcal{X}}} q^2$. That is, $P_\mathcal{X}(X' = x_0 | X = x_0) \neq P_\mathcal{X}(X' = x_0)$. This \emph{should not} be taken as saying $X$ and $X'$ are not independent. Rather, in this case the conditioning on an event (the event $X = x_0$) does something conditioning normally does not do; here the conditioning gives more information about $P_\mathcal{X}$ itself. This distinction is crucial to a proper interpretation of these results.

This result serves as the conceptual foundation for results when even less is known about $P_\mathcal{X}$. That is, the concepts in this section allow us to say things about our confidence when our confidence is even less defined than $P_\mathcal{X}$.

\section{Completely Undefined Probabilities}\label{sec:completely_undefined_probs}

We just explored in Section~\ref{sec:idea_warmup} how in \emph{some cases} we can define a probability even when certain aspects of the probability distribution are undefined. Here we extend those results to a case where \emph{nothing} about the probability function is defined beyond the fact that it is a probability function.

\begin{figure}
% The \phantomcaption allows for an invisible caption.
% \phantomcaption{}\label{fig:second_story_task}
\begin{tcolorbox}[colback=green!10!white,colframe=green!50!black,before upper={\parindent15pt},title=\textbf{The Monty Hallways Gameshow - Second Challenge}]
For your next challenge, you are once again brought into a long hallway. This time the doors are completely blank. Your host assures you that each door corresponds to a unique dairy product and that there is a probability distribution over the doors; the probabilities are hidden. The collection of relevant dairy products is pictured on one of the walls. Before anything occurs, the host points at the image of Dillard's Half-and-Half, asking, ``What is your confidence you'll see Dillard's come from a door in this hallway?''

You reply, ``Well, my confidence is rather undefined at the moment.''

``Of course! Of course!'' says your energetic host, ``How about a minimum confidence?''

``A minimum confidence? Is that like a lower bound on my confidence?''

``Indeed.''

``I'm afraid I cannot lower-bound my confidence above zero.'' you say.

``Well done! You're properly cautious. Now for the big question.''

You are temporarily blindfolded; when un-blindfolded, you see a box of Harriet's Best cream cheese. The gameshow host says, ``Tell me, what is your minimum confidence that if this process were to be repeated, the product would be Harriet's Best cream cheese again?'' Your brow furrows. You spend a while in thought and then come up with an answer. ``Wonderful!'' exclaims the host, ``Only two challenges remain...''

\ 

(The math behind this case is presented in Section~\ref{sec:completely_undefined_probs}.)
\end{tcolorbox}
\end{figure}

Our setup mirrors the situation in Section~\ref{sec:idea_warmup}. This time we sample twice independently from a finite set $\mathcal{Y}$. The random variables $Y$ and $Y'$ represent the first and second samples respectively. The sampling of $Y$ and $Y'$ is performed according to the same distribution over $\mathcal{Y}$. We represent our confidence about which values will be sampled via the confidence function $P_\mathcal{Y}$. In this case, we leave our confidence function \emph{completely} undefined. We are not even given a multiset similar to $M_{P_\mathcal{X}}$ from Section~\ref{sec:idea_warmup}. We observe the event $Y = y_0$ for some $y_0 \in \mathcal{Y}$. In this case we do not have enough information to get an exact confidence that $y_0$ will be sampled again. However, we \emph{can} consider a worst case application of Equation~\ref{eqn:no_pairings} and use that worst case to lower-bound our confidence that $y_0$ will be sampled again as follows:

\begin{equation}\label{eqn:total_ignorance_bound}
P_\mathcal{Y}(Y' = y_0 | Y = y_0) \geq \frac{1}{|\mathcal{Y}|}
\end{equation}

We explain the meaning and derivation of this result in the rest of this section. For a more concrete version of this problem, check out the second challenge of The Monty Hallways Gameshow story. In the gameshow story, the event $Y = y_0$ corresponds to seeing Harriet's Best cream cheese, and the event $Y' = y_0$ represents seeing the cream cheese again. In the story, you know that there is \emph{some} probability distribution governing the sampling process, but you know nothing about that distribution.

Key to this result is the shift from having an undefined or exact confidence to having a lower bound on a confidence. Conceptually, a lower bound of $\alpha$ on a confidence can be understood in several ways. We list two:

\begin{enumerate}
    \item If your confidence is a measure of your belief about a rate of occurrence, then the lower bound of $\alpha$ corresponds to thinking the event is at least $\alpha$-likely to occur.
    \item If your confidence is solely a measure of how much you believe some event $E$ will/has occur(ed) with no reference to an underlying probabilistic mechanism behind $E$, then the meaning of the lower bound is less easy to define. When confidences are understood as ``amounts of belief,'' then a specific numeric confidence corresponds to a specific amount of belief and a completely undefined confidence corresponds to some kind of state of total agnosticism. In this light, a confidence lower bound would correspond to something like an agnosticism which is \emph{restricted} to a particular range of amounts of belief.
\end{enumerate}

We do not claim this is an exhaustive list of the ways to interpret lower bounds on confidences. Our goal here is simply to ballpark ways of interpreting the mathematical results such that the math meaningfully corresponds to the realities probabilities-as-confidences are meant to model.

Given these notions of a bound on a confidence, how did we obtain the bound in Equation~\ref{eqn:total_ignorance_bound}? We did so via an extension of the results contained in Equation~\ref{eqn:no_pairings}. For Equation~\ref{eqn:no_pairings}, we were given the multiset of probabilities associated with the sampling process. In this context, we no longer have that multiset. However, we can consider all possible multisets of probabilities and see if our confidence would always be at least certain amount no matter which multiset was applied. If so, then we can conclude that even without the knowledge/confidence contained in $M_{P_\mathcal{X}}$ from Section~\ref{sec:idea_warmup}, we know that \emph{whatever} that knowledge/confidence is, if we had it and our confidence would be at least $\alpha$, then our confidence can be at least $\alpha$. This can be formalized as follows:

Like $M_{P_\mathcal{X}}$ from Section~\ref{sec:idea_warmup}, let $M_{P_\mathcal{Y}} = (S_{P_\mathcal{Y}}, m_{P_\mathcal{Y}})$ be the multiset of probabilities (our confidences) that values of $\mathcal{Y}$ will be sampled. That is, $S_{P_\mathcal{Y}} = \{p\ |\ \exists y \in \mathcal{Y}.\ P_\mathcal{Y}(Y = y) = p \}$ and $m_{P_\mathcal{Y}}$ is the multiplicity function of those probabilities. In Section~\ref{sec:idea_warmup}, we were \emph{given} (or defined) $M_{P_\mathcal{X}}$ and by doing so partially defined $P_\mathcal{X}$. In this case, we \emph{are not} given (or do not define) $M_{P_\mathcal{Y}}$. Rather, we just defined the relationship between $M_{P_\mathcal{Y}}$ and $P_\mathcal{Y}$. We know from Equation~\ref{eqn:no_pairings} that $P_\mathcal{Y}(Y' = y_0 | Y = y_0) = \sum_{q \in M_{P_\mathcal{Y}}} q^2$. In this case, because $M_{P_\mathcal{Y}}$ is undefined, this value is also undefined.

Fortunately, we can still apply a worst case analysis. Let $\mathcal{M}^{P_\mathcal{Y}}$ be the set of all possible values for $M_{P_\mathcal{Y}}$. That is let:

$$\mathcal{M}^{P_\mathcal{Y}} = \left\{M = (S, m)\ |\ |M| = |\mathcal{Y}| \land \left(\forall p \in S.\ p \geq 0.\right) \land \sum_{p \in S} p \cdot m(p) = 1 \right\}$$

Then with this definition of $\mathcal{M}^{P_\mathcal{Y}}$, we can derive the bound in Equation~\ref{eqn:total_ignorance_bound} as follows.

\begin{align*}
P_\mathcal{Y}(Y' = y_0 | Y = y_0) &= \sum_{q \in M_{P_\mathcal{Y}}} q^2 \\
&\geq \min_{M \in \mathcal{M}^{P_\mathcal{Y}}} \left\{ \sum_{q \in M} q^2 \right\} = \sum_{i = 1}^{|\mathcal{Y}|} \left(\frac{1}{|\mathcal{Y}|}\right)^2 = \frac{1}{|\mathcal{Y}|}
\end{align*}

In other words, the value for $M_{P_\mathcal{Y}}$ that minimizes Equation~\ref{eqn:no_pairings} is $M_{P_\mathcal{Y}} = \left\{\frac{1}{|\mathcal{Y}|}, \frac{1}{|\mathcal{Y}|}, ..., \frac{1}{|\mathcal{Y}|}\right\}$ which would yield a confidence of $\frac{1}{|\mathcal{Y}|}$. Thus this becomes the lower bound.

Having established this method for obtaining confidence lower bounds, we now turn to lower-bounding confidences in more complex scenarios.

\section{Multiple Distributions - One Undefined}\label{sec:hypothesis_testing_math}

In Section~\ref{sec:completely_undefined_probs} we introduced a way to obtain a lower bound on a confidence that a result would repeat when our confidence function was a completely undefined probability function. However, sometimes a person is presented with a context where their model for what occurs is a mix of defined and undefined probability functions. Single hypothesis testing is a classic example of this situation, where the null hypothesis' probability function over the result space is (usually) completely defined but the alternative hypothesis (usually) leaves the probabilities over the result space undefined. In this section we move our analysis toward more complex situations, including that of null hypothesis testing.

As usual, we consider sampling twice from a set. This time we sample from the finite set $\mathcal{Z}$. We represent our uncertainty about sampling with the probability function $P_\mathcal{Z}$. In this case we actually have \emph{two different} distributions with which to sample from $\mathcal{Z}$, the ``heads distribution'' and the ``tails distribution.'' Each time we sample from $\mathcal{Z}$, we first flip a coin to choose which distribution to sample with. The coin is biased and flips heads (event $H$ the first time, $H'$ the second time) with probability $P_\mathcal{Z}(H) = P_\mathcal{Z}(H')$ and tails (events $T$, $T'$) with probability $P_\mathcal{Z}(T) = P_\mathcal{Z}(T') = 1 - P_\mathcal{Z}(H)$. Let $Z$ be the random variable representing our first sample and $Z'$ represent the second.

In this section we let the distribution associated with flipping heads be completely defined. That is, $P_\mathcal{Z}(Z | H)$ and $P_\mathcal{Z}(Z' | H)$ are completely defined. However, we will leave $P_\mathcal{Z}(Z | T)$ and $P_\mathcal{Z}(Z' | T)$ completely undefined like in Section~\ref{sec:completely_undefined_probs}. Under this setup, we obtain our first sample, \emph{but} we do not get to see the coin; we just observe the event $Z = z_0$. Having observed $Z = z_0$, we can obtain the following confidence bound:

\begin{equation}\label{eqn:hype_basis}
P_\mathcal{Z}(Z' = z_0 | Z = z_0) \geq P_\mathcal{Z}(Z' = z_0 | H)P_\mathcal{Z}(H') + \frac{1}{|\mathcal{Z}|}P_\mathcal{Z}(T')^2
\end{equation}

We proceed to explain and derive this result in the rest of this section. To understand the above bound more concretely, consider the example in the third challenge of the Monty Hallways Gameshow. Here heads corresponds to the distribution over the blue doors in the example, and tails corresponds to the yellow doors. The event $Z = z_0$ represents seeing the first block of Grover's Cheddar.

\begin{figure}
% The \phantomcaption allows for an invisible caption.
% \phantomcaption{}\label{fig:third_story_task}
\begin{tcolorbox}[colback=green!10!white,colframe=green!50!black,before upper={\parindent15pt},title=\textbf{The Monty Hallways Gameshow - Third Challenge}]
You are brought to the third and final challenge of today's show. This time there are two sets of doors, colored blue and yellow. On the blue doors, both probabilities and pictures of the dairy products are visible. The yellow doors are completely blank, but your host assures you that for every product shown on a blue door there is a corresponding yellow door and that the yellow doors have some other probability distribution associated with them. To sample a product, your host will first (fairly) flip a fair coin; one side is blue - the other, yellow. The color of the coin flip will determine which set of doors (and thus which distribution) is used to select a dairy product.

\ 

You are blindfolded and neither see the result of the coin flip nor which door opens. When unblindfolded, you see a block of Grover's Cheddar. ``Now...'' the host asks you, ``You must tell me, what is your minimum confidence that if we use the same set of doors (blue or yellow, you do not know) and sample a product again, we'll get another block of Grover's Cheddar?'' This one takes you a while, but after some careful calculations, you offer your answer. Your host is thrilled. ``Congratulations! Someone get this winner their half-and-half!''

\ 

(The math behind this case is presented in Section~\ref{sec:hypothesis_testing_math}.)
\end{tcolorbox}
\end{figure}

Equation~\ref{eqn:hype_basis} appears to use something like our bound from Section~\ref{sec:completely_undefined_probs}. Perhaps the most surprising thing about Equation~\ref{eqn:hype_basis} is that $P_\mathcal{Z}(T')$ is squared. While we use the same sort of reasoning we used in Section~\ref{sec:completely_undefined_probs}, here in Equation~\ref{eqn:hype_basis} we square $P_\mathcal{Z}(T')$ because there's only a $P_\mathcal{Z}(T') = P_\mathcal{Z}(T)$ chance that the result $Z = z_0$ was actually sampled using $P_\mathcal{Z}(\cdot | T)$. In other words,

\bibliography{references}
\bibliographystyle{ieeetr}

\end{document}

